A Dyadic Simulation Approach to Efficient Range-Summability

Efficient range-summability (ERS) of a long list of random variables is a fundamental algorithmic problem that has applications to three important database applications, namely, data stream processing, space-efficient histogram maintenance (SEHM), and approximate nearest neighbor searches (ANNS). In this work, we propose a novel dyadic simulation framework and develop three novel ERS solutions, namely Gaussian-dyadic simulation tree (DST), Cauchy-DST and Random Walk-DST, using it. We also propose novel rejection sampling techniques to make these solutions computationally efficient. Furthermore, we develop a novel k-wise independence theory that allows our ERS solutions to have both high computational efficiencies and strong provable independence guarantees.

==> sections/application.tex <==
\color{black}
\section{Application of Dyadic Simulation on ANNS-$L_1$}\label{sec:ann}
% NOTE: organization of paper       we may need to move the backgrounds of ANN forward and add some contents in introduction.ANNS-$L_1$ 

%[background on ANNS and LSH]

\begin{comment}
We now state and prove a surprising result that get the better of both worlds:  
For $L_2$-norm estimation only, when 4-wise independent hash functions 
are used in each underlying DST, 
our algorithm can achieve the same accuracy guarantees using the same
number of accumulators as when the underlying RVs are assumed to be i.i.d.

Recall that an accumulator $A$ has value $\sum_{i=0}^{U-1}\sigma_i X_i$ at the end of a data stream.
For $L_2$-norm estimation, each $X_i$ has a standard Gaussian distribution $\mathcal{N}(0, 1)$.
Hence, when the underlying RVs $X_0$, $X_1$, $\cdots$, $X_{U-1}$ are assumed
to be independent, each
%In the offline stage, 
%this accumulator $A=\sum_{i=0}^{U-1}\sigma_i X_i$, because each point-update above that increases $A$ by $\delta_t X_{i_t}$ also increases $\sigma_{i_t}$ by $\delta_t$, so the increment is the same for both sides of the equation.
%By the stability property of Gaussian distribution, after the online stage, each accumulatorTherefore, 
accumulator $A_j$, $j = 1, 2, \cdots, r$, has distribution $\mathcal{N}(0, d_2^2)$, where its 
variance $d_2^2 = \sigma_1^2 + \sigma_2^2 + \cdots + \sigma_n^2$ is the squared $L_2$-norm of the data stream.
%Recall that the sketch is comprised of the $r$ accumulators denoted as $A_1, A_2, \cdots A_r$.  
In our algorithm, like in the original algorithm~\cite{stabledist}, the estimator for the squared $L_2$ norm $d_2^2$ is
%Indyk's algorithm~\cite{stabledist} uses the  for , %square of $L_2$ norm
%, we will use the following UMVUE\cite{sttinf} for $d^2_2$, the variance of Gaussian samples whose expectation is known,(for  $0$), which comes from~\cite{ams},  =d_2^2
$
\hat{d_2^2}= \left(A^2_1+A^2_2 + \cdots+A^2_r\right)/r. 
$

%estimated from the following UMVUE (uniform minimum variance unbiased estimator)

We have $E[\hat{d^2_2}] =1/r\cdot \sum_{j=1}^r E[A^2_j] $ by the linearity of expectation.
Note that $A_1, A_2, \cdots, A_r$ are i.i.d. since they are generated by independent DSTs. 
%With a slight abuse of notation, we denote their common distribution as $A$.
Hence we have $E[(\hat{d^2_2})^2] = \left(\sum_{j=1}^r E[A^4_j] +\right.$ $\left. 2 \sum_{j=1}^r\sum_{j'=j+1}^r E[A^2_j]E[A^2_{j'}]\right)/r^2$. 
By~\autoref{th:fourwise}, the values of each $E[A_j^2]$ and $E[A_j^4]$, and hence the values of $E[\hat{d^2_2}]$ and $E[(\hat{d^2_2})^2]$
remain unchanged whether the underlying RVs are 4-wise independent or all-wise independent;  and hence so does $Var[\hat{d^2_2}] =E[(\hat{d^2_2})^2]  - E^2[\hat{d^2_2}]$.   
In other words, 
the statistical efficiency of the estimator $\hat{d_2^2}$ remains the same whether the underlying RVs are 4-wise independent or all-wise independent.

\begin{theorem}\label{th:fourwise}
	Let $A=\sum_{i=0}^{U-1}\sigma_i X_i$ be an accumulator as defined above, and $X_0, X_1$, $\cdots$, $X_{U-1}$ be standard Gaussian RVs.  Then the values of $E[A^2]$ and $E[A^4]$ remain the same whether
	the underlying RVs are $4$-wise independent or all-wise independent.
	% with $E[X] = 0$ and $Var[X] = 1$, then the probability that the estimator in \autoref{eq:gauesti} deviates from $d^2_2$ by at more than $\epsilon d^2_2$ is at most $1/8$. %the probability for an estimate to fail (to have larger relative error than $\epsilon$ can be bounded by $1/4$ with $r = O(1/\epsilon^2)$ accumulators. and use the median of all estimates as the final estimate that all follow marginal distribution $\mathcal{N}(0, 1)$n independently generated 
	%To further boost the success probability to $1-\delta$ for arbitrarily small $\delta$, the streaming algorithm only needs to return the median of $2\log 1/\delta$ independent estimations as above. because they are generated by independent DSTs,
	%	$E[A^2] = \sum_{i=0}^{U-1}\sigma_i^2 E[X^2] = d_2^2$ and $Var[A^2] = \sum_{i=0}^{U-1}\sigma_i^4 (E[X^4]-E^2[X^2]) + 4\sum_{i=0}^{U-1}\sum_{i'=i+1}^{U-1}\sigma_i^2\sigma_{i'}^2 E[X^2]=2d^4_2$. 
\end{theorem}

The proof of \autoref{th:fourwise} is a straightforward adaptation of that of Theorem 2.2 in \cite{ams}, in which each underlying RV is a single-step random walk.

%LSH~\cite{Indyk_ANN_1998} is one of the most popular ANNS solution approaches. 
%In LSH, the key intellectual component of an LSH scheme is its hash function family 
%$\mathcal{H}$.
%Any function $h$ sampled uniformly at random from $\mathcal{H}$ has the following 
%nice collision property:  It maps two distinct points in $\mathcal{D}$ to the same hash %value with probability $p_1$
%if they are close to each other (say no more than distance $r_1$ apart) and with probability $p_2 < p_1$ if they are far apart (say more than $r_2 > r_1$ apart), respectively. 

%In this section, we introduce MP-GRW-LSH, the application of dyadic simulation on ANNS-$L_1$ that improves MP-RW-LSH~\cite{mprwlsh} by scaling highly efficient ANNS queries to huge universes without having to store a large precomputed table. We also show that dyadic simulation is the preferred option over existing range-summable schemes such as EH3~\cite{feigenbaum} on ANNS, because the performance of ANNS is determined by the distribution of the generated range-sums. 
%While the former has a theoretical guarantee on this, the latter does not and can have degraded performances for worst-case queries.
\end{comment}

In this section, we first describe an ERS 
problem that arises in MP-RW-LSH, the aforementioned multi-probe LSH solution
for ANNS-$L_1$ proposed in~\cite{mprwlsh}.  Then we study why this problem cannot be robustly
solved using an existing ERS solution called EH3~\cite{feigenbaum}.  Finally, we describe MP-GRW-LSH, a slight variant of MP-RW-LSH that 
can cleanly and robustly solve this problem using our Gaussian-DST.
% Gaussian-DST and
%has nearly identical query efficacy and better efficiency as 
%MP-RW-LSH.





%[change s to vector t, q to vector q]
\begin{comment}
In ANNS-$L_1$, given a query point $\vec{\mathbf{q}}$, 
we search in a massive dataset $\mathcal{D}$, which lies in a space of high dimensionality (say $m$),  
for one or more points $\mathbf{s}$ in $\mathcal{D}$ that are \emph{among the closest} to $\vec{\mathbf{q}}$ according to the $L_1$ distance.  
Here the $L_1$ distance between any two $m$-dimensional points $\vec{\mathbf{s}}= \langle s_1, s_2, \cdots, s_m\rangle$ and $\vec{\mathbf{q}} = \langle q_1, q_2, \cdots, q_m\rangle$, denoted as $  \|\vec{\mathbf{q}} - \vec{\mathbf{s}}\|_1$, 
is defined as  $\sum_{j=1}^m |q_j - s_j|$.
\end{comment} 
%\subsection{Locality-Sensitive Hashing (LSH)}d(\mathbf{q}, \mathbf{s})=
\subsection{The RW-LSH Algorithm}

LSH~\cite{Indyk_ANN_1998} is one of the most popular ANNS solution approaches. 
%JFM-1 (new) We first describe RW-LSH, % (Random Walk LSH), 
% and then show how to use dyadic simulation to efficiently implement our ERS-based variant called BM-LSH.(an $m$-dimensional dataset) 
In an LSH scheme, typically a vector of $M > 1$ LSH functions $\vec{\mathbf{g}} = \langle g_1$, $g_2$, $\cdots$, $g_M\rangle$ 
are used to map each point $\vec{\mathbf{s}}$ in $\mathcal{D}$ to an $M$-dimensional vector of independent hash values 
${\overrightarrow{\mathbf{g}(\mathbf{s})}} = \langle g_1(\vec{\mathbf{s}}), g_2(\vec{\mathbf{s}}), \cdots, g_M(\vec{\mathbf{s}})\rangle$.  
This point $\vec{\mathbf{s}}$ is to be stored in a hash bucket indexed 
% \textbf{Jingfan: We do not need to mention $g(\cdot)$ since use hash vector as index in hash table is common sense for readers and our iDEC also write as ``vector as hash key''.}
%({\color{red} say using a conventional hash function $g(\cdot)$}) 
by the vector ${\overrightarrow{\mathbf{g}(\mathbf{s})}}$;
hence we identify this hash bucket as ${\overrightarrow{\mathbf{g}(\mathbf{s})}}$. 
% \textbf{Huayi: I think we need the following sentence to explain each hash table needs one LSH function vector and the meaning of $n$.}
%{\color{red} These $n$ points in $\mathcal{D}$ are 
%stored in a hash table
%using their corresponding vectors as hash keys.}
%({\it e.g.}, the point $\beta$ is to be stored in hash bucket %
%$g(\langle h_1(\beta), h_2(\beta), \cdots, h_k(\beta)\rangle)$.  
Then given a query point $\vec{\mathbf{q}}$, the search procedure, in a standard LSH solution, is to
probe all points in the \emph{epicenter bucket} ${\overrightarrow{\mathbf{g}(\mathbf{q})}}$
%bin 
%that the vector $\langle h_1(\alpha), h_2(\alpha), \cdots, h_k(\alpha)\rangle$ would be inserted into, 
in the hope that 
some nearest neighbors of $\vec{\mathbf{q}}$ are mapped to the same vector (bucket). %bin.
%We regard this search procedure as hard-decision decoding, since 
%the query point $\alpha$ is ``decoded'' to precisely the vector 
%$\langle h_1(\alpha), h_2(\alpha), \cdots, h_k(\alpha)\rangle$ and only the corresponding bucket is probed. 
%$\mathbf{s}\in\mathbb{Z}^{m\smash[t]{\mathstrut}}_{\geq 0}$ is a data or query point,

%A standard LSH solution is one in which only a single hash bucket is searched in each hash table.   is one in which the algorithm(as in standard LSH)


Unlike a standard LSH solution,
a multi-probe LSH solution probes not only the epicenter bucket, but also 
$T > 0$ other nearby buckets whose success probabilities (of containing a nearest neighbor) are among the highest.
%$T$  (excluding the epicenter bucket).
Among LSH solutions, a multi-probe one, if it can be found, is arguably the most desirable one because its index size for achieving the 
same query accuracy is much smaller than that of a standard LSH solution~\cite{mprwlsh}.  


%We now describe what 

%{\color{blue} (Add by Huayi) To simplify notation, we focus on only one hash function $g(\vec{\mathbf{s}})$ and drop its subscript in the sequel.}
An LSH function $g(\vec{\mathbf{s}})$ in RW-LSH~\cite{mprwlsh}
%the first multi-probe solution for ANNS-$L_1$. % and in BM-LSH, our ERS-based variant of RW-LSH that has an efficient implementation with dyadic simulation. 
%To simplify notation, we focus on only one hash function $g(\mathbf{s})$ and drop its subscript in the sequel. 
%l, with the understanding that each $g_j(\mathbf{s})$, $j=1,2,\cdots, M$, is an independent instance of $g(\mathbf{s})$.
%In both LSH schemes, same
takes the  following form:  
$g(\vec{\mathbf{s}}) \triangleq  \left\lfloor (f(\vec{\mathbf{s}}) + B)/W \right\rfloor$, 
where  $W > 0$ is a constant and $B$ is a RV (fixed after generation) uniformly distributed in $[0, W]$. % In this section and~\autoref{sec:eva}, we reuse the letter $W$, since it will not cause confusions.
Here $f(\vec{\mathbf{s}})$ is called the \emph{raw hash value} of $\vec{\mathbf{s}}$. 


Before we describe such an $f(\cdot)$, we need to introduce some notations.
Let $\tau$ be a sequence of independent RVs $X_0$, $X_1$, $X_2$, $\cdots$ 
%{\bf [add superscript $\tau$ to them ]  JFM: maybe not} 
that each has a single-step random walk distribution.
When necessary, we call $\tau$ a {\it strict} random walk sequence to emphasize the (strict) independence among its steps.
% {\bf[delete?] and to highlight its difference with  
%a random walk (sequence) whose steps are strongly correlated. } 
Let $q$ and $s$ be two nonnegative integers such that $q \le s$.  
We define $S^{\tau}[q, s)$ as the $(s-q)$-step random walk $X_q+ X_{q+1} + \cdots + X_{s-1}$.  
Clearly, $S^{\tau}[q, s)$ is also a range-sum, with the underlying RVs being the sequence $\tau$.  
For notation convenience in the following, we also define the value of $S^{\tau}[s, q)$ as $-S^{\tau}[q, s)$.

In RW-LSH, the raw hash value function $f(\cdot)$ is parameterized by a vector of $m$ (which is also the dimension of the dataset $\mathcal{D}$) 
such strict random walk sequences $\vec{\bm{\tau}} = \langle \tau_1, \tau_2, \cdots, \tau_m \rangle$ that 
are  independent.
%Each $\tau_j$ is a sequence of single-step random walks that are mutually independent. 
%i.i.d. random variables, each of which takes value $1$ or $-1$ with equal probability $1/2$;  the value of each random variable is fixed 
%once it is generated. %, just as the computational model in \autoref{sec:overview}.  
%\textbf{In the sequel, we refer to such a random walk with mutually independent steps as a ``real'' random walk, in contrast to other instances that does not guarantee mutual %independent steps.}
Given a data point $\vec{\mathbf{s}} = \langle s_1, s_2, \cdots, s_m \rangle$, the raw hash value $f(\vec{\mathbf{s}})$ is defined as $\sum_{j=1}^m S^{\tau_j}[0, s_j)$.
In other words, $f(\vec{\mathbf{s}})$ is the result of randomly walking $s_1$ steps along sequence $\tau_1$, $s_2$ steps along $\tau_2$, $\cdots$, and $s_m$ steps along $\tau_m$.
RW-LSH requires that each $s_j$, $j = 1, 2,\cdots, m$, be a nonnegative even integer.  

%This requirement is imposed on all data points in $\mathcal{D}$  
%and all query points, to guarantee a monotonocity condition that, as we will explain shortly, qualifies a hash function family as LSH.  

We now fix a query point $\vec{\mathbf{q}}$ and a point $\vec{\mathbf{s}}$ in the dataset $\mathcal{D}$.  
We now state some facts that will be used both next and soon in~\autoref{sec:grwlsh}.
Let $d_1$ be the $L_1$ distance between $\vec{\mathbf{q}}$ and $\vec{\mathbf{s}}$, that is, $d_1 = \sum_{j=1}^m |s_j-q_j|$.
%$d_1$ is a nonnegative integer since every $s_j$ and $q_j$ is.
%The performance of LSH heavily relies on the distribution of 
Then, $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})= \sum_{j=1}^m\left(S^{\tau_j}[0, s_j) -S^{\tau_j}[0, q_j) \right) =  \sum_{j=1}^mS^{\tau_j}[q_j, s_j)$~\cite{mprwlsh}. 
%Here, we have to clarify a subtle issue on notation. We have
%defined the range-sum $S^{\tau_j}[q_j, s_j)$ only when $q_j\leq s_j$, but it might be $q_j > s_j$, in which case we define $S^{\tau_j}[q_j, s_j) \triangleq -S^{\tau_j}[s_j, q_j)$.
%Since $f(\mathbf{s})  - f(\mathbf{q})$  .
%the random walks   $\langle \tau_1, \tau_2, \cdots, \tau_m \rangle$ are mutually independent, and because$f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$ has the same distribution as a  
%each   has the distribution of $d_1$-step random walk, because it is the sum of $m$ independent range-sums,
Note that each range-sum $S^{\tau_j}[q_j, s_j)$ has the distribution of a $|s_j - q_j|$-step random walk \textbf{($X^{*|s_j - q_j|}$ where $X$ is a single-step random walk)}
whether $q_j\leq s_j$ or $q_j> s_j$, since (the pdf of) every underlying single-step random walk is symmetric about $0$.
Since the random walks $S^{\tau_j}[q_j, s_j)$, $j = 1, 2, \cdots, m$, are independent (as they are along independent sequences), $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$
has the distribution of a $d_1$-step random walk, and hence is parameterized only by  $d_1$.
When $d_1$ is not small (say when $d_1 > 25$), this distribution can be closely approximated as $\mathcal{N}(0, d_1)$.
It has been shown in~\cite{mprwlsh} that this distribution being approximately Gaussian leads to every nice property of RW-LSH and its multi-probe 
extension MP-RW-LSH.

%highly efficient (w.r.t. query time) and
%effective (w.r.t. query accuracy).

 %(thanks to sin$|q_j - s_j|$-step random walk gle-step random walk has a symmetric distribution about 0).the number of steps
% Here we need to use a property of  (and the same for Gaussian distribution $X$): and, it because, the distribution of the range-sum of $|s_j-q_j|$ i.i.d. steps,
 %$S^{\tau_j}[s_j, q_j)$ is symmetric about $0$, or in other words $S^{\tau_j}[s_j, q_j)$ and $-S^{\tau_j}[s_j, q_j)$ have the same distribution, because
%the underlying RV $X$ at each step is symmetric about $0$.

%[JFM] Recall that the performance of (standard or multi-probe) LSH relies on the distribution of 

\begin{comment}
Now we are ready to derive the pdf of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$.

 which we already know is the sum of $m$ independent range-sums $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality), so it is important that each $S^{\tau}[q, s)$ is the range-sum of a \emph{strict} random walk. Under this condition,  $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$  is a strict random walk of $d_1$ i.i.d. steps, which is  parameterized only by  $d_1$.
When $d_1$ is not small, the distribution of a $d_1$-step random walk can be very closely approximated as the Gaussian distribution $\mathcal{N}(0, d_1)$.
It has been shown in~\cite{mprwlsh} that this Gaussian distribution alone makes MP-RW-LSH highly efficient (w.r.t. query time) and
effective (w.r.t. query accuracy).


%It is not hard to show that , is a  this $d_1$-step random walk.  Therefore,  , which is JFM] Since  if the random walks are strict, and in general relies onthe distribution of each range-sum .[], $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$ is a deterministic function of $d_1$


[duplicated] When $d_1$ is not small, the distribution of $d_1$-step random walk can be very closely approximated as the Gaussian distribution $\mathcal{N}(0, d_1)$.
It has been shown in~\cite{mprwlsh} that this Gaussian distribution alone that makes MP-RW-LSH highly efficient (w.r.t. query time) and
effective (w.r.t. query accuracy).
It is not hard to show that $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$, the marginal 
(collision) probability for $\vec{\mathbf{s}}$ to have the same LSH value (by the LSH function $g()$) as the query point $\vec{\mathbf{q}}$, is a (deterministic) linear functional of the pdf of this $d_1$-step random walk.  Therefore, the performance guarantee of LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality), which is a deterministic function of $d_1$ (parameterized by $W$ used  {\color{red}in $g(\vec{\mathbf{s}})$ }) if the random walks are strict.
\end{comment}

%(the total number of $f(\cdot)$ functions)as large as hundreds to

Recall that 
In the MP-RW-LSH scheme, given a query point $\vec{\mathbf{q}}= \langle q_1, q_2, \cdots, q_m \rangle$, we need to compute the raw hash value $f(\vec{\mathbf{q}}) 
= \sum_{j=1}^m S^{\tau_j}[0, q_j)$
for $L M$ ($L$ hash tables each using a vector 
of $M$ hash functions) such ($f$)'s.
Computing these range-sums one (random walk) step at a time is a relatively computationally heavy task, since
%is to compute, given a query point $\vec{\mathbf{q}}= \langle q_1, q_2, \cdots, q_m \rangle$,
%$L M$ ($L$ hash tables each using a vector 
%of $M$ hash functions) such raw hash values of $\vec{\mathbf{q}}$.  
although each step takes only nanoseconds to compute, there
are simply too many of them:
There are a total of $O(LMmU)$ steps, where $LM$  is typically in hundreds, 
the data dimension $m$ can be in thousands, and the maximum possible number of steps $U$ to walk along 
each random walk sequence $\tau$ can be hundreds of thousands.   As a result, it is not uncommon for $LMmU$ to be on the
order of $10^{10}$ or $10^{11}$.  \textbf{For example, on the Enron dataset~\cite{enron}, the respective values are $LMmU = 9 \times 9 \times 1369 \times \SI{505}{K} = 5.60\times 10^{10}$. }
This translates into tens of seconds of or minutes of computation time just for the raw hash values
of $\vec{\mathbf{q}}$.  In contrast, the rest of the ANNS query can often be done in tens of milliseconds.  
To reduce the time of computing these range-sums, RW-LSH precomputes and stores all $S^{\tau_j}[0, q_j)$ values for $q_j = 0, 1, 2,\cdots, U$ and for each random walk 
sequence $\tau_j$.  This reduces the time complexity to $O(LMm)$ but bloats the total size of precomputation tables to $O(LMmU)$, which can translate into 
tens of gigabytes of storage as will be shown in~\autoref{sec:eva}.
%The ERS solutions that we will describe soon achieve the better of both worlds: It does not need precomputed tables, and the complexities in both space and evaluation time are as low as $O(LMm\log U)$.
% for each range-sum $S^{\tau}[0, q)$ achieves
\begin{comment}
To reduce the time of evaluating $f(\mathbf{s})$, the baseline solution of RW-LSH precomputes and stores each  $S^{\tau_j}[0, s_j)$ for $t = 2, 4, 6, \cdots, U_j$ where $U_j$ is the maximum possible (even) 
value for the $j^{th}$ coordinate of a data point.  For any random walk $\tau_j$, the baseline RW-LSH needs $U_j$ bytes for storing the precomputed table. Although
the storage cost of each precomputed table, which is roughly $O(mMU)$, supposing $U$ is the maximum value among $U_j$, is small relative to the size of each hash table, which is $O(n_d)$ and  $n_d$ is the size of the dataset, for large datasets, this cost can increase the total index size by several hundred times, for some smaller datasets where both $m$ and $U_j$ are very large (relative to the dataset size), 
as we will show in~\autoref{sec:eva}. 
\end{comment}

%We will explain shortly why this assumption is not 
%overly restrictive for real-world applications. 




%To reduce the storage cost of precomputed tables, the authors of \cite{mprwlsh} proposes ``long jump'', which reduces the storage cost by $32l$ times by paying $l$ CPU instructions for evaluating each range-sum $S^{\tau_j}[0, t)$. Even with this solution, the product of space and time complexities of RW-LSH is still $O(U_j)$ for each random walk, which is not scalable for future databases where $U_j$ might be gigantic.

%efficient range-summable (ERS) algorithms  to save the space of the precompute table
% ERS solutions, which only takes a small space and poly-logarithmic time. We can indeed use dyadic simulation to implement RW-LSH by generating range-summable single-step random walks , but %generate , but a better solution is to generate Gaussian random variables instead, because the latter can be  since it does not require rejection sampling. In BM-LSH, by changing the distribution of each step from a single-step random walk to a standard Gaussian random variable, we reformulate the random walk in RW-LSH to a discrete time Brownian motion. This reformulation is justified because a random walk is statistically close to a Brownian motion when $n$ (the number of steps) is large.
 

 %Since the evaluation of RW-LSH resolves to the ERS problem, 
 %Readers may wonder if
%{\bf no BCH3 anymore} 



We have considered whether EH3~\cite{feigenbaum}, an ERS scheme for single-step random walks, can be used to generate these range-sums for RW-LSH.  
The answer is ``no'' for the following reason.
  %One possible option is  which is shown by~\cite{rusu-jour} as the fastest range-summable scheme that has both theoretical guarantee (approximate $4$-wise independence) and good empirical performance (when estimating the size of joins). However, we show that EH3 is not very suitable for ANNS-$L_1$, for the following reasons.or BCH3~\cite{rusu-jour}
%   Recall that the efficacy of RW-LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ to be of a strict random walk.
  Although every underlying RV generated by EH3 has the  %EH3 scheme in \etal{Feigenbaum}~\cite{feigenbaum} generates range-summable random variables whosebe used to and BCH3of   matches that of
  marginal distribution of a single-step random walk, these %is highly ordered (deterministic)  (as required they only preserves the three-wise independence among  andir generated random variables
RVs are strongly correlated, since as explained earlier EH3 achieves ERS by systematically destroying all independence beyond $4$-wise among the underlying RVs.  
Hence the resulting range-sum $S^\tau[q, s)$ (where $\tau$ is generated by EH3)
%guaranteed to have the same standard deviation as those from an authentic 
%random walk, they may structure when more than three consecutive random variables are concerned. generated are  Thereforefollow a very different distribution than that of
behave very differently from a $(s - q)$-step random walk. %For example, when $[q, s)$ is a dyadic interval of width $2^l$ 
%{\bf JFM: I think $l$ is best. (DO WE WANT TO USE l here?)}, %the range-sum $S^\tau[q, s)$ generated by BCH3 is equal to $0$ with probability $1-2^{-l}$, 
%and has absolute value $2^l$ with probability $2^{-l}$~\cite{rusu-jour}.
%This distortion seriously impacts the distribution of $f(\mathbf{s})  - f(\mathbf{q})$ and the accuracy of RW-LSH.
%EH3 has a slightly better distribution of range-sums than BCH3 that is no longer 0 with high probability, but that is still far from that of a strict random walk.
%Although EH3 has a slightly stronger guarantee than BCH3 of approximate four-wise independence, so it has theoretical guarantees in the accuracy of estimating the $L_2$ moment in data streams in its proposed application, but it suffers from the same problem as above. %the generated range-sums still follow a very different distribution from
% is, its detailed distribution may be very different from the latter.$S^{\tau}[0, 10^6)$ 
For example, when $[q, s)$ is a dyadic range and  $s - q = 4^l$, the range-sum $S^\tau[q, s)$ 
%generated by EH3 
takes values $2^l$ and $-2^l$ each with probability 1/2.
%follows uniform distribution in $\{2^l, -2^l\}$~\cite{rusu-jour}, so its absolute value is always $2^l$! 
\textbf{For other less extreme values of $q$ and $s$, the distribution of $S^\tau[q, s)$ is still very different from a strict random walk, as shown in~\autoref{sec:kstest}}.


\begin{comment}\subsection{Why EH3 Cannot Solve This Problem}
\autoref{fig:distcomp} shows another example in which $[a, b)$ is  $[0, 10^6)$, which is not a dyadic interval. The histogram at the top is plotted from one million range-sums $S^{\tau}[0, 10^6)$ generated from EH3 with different seeds, and that at the bottom is from %one million range-sums of the same range from , which
a ``real'' random walk with empirically independent steps is generated by the built-in \texttt{mt19937} PRNG (not range-summable) in C++.%, and plot its distribution histogram at the top of \autoref{fig:distcomp}. at the bottom
%plot the histogram of the range-sum  generated from EH3 with one million different seeds  from  (not range-summable) 
%As a reference, we also plot the histogram of $S^{\tau}[0, 10^6)$ in 
 \begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{figures/histogram.eps}
	\caption{Distribution of generated random walks (Y axis normalized to probability density).}\label{fig:distcomp}
\end{figure}
From \autoref{fig:distcomp}, the distribution of range-sums generated by EH3 is far from that of the ``real'' random walk below, but concentrates at some special points near $1000$ (its standard deviation) and $-1000$. 

%In contrast, the distribution of the range-sums generated by dyadic simulation % and of the independent non-range-summable random walk are distributed
%is close to the reference Gaussian distribution. This shows dyadic simulation is more suitable to ANN applications where the distribution of range-sums is crucial to the performance.
%In an even more extreme example, 
%Therefore, the performance of applying EH3 to MP-RW-LSH leads to unstable performance and significant degradation for some special queries on which the distribution of the produced range-sums is far from that of random walks. This will be illustrated by simulations in \autoref{sec:feigen_sim}.

 %preserves the independence between %different steps of the Brownian motion with the use of $O(\log U)$ two-wise independent hash functions (to be explained in ??) %if a two-wise independent hash function is used on each level of the simulation tree (to be explained later), 
%, so it is better suited for this application. of this distribution onof the distribution of range-sums , corresponding to recalls changes with $d_1$


%It has been shown in~\cite{stablelsh} that the performance guarantee of standard 
A key metric for measuring the quality of any LSH function family is $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$, the 
(collision) probability for $\vec{\mathbf{s}}$ to have the same LSH value (by the LSH function $g(\cdot)$) as the query point $\vec{\mathbf{q}}$.
%(so that $\vec{\mathbf{s}}$ can be found by the ANNS query in case it is a nearest neighbor of $\vec{\mathbf{q}}$).
In RW-LSH, this probability is a (deterministic) linear functional of the pdf of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}}) = \sum_{j=1}^mS^{\tau_j}[q_j, s_j)$.
%It as shown in~\cite{} that this pdf leads to virtually every nice property of RW-LSH.
% can be derived from the pdf of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$.
%(parameterized by $W$ {\color{red} used in $g(\vec{\mathbf{s}})$}). For a similar reason, the performance guarantee of multi-probe LSH also relies on the distribution of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$~\cite{mprwlsh}.
We now study how the use of EH3 for generating the sequences $\tau_j$, $j = 1,2, \cdots, m$, impacts 
%the damaging effect of this strong correlation among the random walk steps on 
the collision probability $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$ by distorting the range sums $S^{\tau_j}[q_j, s_j)$, $j=1,2, \cdots, m$.
We do so by zooming in on its damaging effect on a single sequence $\tau_1$ as follows:
%To isolate the effect of a single EH3-generated random walk sequence on the corresponding range sum, 
%$S^\tau[q, s)$ affects the collision probability, we now place further restrictions on these two points while keeping them $d_1$ apart in $L_1$ distance.
We let $\vec{\mathbf{q}} = \vec{\mathbf{s}}$ in every coordinate except the first, where $s_1 = 0$ and $q_1 = D$, so that $d_1 =  \sum_{j=1}^m |s_j-q_j| = D$.  
This way the value $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}}) = S^{\tau_1}[0, s_1)$, and hence the collision probability, is affected by only $\tau_1$.
%When the single-step random walks in the sequence $\tau_1$ is  independent,
%$f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}}) $ is a strict random walk with $d$ steps.  

In \autoref{fig:coll_prob}, we compare this collision probability ($y$-axis), which is a function of $D$ ($x$-axis), in two cases:  (1) \emph{original},
when $\tau_1$ is a strict random walk;  (2) \emph{EH3-augmented}, when $\tau_1$ is generated by EH3.
In case (1), this probability is monotonically decreasing as $D$ increases.
This monotonicity property has been widely used as a litmus test for an ``aspiring'' LSH function family~\cite{Indyk_ANN_1998}.
%qualifying requirement 
% for a (hash) function family to become a legitimate LSH function family [?] {\bf talk with Huayi}.
In contrast, in case (2), the collision probability jumps up and down when $D$ becomes larger.
%The obvious oscillation of the blue line in \autoref{fig:coll_prob} shows that the distortion of the distribution %of range-sums by EH3 shown in \autoref{fig:distcomp} against the ideal case with independent steps. 
%This phenomenon is extreme
This behavior automatically disqualifies the ``EH3-augmented'' RW-LSH, as an LSH function family.  
Furthermore, when the distance $D$ is chosen so that the collision probability (curve) falls into a ``valley'' (e.g., between \SI{16000}{} and \SI{17000}{}), 
%the collision probability becomes close to 0.
%As a result, 
the (success) probability for $\vec{\mathbf{q}}$ to be hashed into the epicenter bucket and be found by the ANNS query becomes very close to 0.
In this case, the query accuracy can be very low, 
%It can be shown that this probability remains low 
even when multi-probe is used, as we will show next to some extent.  
%has a significant influence on the collision probability  against ideal RW-LSH, especially in the ``valleys'' in which it is impossible to find the data point in the epicenter bucket! 
%(The first two valleys occur at distance $16384$ and $49152$.) 
%As a result, it is difficult to guarantee robust performance when EH3 is used to implement RW-LSH.  

% happens to cause the

\begin{comment}
[added]
To further verify 
We have evaluated the ANNS-$L_1$ query accuracy of MP-RW-LSH using EH3 on the Enron dataset (see ???), when the distance of the nearest neighbor to a query point
We have found that its recall value is an order of and that of MP-RW-LSH using precomputed tables.
show 
%tune the parameter for the ANNS with EH3
%which may lead to significant performance degradation in some bad cases. 


%[maybe still useful]
%When the single-step random walks in the sequence $\tau_1$ is mutually indepdent,
%$f(...) - f(...)$ is an authentic random walk with $d$ steps.  


[duplicate]
When the single-step random walks in the sequence $\tau_1$ is mutually indepdent,
$f(...) - f(...)$ is an authentic random walk with $d$ steps.  






[duplicate]
it is the sum of $m$ independent range-sums, and the range-sum on the $j^{th}$ coordinate is a $|q_j - s_j|$-step random walk. Therefore, the performance guarantee of LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality).

[mostly spent]
hashed by a single LSH function $g$.  
in the following (overly simple) simulation, we set the LSH bucket width $W=122$ (same as the simulation below) and regard the range-sum $S^\tau[0, d)$ as the difference of the raw hash values $f(\mathbf{s}) - f(\mathbf{q})$, corresponding to the case where %$m=1$, $\mathbf{s}=\langle 0\rangle$, and $\mathbf{q}=\langle d\rangle$. 
$\mathbf{s}$ and $\mathbf{q}$ differ only at the $j^{th}$ coordinate, with $s_j=0$ and $q_j=d$. We plot the frequency of hash collisions (\ie $g(\mathbf{s}) = g(\mathbf{q})$) in one million runs for each $d$ on a wide range in \autoref{fig:coll_prob}, against ideal RW-LSH. %(directly computed from the property that $f(\mat

[duplicate]In this section, we show why existing range-summable generation schemes, such as EH3~\cite{feigenbaum}, is not suitable for ANNS.  In particular, we show by simulation that the dependency between the components of the EH3 scheme interferes the distribution of the difference of raw hash values $f(\mathbf{s})  - f(\mathbf{q})$, making it far from Gaussian.

% samplesThe distribution of the final position shold$To compare the distribution of range-sums, we generate $1$ million range-sums of 1 million standard gaussian random variables from existing range-summable sketches for $L_1$ \cite{feigenbaum} and dyadic simulation and plot the histograms as \autoref{fig:distcomp} against the distribution of one-million step random walks and reference Gaussian $\mathcal{N}(0, 10^6)$. Ideally, the range-sums should follow Gaussian distribution with mean $0$ and standard deviation $1000$ (bottom figure). 



%[maybe still useful]
%it is the sum of $m$ independent range-sums, and the range-sum on the $j^{th}$ coordinate is a $|q_j - s_j|$-step random walk. Therefore, the performance guarantee of LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality).

%[mostly spent]
%hashed by a single LSH function $g$.  
%in the following (overly simple) simulation, we set the LSH bucket width $W=122$ (same as the simulation below) and regard the range-sum $S^\tau[0, d)$ as the difference of the raw hash values $f(\mathbf{s}) - f(\mathbf{q})$, corresponding to the case where %$m=1$, $\mathbf{s}=\langle 0\rangle$, and $\mathbf{q}=\langle d\rangle$. 
%$\mathbf{s}$ and $\mathbf{q}$ differ only at the $j^{th}$ coordinate, with $s_j=0$ and $q_j=d$. We plot the frequency of hash collisions (\ie $g(\mathbf{s}) = g(\mathbf{q})$) in one million runs for each $d$ on a wide range in \autoref{fig:coll_prob}, against ideal RW-LSH. %(directly computed from the property that $f(\mathbf{s}) - f(\mathbf{q})$ is $\mathcal{N}(0, d)$, the approximation of a $d$-step random walk).
%especially the collision probability (of having the same hash value) of RW-LSH. We draw   with a varying number of steps generated by EH3 similarly to the simulation above. % The following simulation provides a more intuitive view on how the distribution of the random walk (of the difference of raw hash values) influence the performance of ANNS. 
%In this   %fix the query point at $0$, and increase the first coordinate of the nearest neighbor while fixing the other coordinates at $0$.  (equivalent to the case when data and query points are one-dimensional, the query points is $0$, and the data point $d$ is moving).
%\autoref{fig:coll_prob} shows the  of EH3 against 
%

\begin{figure}[!ht]
	\centering
	\caption{Comparison of collision probabilities, $W=122$.}\label{fig:coll_prob}
	\includegraphics[width=0.51\textwidth]{figures/collprob.eps}
\end{figure}

% Figure.\, \ref{fig:coll_prob} gives an example in which the dependence of ETH3 significantly affect the collision probability (of finding a nearest neighbor in the same bucket). %Therefore, the generated sequence is not a real random walk, so $f(\mathbf{s}) - f(\mathbf{t})$ will not always converge to Gaussian distribution as required by the LSH function and is very sensitive to input. 
%We will show in ??? that the range-summable ``random-walk'' scheme by~\cite{feigenbaum} is not suitable for ANNS-$L_1$.


%\textbf{The probability of $|g(\mathbf{s}) - g(\mathbf{q})|=1$ also oscillates in a similar manner, so the probability of finding $\mathbf{s}$ even with multi-probe used is not stable. Note that the numbers in \autoref{fig:coll_prob} do not directly explain the next experiment, because the collision probability depends on the nearest neighbor $\mathbf{s}$, which is no longer $\langle 0\rangle$ in real datasets. }

%In comparison, dyadic simulation can generate range-summable random variables that are nearly perfectly independent, so it is better suited for the ANNS-$L_1$ application. We can indeed use dyadic simulation to generate empirically independent range-summable single-step random walks as in \autoref{sec:randw}, but a better solution is to generate Gaussian random variables instead, because the latter can be generated four times as fast as random walks since it does not require rejection sampling. In BM-LSH, by changing the distribution of each step from a single-step random walk to a standard Gaussian random variable, we reformulate the random walk in RW-LSH to a discrete time Brownian motion. This reformulation is justified because a random walk is statistically close to a Brownian motion when $n$ (the number of steps) is large.

%Since the range-sum of  we may use (rounded) Gaussian distribution approximation in rejection sampling. However, we think it might be better to just take the easy step: to use the range-summable scheme for Gaussian distribution in this application. For this purpose
%We reformulate RW-LSH to a closely related stochastic process, a discrete time Brownian motion. 







\begin{comment}
\textcolor{teal}{
How to efficiently search for similarity on large (large element number, high dimension) databases? 
(definition of c-ANN)
We focus on $l_1$ distance, because it is important (robust to outliers) and underexplored.
A thread of high performance ANN by Locality Sensitive Hashing (LSH) indices. For similar pairs of (data and query) points that are closer under $l_1$ metric (than a certain threshold), the LSH function maps them to the same bucket with higher probability. But for dissimilar pairs of points, this LSH function maps them to the same bucket with very low probability.(definition of LSH)
% One basic LSH is constructed with stable distribution, which is generic for $l_p$ distance with $1\leq p\leq 2$. 
In addition to the ``hard decoding" schemes that works only when the data and query are in the same bucket, researchers have put forward ``soft decoding" schemes, such as SRS and multiprobe \cite{multiprobe}, which also search nearby buckets for data candidates. These schemes achieve higher memory efficiency, but they require the distribution of the difference of hash values $f(\mathbf{x})-f(\mathbf{q})$ to be concentrated so that near neighbors will always be hashed close to the query.  However, the only? $l_1$ LSH function $f$ till now is based on stable distributions \cite{stablelsh}, under which the distribution of $f(\mathbf{x})-f(\mathbf{q})$ follows the corresponding stable distribution for $l_p$ norm with $1\leq p\leq 2$. Although Gaussian distribution (stable for $l_2$) is nicely concentrated, Cauchy distribution (stable for $l_1$) has a heavy tail. As a result, a large proportion of data points may be hashed far away from the query point under the Cauchy scheme, which is why multiprobing performs well on $l_2$ but is less effective on $l_1$. 
}
 
% \subsection{Comparison with EH3 Scheme}\label{sec:feigen_sim}
 %However, no existing range-summable scheme maintains the distribution of the range-sum as perfect Gaussian as required by the LSH propery (and multiprobing). 
%[duplicate]In this section, we show why existing range-summable generation schemes, such as EH3~\cite{feigenbaum}, is not suitable for ANNS.  In particular, we show by simulation that the dependency between the components of the EH3 scheme interferes the distribution of the difference of raw hash values $f(\mathbf{s})  - f(\mathbf{q})$, making it far from Gaussian.
 
%[duplicate]At first, we compare the distribution of generated range-sums from simulation. In each run of the simulation, we generate the final position of a random walk or a Brownian motion with the following three schemes. \textbf{Sequence of schemes?} The first one is dyadic simulation for standard Gaussian target distribution, which generates the final position of a Brownian motion $S^{\zeta}[0, 10^6)$. The second scheme is EH3, which generates the final position of a ``random walk'' $S^{\tau}[0, 10^6)$ with the same number of steps. The third scheme is a ``real'' random walk $S^{\tau}[0, 10^6)$ from empirically independently steps (not range-summable) generated by the built-in \texttt{mt19937} PRNG in C++. %The third scheme is to use range-summable  to generate a random walk for the same $\tau(t)$ at $t=10^6$. 
%For all three schemes above, we draw the histogram (normalized to probability density) from one million independent runs and show at the bottom of \autoref{fig:distcomp} the reference Gaussian distribution $\mathcal{N}(0, 10^6)$ , %draw the histogram for the distribution of the final position, 
%to which all of the top three figures should converge. %is the distribution should all converge to with mean $0$ and standard deviation $1000$ (bottom figure). 

% samplesThe distribution of the final position shold$To compare the distribution of range-sums, we generate $1$ million range-sums of 1 million standard gaussian random variables from existing range-summable sketches for $L_1$ \cite{feigenbaum} and dyadic simulation and plot the histograms as \autoref{fig:distcomp} against the distribution of one-million step random walks and reference Gaussian $\mathcal{N}(0, 10^6)$. Ideally, the range-sums should follow Gaussian distribution with mean $0$ and standard deviation $1000$ (bottom figure). 
 

 
%[duplicate] From \autoref{fig:distcomp}, the distribution of range-sums generated by EH3 is far from that of the ``real'' random walk, but concentrates at some special points near $\pm1000$ (in order to have $0$ mean and $1000$ standard deviation). In contrast, the distribution of the range-sums generated by dyadic simulation % and of the independent non-range-summable random walk are distributed
%is close to the reference Gaussian distribution. This shows dyadic simulation is more suitable to ANN applications where the distribution of range-sums is crucial to the performance.
% \textcolor{teal}{However, no existing range-summable scheme maintains the distribution of the range-sum as perfect Gaussian as required by the LSH propery (and multiprobing). For example, the scheme in \cite{feigenbaum} can only guarantee approximate four-wise independence, which sacrifices all higher orders of independence in return for range-summability, and although \cite{rusu-jour} described several range-summable schemes with a higher degree of independence, the time complexity of these schemes is too high. }%Four-wise independence is sufficient for bounding the variance of the estimator in the streaming application, but for ANN, 
%To intuitively show  the impact of this distribution on the performance of ANNS, especially the collision probability (of having the same hash value) of RW-LSH. We draw \autoref{fig:coll_prob}  with a varying number of steps generated by EH3 similarly to the simulation above. % The following simulation provides a more intuitive view on how the distribution of the random walk (of the difference of raw hash values) influence the performance of ANNS. 
%In this (overly simple) simulation, we set the LSH bucket width $W=100$ and regard the range-sum $S^\tau[0, d)$ as the difference of the raw hash values $f(s) - f(q)$, corresponding to the case where $m=1$ and $s=\langle 0\rangle$. %fix the query point at $0$, and increase the first coordinate of the nearest neighbor while fixing the other coordinates at $0$.  (equivalent to the case when data and query points are one-dimensional, the query points is $0$, and the data point $d$ is moving).
%\autoref{fig:coll_prob} shows the ratio of hash collisions in one million runs for each $d$ of EH3 against ideal RW-LSH (directly computed from the property that $f(s) - f(q)$ is $\mathcal{N}(0, d)$, the approximation of a $d$-step random walk).
 %\begin{figure}
 %	\centering
 %	\includegraphics[width=0.48\textwidth]{figures/coll_prob_100.png}
 %	\caption{Comparison of collision probabilities.}\label{fig:coll_prob}
 %\end{figure}
% Figure.\, \ref{fig:coll_prob} gives an example in which the dependence of ETH3 significantly affect the collision probability (of finding a nearest neighbor in the same bucket). %Therefore, the generated sequence is not a real random walk, so $f(\mathbf{s}) - f(\mathbf{t})$ will not always converge to Gaussian distribution as required by the LSH function and is very sensitive to input. 
 %We will show in ??? that the range-summable ``random-walk'' scheme by~\cite{feigenbaum} is not suitable for ANNS-$L_1$.
%The obvious oscillation of the blue line in \autoref{fig:coll_prob} shows that the distortion of the distribution of range-sums by EH3 shown in \autoref{fig:distcomp} has a significant influence on the collision probability  of RW-LSH against the ideal case with independent steps. This phenomenon is extreme in the ``valleys'' in which it is impossible to find the data point in the epicenter bucket! (The first two valleys occur at distance $16384$ and $49152$.) As a result, it is difficult to guarantee consistent performance when EH3 is used to implement RW-LSH, %tune the parameter for the ANNS with EH3
%which may lead to significant performance degradation in some bad cases.
%\subsection{Comparison between Feigenbaum and Dyadic}
% \begin{table}[!htb]
% 	\caption{Comparison between MP-BM-LSH and MP-RW-LSH(EH3) on synthetic dataset. $M=7$, $W=100$}\label{tab:feigen_vs_dyadic}
% 	\centering
% 	\begin{tabular} {@{}c c c c c@{}}
% 		\specialrule{.1em}{.05em}{.05em} 
% 	\multirow{2}{*}{$L$} & \multicolumn{2}{c}{MP-BM-LSH}  & \multicolumn{2}{c}{MP-RW-LSH (EH3)} \\\cline{2-5}
% 	& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
% 	6  & 0.0820 & 1.0878 & 0.0065 & 0.9088\\
% 	10 & 0.1287 & 1.7429 & 0.0129 & 1.4614  \\
% 	20 & 0.2402 & 3.3721 & 0.0228 & 2.8278  \\
% 	40 & 0.4201 & 6.7092 & 0.0442 & 5.5682\\
% 		\specialrule{.1em}{.05em}{.05em} 
% 	\end{tabular}
% \end{table} 
\begin{comment}
\begin{table}[!htb]
	\caption{Comparison between MP-BM-LSH and MP-RW-LSH(EH3) on synthetic dataset. $M=7$, $W=100$}\label{tab:feigen_vs_dyadic}
	\centering
	\begin{tabular} {@{}c c c c c@{}}
		\specialrule{.1em}{.05em}{.05em} 
		\multirow{2}{*}{$L$} & \multicolumn{2}{c}{MP-BM-LSH}  & \multicolumn{2}{c}{MP-RW-LSH (EH3)} \\\cline{2-5}
		& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
		6  & 0.0820 & 1.03+0.06 & 0.0065 & 0.85+0.06\\
		10 & 0.1287 & 1.65+0.10 & 0.0129 & 1.37+0.10  \\
		20 & 0.2402 & 3.17+0.20 & 0.0228 & 2.64+0.19  \\
		40 & 0.4201 & 6.26+0.45 & 0.0442 & 5.18+0.40\\
		\specialrule{.1em}{.05em}{.05em} 
	\end{tabular}MP-RW-LSH (precomputed) and MP-RW-LSH (EH3) on synthetic Enron dataseComparison between two different MP-RW-LSH
\end{table}
\begin{table}[!htb]
\caption{Original vs EH3-augmented. }\label{tab:feigen_vs_dyadic_another}
\centering
%\begin{tabular} {@{}c c c c c@{}}
%\specialrule{.1em}{.05em}{.05em} 
%\multirow{2}{*}{$L$} & \multicolumn{2}{c}{Precomputed}  & \multicolumn{2}{c}{EH3} \\\cline{2-5}
%& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
%10 & 0.1111 & 2.64+2.42 & 0.0100 & 0.64+1.12  \\
%15 & 0.1647	& 4.09+4.98 & 0.0147 & 1.05+1.64 \\
%20 & 0.2080	& 4.70+8.21 & 0.0180 & 1.25+2.16  \\
%\specialrule{.1em}{.05em}{.05em} 
%\end{tabular}
\begin{tabular} {@{}c | c c c c@{}}
	\specialrule{.1em}{.05em}{.05em} 
	 \multicolumn{2}{c} {$L$ } & 10 & 15 & 20 \\
	\specialrule{.1em}{.05em}{.05em} 
	  \multirow{2}{*}{Recall} &original & 0.1111 & 0.1647 & 0.2080\\\cline{2-5}
 &EH3-augmented& 0.0100& 0.0147 & 0.0180	\\
	\specialrule{.1em}{.05em}{.05em} 
\end{tabular}
\end{table}  
% \begin{table}[!htb]
% 	\caption{Comparison results on Enron dataset with synthetic queries. }\label{tab:feigen_vs_dyadic_another}
% 	\centering
% 	\begin{tabular} {@{}c c c c c@{}}
% 		\specialrule{.1em}{.05em}{.05em} 
% 		\multirow{2}{*}{$d$ } & \multicolumn{2}{c}{Precomputed}  & \multicolumn{2}{c}{EH3} \\\cline{2-5}
% 		& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
% 		6400  & 0.5880 & 10.58+2.77 & 0.4321 & 6.41+1.01 \\
% 		8400 & 0.1709 & 6.68+2.35 & 0.1109 & 3.25+1.01  \\
% 		13300 & 0.0208	& 2.44+2.14 & 0.0019 & 0.65+1.01  \\
% 		16600 & 0.0084	& 1.33+2.10 & 0.0001 & 0.20+1.02 \\
% 		\specialrule{.1em}{.05em}{.05em} 
% 	\end{tabular}
% \end{table} 
% in the worst casethe Audio dataset (to define in \autoref{subsec:exp_set}). Each query is generated by conduct the following experiment in in the worst cases
%$M=9$, $W=122$between MP-GRW-LSH and MP-RW-LSH(EH3)

\begin{comment}
Description for varying distance: To show how the performance of EH3-based MP-RW-LSH degrades, we compare it  with the vanilla MP-RW-LSH with precomputed tables~\cite{mprwlsh}. %on the  dataset . 
In the experiments, we use Enron (see \autoref{tab:dataset-stats}) as the dataset $\mathcal{D}$, and generate \SI{10000} synthetic queries from the following procedure for each $d$. First, we randomly sample one point from the Enron database. Then, we generate the query point from randomly choosing one coordinate of the sampled data point and adding $d$ while keeping other coordinates unchanged, similar to the restriction above. %which is a variable parameter reflecting how far the query is from its neareat neighborroughly the position of the first ``valley'' in \autoref{fig:coll_prob}, to this coordinate value. MP-BM-LSH (from dyadic simulation) and MP-RW-LSH (from EH3) with different number of hash tables 
For different distance value $d$, the recalls and query times of both algorithms reported in~\autoref{tab:feigen_vs_dyadic} are averaged for these \SI{10000} queries.
We use the same index structure (hash tables) as in \autoref{sec:eva}, with the same set of parameters $M=9$, $T=100$, $W=122$. We show how recall and query time (written as $t_1+t_2$) change when  $d$ increases.
%As an example of the worst case, we generate the distance between the data and query points areplease refer to \autoref{subsec:ann-comp-algorithmsfor the meaning of these parameters)



%\textbf{Huayi Paragraph for the generation of synthetic dataset: \autoref{fig:distcomp} clearly shows that the success probability of EH3-based LSH is close to 0 for distance equal to 17600 when hash bucket width $W=100$. Based on this fact, we generate synthetic dataset where the distance of each query point to its corresponding nearest neighbor is 17600. More precisely, we first randomly sample one point from database. Then we generate the query point from randomly choosing one coordinate of the sampling point and adding 17600 on the coordinate value of this point. We use such generation process in order to achieve the similar success probability value as shown in \autoref{fig:distcomp}. We generate 1000 different query points and report the query performance of Feigenbaum and Dyadic on the synthetic dataset with different number of hash tables in~\autoref{tab:feigen_vs_dyadic}.}$M=9$, $W=122$index structure (hash tables) , with the same, which is roughly the position of the first ``valley'' in \autoref{fig:coll_prob},
We illustrate this ``fall into the valley'' effect by performing the following controlled ANNS-query experiment involving both 
the original and the  EH3-augmented MP-RW-LSH.  
%To show how the performances of EH3-based MP-RW-LSH (EH3-based for short in the sequel) degrades, we compare it  with the original MP-RW-LSH with precomputed tables~\cite{mprwlsh} (Precomputed for short).
In this experiment, we use Enron (see \autoref{tab:dataset-stats}) as the dataset $\mathcal{D}$ and generate \SI{10000}{} synthetic queries that target a 
``statistical fall'' distance
$D$ = \SI{13300}{}.  This $D$ is not in the middle of the first ``valley'' (between \SI{16000}{} and \SI{17000}{}) shown in~\autoref{fig:coll_prob} (for the $s_j = 0$ case)
for the following reason.
Even when $D$ is fixed, the value of an EH3-generated range-sum 
$S^{\tau_j}[s_j, s_j + D]$, and hence the shape of the corresponding collision probability curve, varies when $s_j$ varies (as 
it does in this experiment), so this $D$ optimizes, to some extent, the probability of ``fall'' over the set of $s_j$ values that are actually encountered.
% this $D$ is not in the middle the first ``valley'' shown \autoref{fig:coll_prob}).  
Each query is generated as follows.  First, we randomly sample a point $\vec{\mathbf{s}}$ from $\mathcal{D}$.  Then, we pick a dimension $j$ uniformly at
random (out of the $m$ dimensions), and set the query point $\vec{\mathbf{q}}$ such that $\vec{\mathbf{q}}$ is identical to $\vec{\mathbf{s}}$ in every dimension except the $j^{th}$, where $q_j = s_j + D$.
%Note that despite our ``statistically targeted push'', 
%only a small percentage of query points actually ``fall into the valley'', 
%and hence we are not overly ``exaggerating'' EH3's damaging effect here.
%generate the query point from randomly choosing one coordinate of the sampled data point and adding \SI{13300}{} to this coordinate value while keeping other coordinates %unchanged, similar to the restriction above. 
For both the original and the EH3-augmented, we use the same set of parameters $M=9$, $T=100$, $W=122$ as in~\autoref{sec:eva}, and report their average 
recalls (over these \SI{10000}{} queries)
under the same set of $L$ (number of hash tables) values.
\autoref{tab:feigen_vs_dyadic_another} shows that recall values of the original are between $11.1$ and $11.6$ times larger than those of EH3-augmented. 
%Note that here the recalls are lower than those in~\autoref{sec:eva}, because $d$, the distance between the query point and its nearest neighbor is \SI{13300}{}, which corresponds with the ``valley'' in \autoref{fig:coll_prob}, are ??? times of those typical in ~\autoref{sec:eva}. Under such a large distance, the recalls of EH3-based is approximately equal to $0$ while Precomputed still have recalls around $0.1$. 
\begin{comment}
Therefore, the performance of EH3-based is not robust, even if its query times may be shorter than those of Precomputed.
{\bf JFM: I suggest removing ``query times'', because the story is distracting.}
For query efficiency, EH3-based has a shorter $t_1$ than Precomputed, because it hardly finds any candidate.  As we will shown later in \autoref{sec:eva}, we have found that $t_1$ is roughly linear to the number of candidates found in probing the buckets. Its $t_2$ is also shorter, because it is faster to compute a range-sum by EH3 in this case than to read from the precomputed table in DRAM.
\end{comment}

%\textbf{Original description:\autoref{tab:feigen_vs_dyadic_another} clearly shows that when $d=6400$, a typical distance for queries in the real dataset \autoref{sec:eva}, the recall of EH3-based is lower than that of vanilla MP-RW-LSH by 1.4. This difference becomes more pronounced when $d$ increases. For example, when $d=$\SI{13300}{}, vanilla MP-RW-LSH achieves recall $0.0208$, but recall value of EH3-based MP-RW-LSH is only $0.0019$, which is 10.9 times smaller than the recall value of vanilla MP-RW-LSH. This corresponds with the ``valley'' in \autoref{fig:coll_prob}, where success probability of EH3-based MP-RW-LSH is approximately equal to 0 where vanilla MP-RW-LSH still have success probability around 0.1. For query efficiency, EH3 has a shorter $t_1$ than vanilla, because it hardly finds any candidate. For example (\textbf{Huayi: As we will shown later in \autoref{sec:eva}}) we have found that $t_1$ is roughly linear to the number of candidates found in probing the buckets. Its $t_2$ is also shorter, because it is faster to compute a range-sum by EH3 in this case than to read from the precomputed table in DRAM.}

%\autoref{tab:feigen_vs_dyadic_another} clearly shows that, for the same number of hash tables, EH3 has a shorter $t_2$ than DST by a factor of $4.1$ to $4.9$, which is because its algorithm is simpler in using integer operations only and no transforms, and a shorter $t_1$ by a factor of $3.2$ to $4$, which is because it hardly finds any candidate. We have found that $t_1$ is roughly linear to the number of candidates found in probing the buckets. The $t_1$ of DST on the first row of  \autoref{tab:feigen_vs_dyadic_another} with that on the third column of \autoref{tab:perf} measured from normal queries, 

 %times that of EH3, the former can achieve much better accuracy ($9.1$ to $10.1$ times as high recall) than  the latter.
%$t_1$ is shorter for EH3, because it returns fewer candidates.
 
 %Under these schemes, the distribution of $f_{\mathbf{V}}(\mathbf{x})  - f_{\mathbf{V}}(\mathbf{q})$ is far from Gaussian, which directly degrades the performance. The GRW-LSH algorithm


\subsection{Our Clean Solution: MP-GRW-LSH}\label{sec:grwlsh}

%We can certainly solve 
Again we fix $\vec{\mathbf{s}}$ and $\vec{\mathbf{q}}$ that are $d_1$ apart in $L_1$ distance.
The ERS problem in RW-LSH can be solved using our RW-DST as follows.
Each DST instance (one for each random walk sequence) is generated using a different (cheap)  
$2$-wise independent hash function at each of the $\log_2 U$ levels.  This way, 
each range-sum $S^{\tau_j}[q_j, s_j)$, that is a part of $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}})$, is a strict $|s_j - q_j|$-step random walk according to \autoref{cor:stdist}, and hence $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}})$ is a
strict $d_1$-step random walk.   
Since the pdf of $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}})$ statistically defines an RW-LSH scheme, the RW-DST-augmented RW-LSH is statistically equivalent to the original RW-LSH.  

%However, as shown in Table~\ref{tab:perf}, splitting a random walk RV is relatively expensive operation.

\begin{comment}
to generate the underlying range sums.  
Since the behavior of RW-LSH is determined entirely by the pdf of 

 above, because by  \autoref{cor:stdist}, a hashing-based DST with cheap two-wise independent low-level hash functions guarantees that $S^\tau[q, s)$ follows the same distribution as a $|q - s|$-step strict random walk, which %is exactly what is needed by ANNS.
%In \autoref{sec:dsthash},  that a surprisingly cheap implementation of DST that uses  with two-wise independence 
%Therefore, by maintaining $m$ independent instances of such DSTs, one for each random walk $\tau$, we have an efficient DST-based implementation of RW-LSH that
%Therefore, we can evaluate $f(\mathbf{s})$ by generating the range-sum of each random walk $S^{\tau_j}[0, s_j)$ with the method described inn order to generate range-sums of single-step random walks that has the same distribution as ``real'' random walks,  and using . on the $j^{th}$ coordinate this DST uses t.I, which uses the definition of splits in \autoref{sec:randw} and l This leads to the following This implementation , because each of the range-sums $S^{\tau}[q, s)$ is a  random walk by.the DST-based GRW-LSH (defined below) is even better in thatand 
%does not need the precomputed tables and guarantees  the $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$ to be a strict$d_1$-step random walk, which 
is sufficient for all the theoretical efficacy guarantees of RW-LSH as we have shown above.
This is already a desirable solution, yet we will show that it is even better to replace RW-LSH with 
\end{comment}

We propose an even better solution called GRW-LSH (Gaussian random walk LSH).
% that is based on our ERS-Gaussian solution.
In GRW-LSH, a raw hash value function $f$ is defined in the same way as in RW-LSH, except each random walk sequence $\tau_j$ is replaced by 
a Gaussian random walk (GRW) sequence $\xi_j$.  In a GRW sequence, the underlying RVs are i.i.d. with standard Gaussian distribution instead.
%as just explained.  mutually independentin a $v$-step random walk
As a result, each $s_j$-step random walk along $\tau_j$ is replaced by an $s_j$-step GRW along $\xi_j$.
% and the other definitions, such as $g(\vec{\mathbf{s}})$, remain the same.
This way, $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$, which as just explained has the distribution of a $d_1$-step strict random walk %and has a probability distribution very close to the Gaussian distribution $N(0, d_1)$
under RW-LSH, now has Gaussian distribution $\mathcal{N}(0, d_1)$ under GRW-LSH.
Since the former distribution is always statistically close to the latter distribution and especially so when $d_1$ is reasonably large
(say when $d_1 > 25$), GRW-LSH  is statistically very close to RW-LSH.
As a result, its multi-probe extension MP-GRW-LSH has nearly the 
same query efficacy as MP-RW-LSH, as will be shown in \autoref{sec:eva}.  

It is straightforward to implement (the step of hashing $\vec{\mathbf{q}}$ in) GRW-LSH:   Each range-sum $S^{\xi_j} [0, q_j)$ is computed using our Gaussian-DST.
As explained above, using a different
$2$-wise independent hash function at every level of a DST instance is enough to ensure statistical equivalence (between the original GRW-LSH and
the Gaussian-DST-augmented GRW-LSH);  but for all practical purposes, we will use {\tt wyhash} functions instead.  
The Gaussian-DST-augmented GRW-LSH is a better solution than the RW-DST-augmented RW-LSH, since to compute a Gaussian range-sum is several times faster than to compute a random walk range-sum, as shown in \autoref{tab:perf}.

%Therefore, we focus on the DST-based efficient implementation of only GRW-LSH, which we simply refer to as GRW-LSH in the sequel, and we refer to the original scheme in~\cite{mprwlsh} with precomputed tables as RW-LSH. 

\begin{comment}

%replacing a $v$-step random walk (in RW-LSH) by a $v$-step(in GRW-LSH)ERS solution for 
The primary motivation for using Gaussian random walks  is that the it 
can be efficiently computed using our Gaussian-DSTs. 
Our measurements 
show that each dyadic split operation for Gaussian 
can be accomplished in a couple of nanoseconds.  Hence even when $v$ is as large as $2^{20}$, the $20$ dyadic splits involved to 
compute the $v$-step Gaussian random walk take a total of roughly \SI{95.1}{ns} to compute.  In comparison, in RW-LSH, even to read a precomputed value from the gigantic 
table (stored in DRAM) takes tens of nanoseconds.  Hence GRW-LSH usually affords faster LSH computation while paying zero storage cost for it.  
This said, we do not consider
GRW-LSH a separate contribution to the LSH literature, since it is conceptually very close to RW-LSH.  We consider it a contribution to the ERS literature as a novel application of 
our ERS-for-Gaussian solution.



%[to move with the closeness paragraph several paragraphs before]
%Since the latter is always statistically close to the former and especially so when $v$ is reasonably large
%(say when $v > 25$), the resulting GRW-LSH (... LSH) is statistically close to RW-LSH.  

We stress the difference between our GRW-LSH and the traditional GP(Gaussian projection)-LSH~\cite{Datar_LSH_2004}, which also uses Gaussian random variables, that GP-LSH  is suitable for querying on $L_2$ distance, but our GRW-LSH focuses on $L_1$ distance. In GP-LSH, the raw hash value $f(\mathbf{s})$ is defined as $\vec{\mathbf{s}}\cdot \vec{\bm{\eta}}$, where ``$\cdot$'' is the inner product (which is mathematically a {\it projection}) and $\vec{\bm{\eta}}=\langle \eta_1,\cdots, \eta_m\rangle$ is an $m$-dimensional i.i.d. standard Gaussian random vector (fixed after generation). The most stressed difference is that in GRW-LSH, the $j^{th}$ dimension contributes to $f(\mathbf{s})$ a $s_j$-step Gaussian random walk, which is the sum of $s_j$ i.i.d. standard Gaussian RVs, whereas in GP-LSH, it contributes $s_j\eta_j$, which is $s_j$ times a fixed Gaussian RV $\eta_j$. 
Therefore, for GP-LSH $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$ follows $\mathcal{N}(0, d_2^2)$, which reflects the $L_2$ distance between $\vec{\mathbf{s}}$ and $\vec{\mathbf{q}}$ instead of the $L_1$ distance.

\end{comment}


\begin{comment}
[duplicate]In \autoref{sec:dsthash}, we have shown that a surprisingly cheap implementation of DST that uses low-level hash functions with two-wise independence guarantees the same distribution of range-sums as a ``real'' random walk.
Therefore, by maintaining $m$ independent such DSTs, one for each random walk $\tau$, we have an efficient DST-based implementation of RW-LSH that
%Therefore, we can evaluate $f(\mathbf{s})$ by generating the range-sum of each random walk $S^{\tau_j}[0, s_j)$ with the method described inn order to generate range-sums of single-step random walks that has the same distribution as ``real'' random walks,  and using . on the $j^{th}$ coordinate this DST uses t.I, which uses the definition of splits in \autoref{sec:randw} and l This leads to the following This implementation 
does not need the precomputed tables and guarantees  the $f(\mathbf{s})  - f(\mathbf{q})$ to be a $d_1$-step random walk, because each of the range-sums $S^{\tau}[q, s)$ is a $|q - s|$-step random walk by \autoref{cor:stdist}.
%Obviously, we can avoid the precomputed table by directly generating the range-sum $S^{\tau}[0, t)$ of each random walk $\tau$ with dyadic simulation as . study the efficient implementation with dyadic simulation of only
This DST-based RW-LSH implementation may be useful in some applications that restrict the hash values to integers. However, we will show that the DST-based GRW-LSH (defined below) is even better in that it is faster and as accurate. 
As a result, we focus on the DST-based efficient implementation of only GRW-LSH, which we simply refer to as GRW-LSH in the sequel, and we refer to the original scheme in~\cite{mprwlsh} with precomputed tables as RW-LSH in the sequel. 


[duplicate] In GRW-LSH, the raw hash value function $f$ is %a random walk projection 
parameterized by a vector of $m$ mutually independent Ganssian random walks $\bm{\zeta} = \langle \zeta_1, \cdots, \zeta_m \rangle$. %, which we unrigorously refer as ``Brownian with Gaussian steps motions'' in the sequel to distinguish from the random walks with integer steps in RW-LSH. 
Each  $\zeta_j$ is defined by a sequence of steps that are i.i.d. standard Gaussian RVs, which differs from the (integer-valued random walk) $\tau_j$ at the marginal distribution of each step. Given a data point $\mathbf{s} = \langle s_1, s_2, \cdots, s_m \rangle$, $f(\mathbf{s})$ is defined as $\sum_{j=1}^m S^{\zeta_j}[0, s_j)$.
Similarly, GRW-LSH requires that each $s_j$, $j=1,2,\cdots, m$, be a nonnegative integer. GRW-LSH achieves similar accuracy in ANNS-$L_1$ as RW-LSH, because Gaussian random walks are statistically close to integer-valued random walks when the number of steps is large. %and it is better suited for a DST-based implmentation, 

[duplicate] Our DST-based GRW-LSH implementation is the same as the DST-based RW-LSH above, except that it uses the split definitions in \autoref{sec:gauss} to generate Gaussian steps instead of single-step random walks in \autoref{sec:randw}. It runs faster than the DST-based RW-LSH, because Gaussian distribution is  ``nice'', so its range-sums can be generated four times as fast as those of single-step random walks (shown in \autoref{sec:dyaperf}). %uses the splits described in~ and low-level hash function that are two-wise independent for each Brownian motion $\zeta$, 
It also has a similar guarantee as above that
$f(\mathbf{s}) - f(\mathbf{q}) = \sum_{j=1}^m (S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j))$ is a Gaussian random walk of $\sum_{j=1}^m |s_j-q_j| = d_1$ steps and follows Gaussian distribution $\mathcal{N}(0, d_1)$, for the following 
reason:  For each $j$, $j = 1, 2,\cdots, m$, $S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j)$ equals to either $S^{\zeta_j}[q_j, s_j)$ or $S^{\zeta_j}[s_j, q_j)$ depending on which one in $s_j$ and $q_j$ is greater, which is always an
$|s_j - q_j|$-step Gaussian random walk along the sequence $\zeta_j$, and these 
$m$ Gaussian random walks are mutually independent since they are along different sequences. 
The distribution of $f(\mathbf{s}) - f(\mathbf{q})$ resembles its counterpart in GP-LSH~\cite{Datar_LSH_2004} and differs only in the variance, since the latter follows $\mathcal{N}(0, d_2^2)$ where %$\mathcal{N}(0, d_2^2)$. 
$d_2^2$ is the squared $L_2$ distance between $\mathbf{s}$ and $\mathbf{q}$, \ie $d_2 ^2= \sum_{j=1}^m (s_j-q_j)^2$. This resemblance is important, because it implies that GRW-LSH is an LSH function similarly to GP-LSH and inherits GP-LSH's multi-probe extension~\cite{lv2007multiprobe}, which greatly reduces the number of hash tables for reaching a target query accuracy. We call the version of GRW-LSH with multi-probe extension MP-GRW-LSH in the sequel.
\end{comment}

%Obviously, we can avoid the precomputed table by directly generating the range-sum $S^{\tau}[0, t)$ of each random walk $\tau$ with dyadic simulation as . study the efficient implementation with dyadic simulation of only
%This DST-based RW-LSH implementation may be useful in some applications that restrict the hash values to integers. 



%In GRW-LSH, the raw hash value function $f$ is %a random walk projection 
%parameterized by a vector of $m$ mutually independent Ganssian random walks $\bm{\zeta} = \langle \zeta_1, \cdots, \zeta_m \rangle$. %, which we unrigorously refer as ``Brownian with Gaussian steps motions'' in the sequel to distinguish from the random walks with integer steps in RW-LSH. 
%Each  $\zeta_j$ is defined by a sequence of steps that are i.i.d. standard Gaussian RVs, which differs from the (integer-valued random walk) $\tau_j$ at the marginal distribution of each step. Given a data point $\mathbf{s} = \langle s_1, s_2, \cdots, s_m \rangle$, $f(\mathbf{s})$ is defined as $\sum_{j=1}^m S^{\zeta_j}[0, s_j)$.
%Similarly, GRW-LSH requires that each $s_j$, $j=1,2,\cdots, m$, be a nonnegative integer. GRW-LSH achieves similar accuracy in ANNS-$L_1$ as RW-LSH, because Gaussian random walks are statistically close to integer-valued random walks when the number of steps is large. %and it is better suited for a DST-based implmentation, 



%Let $\mathbf{q}= \langle q_1, q_2, \cdots, q_m \rangle$ be the query point.  
%We denote as $d_1$ the value of the $L_1$ distance between $\mathbf{s}$ and $\mathbf{q}$, that is, $d_1 = \sum_{j=1}^m |s_j-q_j|$;
%$d_1$ is a nonnegative integer since every $s_j$ and $q_j$ is.
%Then 
%Our DST-based GRW-LSH implementation is the same as the DST-based RW-LSH above, except that it uses the split definitions in \autoref{sec:gauss} to generate Gaussian steps instead of single-step random walks in \autoref{sec:randw}. It runs faster than the DST-based RW-LSH, because Gaussian distribution is  ``nice', so its range-sums can be generated four times as fast as those of single-step random walks (shown in \autoref{sec:dyaperf}). %uses the splits described in~ and low-level hash function that are two-wise independent for each Brownian motion $\zeta$, 
%It also has a similar guarantee as above that
%$f(\mathbf{s}) - f(\mathbf{q}) = \sum_{j=1}^m (S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j))$ is a Gaussian random walk of $\sum_{j=1}^m |s_j-q_j| = d_1$ steps and follows Gaussian distribution $\mathcal{N}(0, d_1)$, for the following 
%reason:  For each $j$, $j = 1, 2,\cdots, m$, $S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j)$ equals to either $S^{\zeta_j}[q_j, s_j)$ or $S^{\zeta_j}[s_j, q_j)$ depending on which one in $s_j$ and $q_j$ is greater, which is always an
%$|s_j - q_j|$-step Gaussian random walk along the sequence $\zeta_j$, and these 
%$m$ Gaussian random walks are mutually independent since they are along different %sequences. 
%The distribution of $f(\mathbf{s}) - f(\mathbf{q})$ resembles its counterpart in GP-LSH~\cite{Datar_LSH_2004} and differs only in the variance, since the latter follows $\mathcal{N}(0, d_2^2)$ where %$\mathcal{N}(0, d_2^2)$. 
%$d_2^2$ is the squared $L_2$ distance between $\mathbf{s}$ and $\mathbf{q}$, \ie $d_2 ^2= \sum_{j=1}^m (s_j-q_j)^2$. This resemblance is important, because it implies that GRW-LSH is an LSH function similarly to GP-LSH and inherits GP-LSH's multi-probe extension~\cite{lv2007multiprobe}, which greatly reduces the number of hash tables for reaching a target query accuracy.

%We now describe the implementation of each Brownian motion $\zeta$ via dyadic simulation (here we drop the subscript $j$, with the understanding that each $\zeta_j$ is an independent instance of $\zeta$). Unlike in data streaming, a surprisingly cheap implementation of dyadic simulation has all theoretical guarantees of BM-LSH on ANNS-$L_1$, even though its singletons are not mutually independent. In this implementation, the random strings $C_\alpha$ (in \autoref{sec:overview}) are generated with a two-wise hash function on each level of the simulation tree, so a simulation tree takes only $O(\log U)$ space and generates each range-sum in $O(\log U)$ time. According to \autoref{th:stdist}, this implementation guarantees that each range-sum $S^{\zeta} [a, b)$ follows distribution $\mathcal{N}(0, b-a)$, so for each $a, b = 0, 1, \cdots, U-1$ (without loss of generality, suppose $b> a$), $\zeta(b) - \zeta(a)$ has the same distribution of an
%$(b-a)$-step Brownian motion.
%This is sufficient to show that $f(\mathbf{s}) - f(\mathbf{t})$ follows $\mathcal{N}(0, d_1)$ and all theoretical guarantees of BM-LSH above.


==> sections/datastreaming.tex <==
\color{black}
\section{Data Streaming Application}\label{sec:datastreaming}
%We would like to generalize our scheme to split hash values that follow the general stable distribution, in order to estimate the $l^p$ norm of a stream with format $[a_i, b_i]$. 

%This section is for Danupon's prior works on simulating minwise hashing (MinHash). This scheme can be used to estimate the $F_0$ norm (number of distinct elements) in a stream.and ERM 

% are used  solving with range updates,   We have a unified framework to estimate the $L_1$ or $L_2$ norm under the turnstile model using range-summable Gaussian (described in \autoref{sec:gauss}) and Cauchy random variables via dyadic simulation. We can also estimate the $1$-dimensional size of union using MinHash (uniformly distributed random variables on $[0, 1]$. , in combination with dyadic simulation,
%estimate the frequency moments and size of union of interval streams., and $F_0$ moment (number of distinct elements) (\autoref{sec:l0algo})
%In Section ???, we describe how to provably achieve the same $(\epsilon, \delta)$-approximation as the 
%naive solutions that are efficient with point updates but not efficient with range updates, 

%by using an different 4-way-independent hash function at every level in the 
%case of $L_2$, and by using Nisan's PRNG in the others.  

% the case of $L_2$-norm estimation, we can 
%To achieve an $(\epsilon, \delta)$ approximation theoretically, all of the above algorithms requires a pseudorandom generator as the source of randomness, and we will %specify this proof using $L_0$ estimation as an example.

%JFM-1 (from old 3.0.1) We now turn to estimating the frequency norms of interval streams. 
\begin{comment}
+++++++++++++++++++++++++++++++++++++++++\\
-------------------------------------------------------------------------------------------------------

\textcolor{teal}{ 
	We now turn to estimating the frequency norms of interval streams. We can estimate the first and the second frequency moments ($L_1$ and $L_2$) under the turnstile model using range-summable Gaussian (described in \autoref{sec:gauss}) and Cauchy random variables via dyadic simulation. We further generalize dyadic simulation to generate range-minimizable random variables in  exponential distribution, and propose an algorithm to estimate the $L_0$ frequency moment under the cash register model. To achieve an $(\epsilon, \delta)$ approximation theoretically, all of the above algorithms requires a pseudorandom generator as the source of randomness, and we will specify this proof using $L_0$ estimation as an example.\\
\textbf{Formulation is in introduction}
\\
First, we formulate the problem of frequency moment estimation for interval streams.
\begin{definition}
	Given a stream of tuples of the form $([a_i, b_i], c_i)$, where the interval $[a_i, b_i]\subseteq \mathcal{U}$ and the weight $c_i$ is an integer, suppose we have a counter $x_j$ for each $j\in \mathcal{U}$ that is initialized as $0$. Whenever a tuple $([a_i, b_i], c_i)$ arrives, for each $j\in[a_i, b_i]$ the corresponding counter $x_j$ is incremented with $c_i$. In other words, $x_j = \sum_{i: j\in [a_i, b_i]} c_i$. The $k$-th frequency moment is the $L_p$ norm of all counters $L_p = \left(\sum_{j\in \mathcal{U}} |x_j|^p\right)^{\frac{1}{p}}$. In particular, the $0$-th frequency moment is defined as $L_0 = \sum_{j\in \mathcal{U}} |x_j|^0$, which is the number of nonzero counters.
\end{definition}
If all of the weights $c_i$ are positive integers, this frequency moment problem is in the \emph{cash register model}. Otherwise, if some of the weights are negative integers, this problem is in the \emph{turnstile model}.
\\}

JFM-2 (from old 3.1.3)
As in the definition, computing the exact frequency moment requires $U$ counters \textbf{cite??}, so using $O(\log U)$ memory in practice, we may at best get an estimation of $L_p$ with the following approximation guarantee.
-------------------------------------------------------------------------------------------------------\\+++++++++++++++++++++++++++++++++++++++++
\end{comment}

%By combining 
%, we arrive at 
In this section, we describe a
novel efficient algorithm that contains 
two variants for estimating the $L_2$-norm and the $L_1$-norm respectively of a data stream with range updates.
It combines the classic $L_p$-norm 
sketching algorithm~\cite{stabledist} for a stream of point-updates, 
whose underlying RVs are Gaussian when $p = 2$ and
are Cauchy when $p = 1$, 
with our ERS solutions, \ie Gaussian-DST (in the $L_2$-norm case) and Cauchy-DST (in the $L_1$-norm case). 
%how our  strengthen Indyk's algorithms for two data streaming problems,  namely,for the  and the Cauchy distributions
%the estimations of $L_1$- (\autoref{sec:dstheo}) and $L_2$-norms (\autoref{sec:ersl2}) to efficiently process range-update data streams.  
%The two combined algorithms achieve the same theoretical guarantees as in the original point-update version. 

%the provably achieves $(\epsilon, \delta)$-approximation (defined below) by using one four-wise independent hash function at each level 
%case of $L_2$, and by using Nisan's PRNG in the other cases (\autoref{sec:dstheo}).  that are used at the end as estimators {\bf using polylogarithmic time and space complexities}.

Here we provide an oversimplified description of the original $L_p$-norm sketching algorithm~\cite{stabledist} that is good enough
for our purpose.  
The original algorithm employs a {\it sketch} comprised of $r > 0$ i.i.d. accumulators (viewed as RVs) $A_1, A_2, \cdots, A_r$.  
After a data stream has passed, the values of these $r$ accumulators serve as the raw statistics that the $L_p$-norm of the 
data streaming shall be estimated from, using an estimator that is a (deterministic) function of the raw statistics.

Since $A_1, A_2, \cdots, A_r$ are independent and functionally equivalent, 
it suffices to describe the point-update procedure for one such accumulator, 
which we denote as $A$, in the original algorithm~\cite{stabledist}.  $A$ is initialized to $0$ at the beginning.  
Given a point update $(i_t, \delta_t)$, $A$ is incremented by $\delta_t  X_{i_t}$, where $X_{i_t}$ is 
a standard Gaussian (for $L_2$-norm) or Cauchy (for $L_1$-norm) RV (fixed after being generated on-demand
for the first time) that is associated with 
the counter $\sigma_{i_t}$.  Hence, after the entire data stream has passed, $A = \sum_{i=0}^{U-1}\sigma_i X_i$,
where $\sigma_i$ denotes also the value of the $i^{th}$ counter $\sigma_i$ at the end.  

The original algorithm can handle range updates as follows.
Given a range update $([a_t, b_t), \delta_t)$, %, where $X_{i_t}$ is a random variable that .
%The value (realization) of such an $X_i$ is typically derived,  from the binary string resulting from 
% like those described above, results from 
%hashing the index $i$ using a uniform random hash function $h(\cdot)$, i.e., $X_i = h(i)$).$A$ is incremented by $\sum_{i=a_t}^{b_t-1}\delta_t  X_{i_t}$. can be used to accomplish this task
it makes $b_t - a_t$ point updates to $A$:
\begin{itemize}
	\item For $ i = a_t$ to $b_t- 1$, do $A\gets A + \delta_t  X_i$.
\end{itemize}

This update procedure is inefficient when $b_t - a_t$ is gigantic, as explained earlier.  
However, the net effect of this range update is to increment $A$ by $\delta_t \cdot (\sum_{i=a_t}^{b_t-1} X_i)$,
which boils down to computing the range-sum $S[a_t, b_t)$ in the parenthesis.
%In contrast, our algorithm supports 
In our algorithm, $S[a_t, b_t)$ is efficiently computed using a Gaussian-DST (in the first variant for $L_2$-norm) 
or a Cauchy-DST (in the second variant for $L_1$-norm).

When our algorithm is used instead, we also have $A = \sum_{i=0}^{U-1}\sigma_i X_i$, except that the underlying
RVs $X_0$, $X_1$, $\cdots$, $X_{U-1}$ are generated on demand using a Gaussian-DST or a Cauchy-DST.
Hence if these underlying RVs are assumed to be i.i.d. (which they are, at least empirically), then $A$ produced by 
our algorithm has the same distribution as that produced by the original algorithm.  
%our algorithm is statistically identical to the original algorithm in the following sense.  
In other words, the raw statistics produced by our algorithm have the same distribution as those produced by 
the original algorithm.  Since our algorithm also uses the same estimator function (of the raw statistics), for both the $L_1$-norm 
and the $L_2$-norm cases, our algorithm has the same accuracy guarantees as the original algorithm. 




%For ease of presentation, we assume, for the moment, that the underlying RVs are i.i.d. in both algorithms.  
%Under this assumption,


%, because   as $A$ if they are defined on independently drawn random variables 
%The condition that $A_j$'s are mutually independent can be easily guaranteed by generating each sequence of $X_0, X_1$, $\cdots$, $X_{U-1}$ from independent DSTsof mutually independent .
%{\color{red} At the initialization stage, a series of underlying RVs $X_0, X_1, \cdots,$ $X_{U-1}$ are fixed, according to a target distribution such as Gaussian or Cauchy, and each of them $X_i$ is associated with a counter $\sigma_i$. For now, we assume these RVs are ideally i.i.d., which will be weakened to be practically implementable shortly.}




\begin{comment}
Efficient range updates are supported once the underlying RVs used by $A$ are generated by a DST, because 
the net effect of the range update above is to increment $A$ by $\delta_t \cdot (\sum_{i=a_t}^{b_t-1} X_i)$.  
Hence making this range update is reduced to an ERS problem of computing the range-sum of underlying RVs inside the parenthesis. {\color{blue} This said, we do not consider our
combined algorithm a separate contribution to the data streaming literature, since its raw statistics and the estimators are the same as those in the original point-update algorithm~\cite{stabledist}.  We consider it a contribution to the ERS literature as a novel application of 
our ERS solutions.}




As far as this work is concerned, a data streaming algorithm consists of the following two stages:
online update  In the online stage, it maintains a relatively (to the length
of the data stream) small number of
accumulators, and in the offline stage, after the entire data stream has been processed, it estimates the result using the final state of the accumulators as raw statistics. 
{\color{red} Since the accumulators $A_1, A_2, \cdots, A_r$ are maintained in the same manner but with mutually independent realizations of the underlying RVs, they are i.i.d. random samples in the raw statistics.}

In the offline stage, this accumulator $A=\sum_{i=0}^{U-1}\sigma_i X_i$, because each point update above that increases $A$ by $\delta_t X_{i_t}$ also increases $\sigma_{i_t}$ by $\delta_t$, so the increment is the same for both sides of the equation.}

\end{comment}

% for which a celebrated solution called the Tug-of-War sketch~\cite{} was proposed.  




%where $X_i = h(i)$ as explained earlier.   

%In this work, we consider a more general type of data stream that supports range updates.  


   



\begin{comment}
To this end, we start with an oversimplified characterization of the data stream model that is barely sufficient for all these applications.  In this model, the system stateThe 
is comprised of a large number (say $U$) of counters $\sigma_0$, $\sigma_1$, $\cdots$, $\sigma_{U-1}$ whose values are initialized to 0.  The data stream is comprised of a largeTherefore,  the classic streaming algorithm supports .
number (say $N$) of data items.  Each item, say the $t^{th}$, in On the other hand, 
the data stream is in the form $(l_t, \delta_t)$.  This data item should cause the following update to the system state:   Counter $\sigma_{l_t}$ is to be incremented by $\delta_t$.   
A typical data streaming problem is to estimate 
a certain function of the counter values after the updates caused by all the data items in the data stream are committed to the system state.  
For example, the $L_2$-norm and the $L_1$-norm estimation problems are
to estimate the values of $(\sum_{i=0}^{U-1}|C_i|^2)^{\frac{1}{2}}$ 
(the $L_2$-norm of the system state) and $\sum_{i=0}^{U-1}|C_i|$, respectively.
In a range-update data stream, each data item is in the form $\allowbreak([a_t, b_t), \delta_t)$.  In this case, for each index $i$ in the range $[a_t, b_t)$, the corresponding counter $\sigma_i$ needs to be incremented by 
$\delta_t$.  
\end{comment}

%\begin{definition}
%	A (randomized) switching algorithm returns an $(\epsilon, \delta)$-approximate estimator $\hat{d}_p$ if the probability for the relative error to be greater than $\epsilon$ is at most $\delta$, \ie
%	$	\Pr(|d_p - \hat{d}_p| > \epsilon d_p ) < \delta.$
%\end{definition} 






\begin{comment}
\begin{algorithm}
	\SetAlgoLined\LinesNumbered
	\KwData{a stream of tuples $([a_i, b_i], c_i)$}
	\KwResult{an estimate of the $L_p$ frequency moment of this stream}
     \textbf{Initialization}\\
	Let $Y[1\cdots l]$ be an array of floating point numbers set
	to 0.0 at the beginning of measurement interval\;
	Fix $l$ $p$-stable hash functions $sh_1$ through $sh_l$\;
	\textbf{Online Stage}\\
	\For{each tuple $([a_i, b_i], c_i)$}{
		\For{$k$ from $1$ to $l$}{
			$Y[k] \gets Y[k] + c_i\cdot \sum_{j=a_i}^{b_i} sh_k(j)$\;\label{indyk:update}
		}
	}
	\textbf{Offline Stage}\\
	%\Return $med(|Y[1]|,\cdots,|Y[l]|)/DMed_p$, where $DMed_p$ is the (unique) value $x_0$ such that $\mathcal{P}(|S(p)|>x_0) = 0.5$.\;
	Estimate and return $\hat{d}_p$ by the corresponding estimator.\;
	\caption{Algorithm to estimate $L_p$ norm for $p=1$ or $2$.}\label{algo:indyk}
\end{algorithm}
\end{comment}

\begin{comment}
\begin{algorithm}
	\SetAlgoLined\LinesNumbered
	\KwData{a stream of tuples $([a_t, b_t), \delta_t)$}
	\KwResult{an estimate of the $L_p$ frequency moment of this stream}
	\textbf{Initialization}\\
	Let $A[1\cdots r]$ be an array of floating point numbers set
	to $0.0$ at the beginning of measurement interval\;
	For each $j=1,2, \cdots, r$, fix a sequence of i.i.d. random variables $X_0^j, X_1^j,\cdots, X_{U-1}^j$ drawn from standard Gaussian (for $L_2$) or Cauchy (for $L_1$) distribution\;
	\textbf{Online Stage}\\
	\For{each tuple $([a_t, b_t), \delta_t)$}{
		\For{$j$ from $1$ to $r$}{
			$A[j] \gets A[j] + \delta_t\cdot \sum_{i=a_t}^{b_t-1} X_i^j$\;\label{indyk:update-new}
		}
	}
	\textbf{Offline Stage}\\
	%\Return $med(|Y[1]|,\cdots,|Y[l]|)/DMed_p$, where $DMed_p$ is the (unique) value $x_0$ such that $\mathcal{P}(|S(p)|>x_0) = 0.5$.\;
	Estimate and return $\hat{d}_p$ by the corresponding estimator\;
	\caption{Algorithm to estimate $L_p$ norm for $p=1$ or $2$.}\label{algo:indyk-new}
\end{algorithm}
\end{comment}

%\subsection{Estimation of $L_2$ with Range-updates}\label{sec:ersl2}

It was proven, in the original algorithm~\cite{stabledist}, that 
when the random strings (like our ($C_{\alpha*}$)'s) underlying the ($X_i$)'s are generated using Nisan's PRNG~\cite{nisan}, the value of an accumulator $A$ is statistically indistinguishable from that when the ($X_i$)'s are i.i.d.  
Our algorithm 
provably inherits this property when ($C_{\alpha*}$)'s are generated using Nisan's PRNG. 
% although the underlying RVs ($X_i$)'s are converted from the generated ($C_{\alpha*}$)'s by the DST}
%in the following sense: {\color{red} The value of $A$ generated using a DST using a Nisan's PRNG as its hash function is statistically 
%indistinguishable from that generated when the ($X_i$)'s are strictly i.i.d.  } We omit its proof, since it is a minor modification of 
%that in~\cite{stabledist}.  
As a result, our algorithm (both the $L_1$-norm and the $L_2$-norm variants) inherits all the accuracy guarantees proved in~\cite{stabledist}, when every underlying DST is powered by a Nisan's PRNG.

\begin{comment}
For $L_1$ estimation, $X_1, X_2$, $\cdots$, $X_n$ are i.i.d. standard
Cauchy random variables, 
whose pdf is $f_X(x) = 1/(\pi(1+x^2))$. 
 By the stability property of Cauchy distribution under $L_1$~\cite{stabledist}, in the offline stage, the accumulator $A$  follows 
 $\mathrm{Cauchy}(0, d_1)$, where $d_1 = |\sigma_1| + |\sigma_2| + \cdots + |\sigma_n|$ is the $L_1$ norm of the data stream. 
 To estimate the $L_1$ norm, the following median estimator is used %of $l$ sketches(for the scale parameter of a Cauchy random variable centered at $0$)  for $d_1$ Indyk's algorithm~\cite{stabledist} uses
 \begin{equation}\label{eq:cauesti}
 	\hat{d}_1 = med(|A_1|, |A_2|, \cdots,|A_r|).
 \end{equation}
{\bf JFM new} Generating the underlying RVs with a hashing-based Cauchy-DST is empirically valid, and has only $O(\log U)$ complexity in terms of space and update time.

[JFM new] In order to guarantee some approximation ratio (say $\epsilon$), the same argument for $L_2$ cannot be used here, because the median estimator is not ``well-bahaved''.
However, we may use the same argument as in the classical point-update algorithm~\cite{stabledist}: Use Nisan's PRNG to provably ``fool'' the online stage combined with the DST, so that it produces raw statistics that are indistinguishable from those in the ideal case. We only need to show in the proof that the newly added DST part also has a small space bound. As a result, the estimator in the offline stage has the same guarantees, such as approximation ratio, as the ideal case.
With this theoretically strong implementation, each accumulator has roughly $O(\log ^2 U)$ complexities in space and update time.


\end{comment}

As mentioned in \autoref{sec:indepguarantee}, Nisan's PRNG is computationally inefficient.     
In comparison, 4-wise independent 
hash functions are much more efficient computationally but provide much weaker theoretical guarantees.
We now state and prove a surprising result that get the better of both worlds:  
For $L_2$-norm estimation only, when 4-wise independent hash functions 
are used in each underlying DST, 
our algorithm can achieve the same accuracy guarantees using the same
number of accumulators as when the underlying RVs are assumed to be i.i.d.

Recall that an accumulator $A$ has value $\sum_{i=0}^{U-1}\sigma_i X_i$ at the end of a data stream.
For $L_2$-norm estimation, each $X_i$ has a standard Gaussian distribution $\mathcal{N}(0, 1)$.
Hence, when the underlying RVs $X_0$, $X_1$, $\cdots$, $X_{U-1}$ are assumed
to be independent, each
%In the offline stage, 
%this accumulator $A=\sum_{i=0}^{U-1}\sigma_i X_i$, because each point-update above that increases $A$ by $\delta_t X_{i_t}$ also increases $\sigma_{i_t}$ by $\delta_t$, so the increment is the same for both sides of the equation.
%By the stability property of Gaussian distribution, after the online stage, each accumulatorTherefore, 
accumulator $A_j$, $j = 1, 2, \cdots, r$, has distribution $\mathcal{N}(0, d_2^2)$, where its 
variance $d_2^2 = \sigma_1^2 + \sigma_2^2 + \cdots + \sigma_n^2$ is the squared $L_2$-norm of the data stream.
%Recall that the sketch is comprised of the $r$ accumulators denoted as $A_1, A_2, \cdots A_r$.  
In our algorithm, like in the original algorithm~\cite{stabledist}, the estimator for the squared $L_2$ norm $d_2^2$ is
%Indyk's algorithm~\cite{stabledist} uses the  for , %square of $L_2$ norm
%, we will use the following UMVUE\cite{sttinf} for $d^2_2$, the variance of Gaussian samples whose expectation is known,(for  $0$), which comes from~\cite{ams},  =d_2^2
$
	\hat{d_2^2}= \left(A^2_1+A^2_2 + \cdots+A^2_r\right)/r. 
$

%estimated from the following UMVUE (uniform minimum variance unbiased estimator)

We have $E[\hat{d^2_2}] =1/r\cdot \sum_{j=1}^r E[A^2_j] $ by the linearity of expectation.
Note that $A_1, A_2, \cdots, A_r$ are i.i.d. since they are generated by independent DSTs. 
%With a slight abuse of notation, we denote their common distribution as $A$.
Hence we have $E[(\hat{d^2_2})^2] = \left(\sum_{j=1}^r E[A^4_j] +\right.$ $\left. 2 \sum_{j=1}^r\sum_{j'=j+1}^r E[A^2_j]E[A^2_{j'}]\right)/r^2$. 
By~\autoref{th:fourwise}, the values of each $E[A_j^2]$ and $E[A_j^4]$, and hence the values of $E[\hat{d^2_2}]$ and $E[(\hat{d^2_2})^2]$
remain unchanged whether the underlying RVs are 4-wise independent or all-wise independent;  and hence so does $Var[\hat{d^2_2}] =E[(\hat{d^2_2})^2]  - E^2[\hat{d^2_2}]$.   
In other words, 
the statistical efficiency of the estimator $\hat{d_2^2}$ remains the same whether the underlying RVs are 4-wise independent or all-wise independent.

 \begin{theorem}\label{th:fourwise}
 Let $A=\sum_{i=0}^{U-1}\sigma_i X_i$ be an accumulator as defined above, and $X_0, X_1$, $\cdots$, $X_{U-1}$ be standard Gaussian RVs.  Then the values of $E[A^2]$ and $E[A^4]$ remain the same whether
 the underlying RVs are $4$-wise independent or all-wise independent.
 % with $E[X] = 0$ and $Var[X] = 1$, then the probability that the estimator in \autoref{eq:gauesti} deviates from $d^2_2$ by at more than $\epsilon d^2_2$ is at most $1/8$. %the probability for an estimate to fail (to have larger relative error than $\epsilon$ can be bounded by $1/4$ with $r = O(1/\epsilon^2)$ accumulators. and use the median of all estimates as the final estimate that all follow marginal distribution $\mathcal{N}(0, 1)$n independently generated 
	%To further boost the success probability to $1-\delta$ for arbitrarily small $\delta$, the streaming algorithm only needs to return the median of $2\log 1/\delta$ independent estimations as above. because they are generated by independent DSTs,
%	$E[A^2] = \sum_{i=0}^{U-1}\sigma_i^2 E[X^2] = d_2^2$ and $Var[A^2] = \sum_{i=0}^{U-1}\sigma_i^4 (E[X^4]-E^2[X^2]) + 4\sum_{i=0}^{U-1}\sum_{i'=i+1}^{U-1}\sigma_i^2\sigma_{i'}^2 E[X^2]=2d^4_2$. 
\end{theorem}

The proof of \autoref{th:fourwise} is a straightforward adaptation of that of Theorem 2.2 in \cite{ams}, in which each underlying RV is a single-step random walk.

% originally to Gaussian distribution.

\begin{comment}

unbiased and has the same efficiency (variance) as the ``best'' estimator in the ideal case even if the underlying RVs $X_0, X_1, \cdots, X_{U-1}$ are weakened to being $4$-wise independent. By \autoref{th:nwise}, this condition can be easily satisfied by 
a hashing-based Gaussian-DST whose low-level hash functions are $4$-wise independent, each of which has $O(1)$ space and time complexity if implemented by polynomial hashing~\cite{univhash}. Therefore, each accumulator, together with the DST that serves it, has only $O(\log U)$ complexity in terms of space and update time.

Furthermore, if $A_j$'s are i.i.d. as the $A$ above for $j=1,2,\cdots, r$,  then $E[\hat{d^2_2}] = d_2^2$ and $Var[\hat{d^2_2}] = 2d_2^4/r$.


$X_1, X_2$, $\cdots$, $X_{U-1}$ % (here we drop the superscript $j$, since they are i.i.d. sequences for $j=1, 2, \cdots, r$) $f(\cdot)$ 
are i.i.d. standard Gaussian RVs, with pdf $f_X(x) = 1/\sqrt{2\pi} \cdot e^{-x^2/2}$, expectation $E[X]=0$, variance $Var[X] = E[X^2]=1$ and fourth moment $E[X^4]=3$. 
%After the online stage (having processed the entire stream), the accumulator $A[j] = \sigma_1X^j_1 + \sigma_2X^j_2 + \cdots + \sigma_nX^j_n$, where $\sigma_0, \sigma_1, \cdots, \sigma_{U-1}$ are the value of counters (defined in \autoref{sec:streamintro}), because each range-update $\delta_t \cdot X^j_{i_t}$ corresponds to incrementing $\sigma_{i_t}$ by $\delta_t$. 


%Therefore,  the following estimator

Given $r$ accumulators $A_1, A_2, \cdots A_r$, the squared $L_2$ norm $d_2^2$ is then estimated from the following mean-value estimator:
%Indyk's algorithm~\cite{stabledist} uses the  for , %square of $L_2$ norm
%, we will use the following UMVUE\cite{sttinf} for $d^2_2$, the variance of Gaussian samples whose expectation is known,(for  $0$), which comes from~\cite{ams},  
\begin{equation}\label{eq:gauesti}
	\hat{d_2^2}= \left(A^2_1+A^2_2 + \cdots+A^2_r\right)/r, 
\end{equation}
which is the UMVUE (uniform minimum variance unbiased estimator) for the variance of Gaussian samples with known mean $0$~\cite{sttinf},  the ``best'' unbiased estimator for these raw statistics. Its variance $Var[\hat{d_2^2}] = d^4_2/r\cdot (E[X^4]-E^2[X^2])= 2d^4_2/r$. % because of the fact $E[X^4]=3$. , where $X$ is standard Gaussian $\mathcal{N}(0, 1)$, .it does not require the underlyingthe sense  bthe same We still The weakened assumption can now be easily met with is  ``well-behaved'' in that even in this weakened setting, itfrom being mutuallyThe range-sum of $4$-wise independent underlying RVs can be efficiently computed by independent ideally to beingcombined with  Since each such low-level hash function
We now weaken the assumption on 

For $L_2$, Our combined streaming algorithm has the same theoretical guarantees on accuracy even if a practical hashing-based DST is used instead of an ideal one, thanks to the ``well-behaved'' estimator $\hat{d_2^2}$.
By~\autoref{th:fourwise}, the estimator $\hat{d_2^2}$  is  still unbiased and has the same efficiency (variance) as the ``best'' estimator in the ideal case even if the underlying RVs $X_0, X_1, \cdots, X_{U-1}$ are weakened to being $4$-wise independent. By \autoref{th:nwise}, this condition can be easily satisfied by 
a hashing-based Gaussian-DST whose low-level hash functions are $4$-wise independent, each of which has $O(1)$ space and time complexity if implemented by polynomial hashing~\cite{univhash}. Therefore, each accumulator, together with the DST that serves it, has only $O(\log U)$ complexity in terms of space and update time.
%have the same theoretical guarantees, because this estimator is well-behaved by  It is still unbiased and has the same , even if the condition on the RVs $X^j_0, X^j_1$, $\cdots$, $X^j_{U-1}$ is weakened from mutual independence in the ideal case to $4$-wise independence that be practically guaranteed by generating RVs from $X^j_i \triangleq h^j(i)$, where $h^j(\cdot)$ is a . %Therefore, we can simply generate each underlying random variable $X^j_i$ as . 

\end{comment}


%To support range-updates for $L_2$ estimation, we only need to make $h^j(\cdot)$ for each $j=1,2,\cdots, r$ efficiently range-summable., which was originally for $X$'s that arebut can be easily generalized to as well
%By , such a four-wise independent ERS hash function can be emulated by a DST   that is implemented by  four-wise independent low-level hash functions.  

%\subsection{Estimation of $L_1$ with Range-updates}\label{sec:dstheo}

%\subsection{Indyk's Streaming Algorithm for $L_1$ and $L_2$}\label{sec:strl1l2}

%is the state of the data structures, more 
%A data streaming algorithm, from a statistical point of view, constructs an estimator from some raw statistics, which are specifically the values of accumulators  after processing the data stream. During the online stage, the accumulators are updated on the arrival of each tuple in the input stream, and this framework of updating is similar for $L_1$ and $L_2$ as in \autoref{algo:indyk-new}. After having processed the entire data stream, the value of the $j^{th}$ accumulator is $A[j] = \sigma_1X^j_1 + \sigma_2X^j_2 + \cdots + \sigma_nX^j_n$, , because  $ \sigma_i = \sum_{t: a_t \leq i < b_t} \delta_t$.
%\begin{alignat}{2}
%A[j] &=  \sum_t  \sum_{i=a_t}^{b_t-1}\delta_t X^j_i &{}={}& \sum_{i=0}^{U-1} \sum_{t:a_t\leq i < b_t}\delta_t X^j_i \nonumber\\
%&=\sum_{i=0}^{U-1} X^j_i \sum_{t:a_t\leq i < b_t}\delta_t  &{}={}& \sum_{i=0}^{U-1} \sigma_i X^j_i, \nonumber
%\end{alignat}
%where $\sigma_0, \sigma_1, \cdots, \sigma_{U-1}$ are the value of counters (defined in \autoref{sec:streamintro}). In the offline stage, the algorithm returns an estimate of the frequency norm from these accumulator values (raw statistics). 

%each range-update $\delta_t \cdot X^j_{i_t}$ corresponds to incrementing $\sigma_{i_t}$ by $\delta_t$.


\begin{comment}
[duplicate] When it comes to $L_1$, the median estimator is used, which is not of a ``nice'' form, so the same argument for $L_2$ cannot be used. Instead, we use Nisan's PRNG to generate underlying random variables that are indistinguishable from being truly random to any space-bounded finite space machine (FSM). Since the online stage is such an FSM, it outputs the raw statistics that is indistinguishable for any estimator from the ideal case when all underlying random variables are mutually independent, and when the accuracy of estimation is guaranteed as in~\cite{stabledist}.

 ==================== old below
 

% The critical part of this algorithm is a set of \emph{p-stable hash functions} $sh_i$, $i=1,\cdots, l$, which maps an integer $j\in \mathcal{U}$ into a random value drawn from the stable distribution $S(p)$. 


The following property earns the name for the stable distributions. Let $X_1, X_2, \cdots, X_n$ denote mutually independent random variables that have distribution $S(p)$, then $a_1X_1 + a_2X_2 + \cdots + a_nX_n$ has the same distribution as $(|a_1|^p + |a_2|^p + \cdots + |a_n|^p)^{1/p}X$, where $X$ is a random variable having distribution $S(p)$. It is not hard to verify that the aforementioned Gaussian and Cauchy random variables satisfy the stability property with parameter $p$ equal to $2$ and $1$, respectively.

=================== old above
 

 
Indyk's algorithm~\cite{stabledist} (\autoref{algo:indyk-new}) is a general approach to estimate the $L_p$ norm with $0<p\leq 2$ of a data stream in low space complexity, which relies on the following property of stable distributions $S(p)$.  Let $X_1, X_2, \cdots, X_n$ denote mutually independent random variables that have distribution $S(p)$, then $a_1X_1 + a_2X_2 + \cdots + a_nX_n$ has the same distribution as $(|a_1|^p + |a_2|^p + \cdots + |a_n|^p)^{1/p}X$, where $X$ is a random variable having distribution $S(p)$. %(and ) distribution. %a large number of mutually independent random variables from the family of stable distributions, which, discovered first by Paul L\'evy, is a natural generalization of the Gaussian distribution~\cite{zolotarev1986one} for the following property. 
We only consider two special cases for $p=2$ ($S(2)$ is Gaussian distribution) or $1$ ($S(1)$ is Cauchy) here, because the specific dyadic simulation scheme for general stable distributions, whose pdf has no closed-form expression, remains an open problem. 

 \end{comment}

%random variables to be mutually independent to guarantee the $(\epsilon, \delta)$-approximation of the estimation. %while guaranteeing the estimation is independent.




%By a simple application of Chebyshev's inequality, the probability for an estimate to fail (to have larger relative error than $\epsilon$ can be bounded by $1/4$ with $r = O(1/\epsilon^2)$ accumulators. To further boost the success probability to $1-\delta$ for arbitrarily small $\delta$, Indyk's algorithm performs $O(\log 1/\delta)$ independent estimations and use the median of all estimates as the final estimate. 

%JFM-5 (old 5.2.2) The hash functions $sh_i$, $i=1,\cdots, l$ maps each integer $j\in \mathcal{U}$ into a random value drawn from the stable distribution $S(p)$, in such a way that (a) the same flow label will always be mapped to the same random value and (b) different flow labels are mapped to independent random values. In addition, these $p$-stable hash functions are independent of one another.
%end
%By the stability of Gaussian distribution, assuming all random samples $sh_k(j)$ are independent and have infinite precision for all $j$ and $k$, 
%Under this assumption of independent hashes the stable distribution under $L_1$ norm

 %Because Cauchy distribution has no mean or variance, we use $(\epsilon, \delta)$-approximation (defined below) to measure the accuracy.
 %According to Lemma 2 of \cite{stabledist}, $\hat{d}_1 $ is $(\epsilon, \delta)$-approximate if $r=O(1/\epsilon^2\log1/\delta)$ accumulators that follow i.i.d. $\mathrm{Cauchy}(0, d_1)$ are used. %This leads to the same asymptotic space complexity as in the $L_2$ moment estimation.
% Cauchy distribution has the following : Let $X_1, X_2, \cdots, X_n$ denote i.i.d. standard  Cauchy random variables with distribution $X$, then $\sigma_1X_1 + \sigma_2X_2 + \cdots + \sigma_nX_n$ has the same distribution as $\left(|\sigma_1| + |\sigma_2| + \cdots + |\sigma_n|\right)\cdot X$. As a result, each accumulator $A[j]$ 
%after the online stage (the raw statistics) [j]
%When it comes to $L_1$, the median estimator is used, which is not of a ``nice'' form, so the same argument for $L_2$ cannot be used. Instead, we use Nisan's PRNG to generate underlying random variables that are indistinguishable from being truly random to any space-bounded finite space machine (FSM). Since the online stage is such an FSM, it outputs the raw statistics that is indistinguishable for any estimator from the ideal case when all underlying random variables are mutually independent, and when the accuracy of estimation is guaranteed as in~\cite{stabledist}.




==> sections/evaluation_simple.tex <==
\section{Evaluation of MP-GRW-LSH}\label{sec:eva}

In this section, we study, via evaluations over frequently used datasets, whether MP-GRW-LSH
can achieve similar ANNS-$L_1$ query efficacies as 
MP-RW-LSH while not 
using a precomputed table as MP-RW-LSH does.  
%in reducing the index size 
%against MP-RW-LSH in terms of ANNS-$L_1$ query efficacy.  
For each query point $\vec{\mathbf{q}}$, we compute the range-sums involved in computing its $L M$ hash values using 
Gaussian-DST in MP-GRW-LSH, and using a precomputed table in MP-RW-LSH.

%We do not evaluate our range-efficient data streaming algorithm
%(for $L_1$ or $L_2$ estimation), because it generate sketches that are identical to those generated by the original range-inefficient {\bf (point-update)} algorithms~\cite{stabledist},
%and this range-efficiency aspect has been evaluated in~\autoref{sec:datastreaming}.


\begin{comment}
performance of both Indyk's algorithm and MinHash without dyadic simulation has been theoretically established in literature~\cite{stabledist, minhashesti}. 

dyadic simulation in two aspects. The first aspect is correctness. Although dyadic simulation is defined in \autoref{sec:dyasim} to be mathematically correct given some assumptions (fresh RV), our implementation is based on a hash function~\cite{wyhash} that does not meet the assumptions for the sake of efficiency, so we validate that the generated singletons are empirically i.i.d. via Kolmogorov-Smirnov testing in \autoref{sec:kstest} \textbf{not moved yet}.
The second aspect is the performance in speed and accuracy in real-life applications. We do not evaluate data streaming, because the performance of both Indyk's algorithm and MinHash without dyadic simulation has been theoretically established in literature~\cite{stabledist, minhashesti}. We do not experimentally compare with range-efficient sampling in estimating $F_0$~\cite{rangeeff, twoimpf0}, because these schemes are not implemented by the authors, and we do not have a well-received benchmark for fair comparison. 

% (with the template-generated probing sequence) 
%CP-LSH, and SRS.
% \textbf{Huayi: I do not think it is necessarily to mention this is SRS's variant, in this thesis, the author also call it as SRS and do experiments for $L_1$ distance in a whole chapter.}


Therefore, for the second aspect, we
compare only the ANNS-$L_1$ query performance of MP-GRW-LSH (based on our DST)
against MP-RW-LSH~\cite{mprwlsh} (based on precomputed tables). %those of the following  LSH schemes: 


We only compare with MP-RW-LSH, because in \cite{mprwlsh}, MP-RW-LSH is shown to achieve a much better tradeoff between the query efficiency and scalability than CP-LSH, SRS~\cite{SRS},  and QALSH~\cite{QALSH}, three state-of-the-art LSH solutions for ANNS-$L_1$. 
\textbf{summarize the comparison results in MP-RW-LSH}.
Specifically, compared with CP-LSH, MP-RW-LSH has much better scalability (having $14.8$ to $53.3$ times smaller index size), but only pays slightly longer ($1.3$ to $2.2$ times) query time. Compared with SRS, MP-RW-LSH has consistently smaller index sizes (excluding the \SI{8}{GB} fix cost per hash table) and much shorter query times, especially on large datasets. Compared with QALSH (running on a Ubuntu RAM disk to avoid paying disk I/O's), MP-RW-LSH has much smaller ($1.79$ to $73.2$ times) index sizes and much shorter ($1.8$ to $46.2$ times) query times when achieving similar or higher query accuracy.
\end{comment}
%Among all baseline LSH schemes for ANNS-$L_1$, 

%CP-LSH (in terms of query efficiency) and SRS (in terms of scalability) are two state-of-the-art LSH solutions for ANNS-$L_1$. Although  both CP-LSH and SRS, it has to store all hash values in a precomputed table, because there is no suitable range-summable hashing schemes.  \textbf{For each hash table (with $M$ hash functions), a maximum of $mUM$ bytes is needed for storing the precomputed table, which can cause problems when scaling to datasets with high dimensions and large universes. With dyadic simulation, we can drastically reduce the memory overhead to $O(mM\log U)$ (for storing the seeds of the splitting mechanism) and increases the time complexity of evaluating one LSH function only slightly from $O(m)$ to $O(m\log U)$.}
%Our evaluations show conclusively that although its baseline RW-LSH is ``mediocre'' compared to CP-LSH and SRS,
%MP-RW-LSH achieves a much better tradeoff between the query efficiency and scalability than both CP-LSH and SRS.


\subsection{Experiment Settings}\label{subsec:exp_set}
\noindent
\textbf{Evaluation Datasets.}
\begin{table}[!ht]
\caption{Datasets summary.}\label{tab:dataset-stats}
\centering
{\begin{tabular}{@{}ll cccccc@{}}
\specialrule{.1em}{.05em}{.05em} 
 \multicolumn{2}{c}{Dataset} & $n_d$ & $m$ & $n_q$ & $U$ & Type\\ 
\specialrule{.1em}{.05em}{.05em} 
  \multirow{4}{*}{Small} &Audio~\cite{audio} &53.3K & \num{192} & \num{200} & 200K &Audio\\
&MNIST~\cite{mnist} & 69.0K & \num{784} & \num{200} &2K &Image\\ 
&Enron~\cite{enron} & 95.0K  & \num{1369}  & \num{200} &505K &Text  \\
&Trevi~\cite{Trevi} & 99.9K & \num{4096} & \num{200} &510 &Image\\ 
\specialrule{.1em}{.05em}{.05em}
 \multirow{2}{*}{Medium} &GIST~\cite{sift-gist} & 1.0M & \num{960} & 1K &3K &Image\\ 
&GloVe~\cite{glove} & 1.2M & \num{100} & \num{200} &25K &Text\\ 
\specialrule{.1em}{.05em}{.05em} 
  \multirow{2}{*}{Large} &Deep10M~\cite{deep} & 10.0M & \num{96} & 10K &3K &Image\\
&SIFT50M~\cite{sift-gist} & 50.0M & \num{128} & 10K &\num{510} &Image\\ 
\specialrule{.1em}{.05em}{.05em} 
\end{tabular}}
\end{table}
% \subsection{Evaluation Datasets}\label{subsec:datasets}
We use the same eight widely used publicly available datasets of diverse dimensions, sizes (number of points), and types, as used in~\cite{mprwlsh}. 
% that are widely used in the ANNS literatures. 
%{\bf [not true. Delete this?]The SIFT50M dataset contains 50 million points sampled uniformly at random from the 1 billion points contained in SIFT1B~\cite{sift-gist}, since the index sizes of the
%algorithms that MP-RW-LSH was compared with would be too large to fit into the main memory.}
%We cannot use SIFT1B instead since 
%the resulting index structures of CP-LSH and SRS would not fit into the main memory. 
We normalize the coordinates of all data points to nonnegative even integers using the shift-scale-round operation suggested in~\cite{mprwlsh} in all eight datasets. %To meet the requirement of MP-RW-LSH, we multiply each coordinate of all normalized data and query points by a factor of $2$ to make them nonnegative even integers. 
For each of 
the eight normalized datasets, Table~\ref{tab:dataset-stats} shows its size $n_d$ (number of data points), its dimension $m$, the number of queries $n_q$ processed on it, 
% the maximum coordinate value $U$ across all its dimensions \textcolor{red}{(U for universe)},
its maximum universe $U$ among all coordinates
 and its type.
% and the query time $t_{BF}$ (BF stands for ``Brute Force") that a brute-force linear scan takes on it.
We drop the word ``normalized'' in the sequel with 
the understanding that all datasets we refer to by names have been normalized.



% \end{tabular}
\noindent\textbf{Performance Metrics.} 
%Unless otherwise specified, the number of nearest neighbors searched K is 50 in our experiments.
%in performing 
%approximate K nearest neighbors searches (in $L_1$ distance). 
We evaluate the performances of both algorithms in three aspects:  scalability, query efficiency, and query accuracy.  Both algorithms are implemented and optimized for in-memory operations, and are hence evaluated as such.
To measure scalability (how well an algorithm can scale to very large datasets), we use the {\it index size} (excluding the size of the original dataset).
% and {\it indexing time} (time 
% needed to build the index).  
% Each index size or indexing time value presented
% in this section is the average over several independent runs.  
For each query, each algorithm being evaluated needs to find $K = 50$ nearest neighbors in $L_1$ distance.  
To measure query efficiency, we use {\it query time}.
To measure query accuracy, we use {\it recall}, 
%of an ANNS algorithm 
%The concepts of recall and overall ratio are 
defined as follows.  For a query point $\vec{\mathbf{q}}$, let the query result be $R$ %= \{\mathbf{o_1}, \mathbf{o_2}, \cdots, \mathbf{o_k}\}$ %with its elements sorted in 
%the increasing order of their $L_1$ distances to $\mathbf{q}$, and
and  %=\{\mathbf{{o_1}^*}, \mathbf{{o_2}^*}, \cdots, \mathbf{{o_k}^*}\}$
the actual $K$ nearest neighbors be $R^*$. % similarly sorted. 
The  recall is defined as % $\frac{1}{k} \sum_{i=1}^k ||\mathbf{q}- \mathbf{o_i}||_1 / ||\mathbf{q}-\mathbf{{o_i}^*}||_1$ and 
$|R \cap R^{*}| / K$. %, respectively. 
Each query time or recall value presented in Table~\ref{tab:query}  is the average over many queries. 
% We will mainly use recall as the quality metric which is the most commonly used metric in the
% ANN search literatures~\cite{lv2007multi,Sun16_thesis}. \textbf{Huayi: This sentence might note needed, since we have include both overall ratio and recall except for the two figures.}and \autoref{fig:recall_time}

\noindent
\textbf{Implementation Details.}
%\textbf{Huayi: We can merge implementail details into above sections if needed for space.}
We implement MP-GRW-LSH
% Gaussian-DST-augmented GRW-LSH
 in C++, which uses \texttt{wyhash}~\cite{wyhash} as the hash function  for the splits. For MP-RW-LSH, we 
use the C++ source code used in~\cite{mprwlsh}, which builds on an efficient open-source C++ LSH implementation called \texttt{FALCONN}\footnote{\url{https://github.com/FALCONN-LIB/FALCONN}}.
%for indexing and querying in LSH.
% (the aforementioned third refinement in Sect\,\ref{subsec:mplsh}) 
We compile all C++ source codes using g++ 9.3 with -O3.  
All experiments are done on a workstation running Ubuntu 18.04 with 
Intel(R) Core(TM) i7-9800X \SI{3.8}{GHz} CPU, \SI{128}{GB} DRAM.
% {\color{red} and \SI{4}{TB} hard disk drive (HDD).}


%\subsection{Parameter Settings}\label{sec:parameter}\
\noindent
\textbf{Parameter Settings.}
%Now, we describe how we tune the parameters for the best query performance. 
In both MP-GRW-LSH and MP-RW-LSH, we have four parameters to tune:  $M$ (the dimension of an LSH function vector), 
$W$ (the bucket ``width''),  $L$ (the number of hash tables), and the multi-probe parameter $T$ (number of additional buckets to be probed in each hash table). For both algorithms, we use the same set of parameters suggested by the authors of MP-RW-LSH~\cite{mprwlsh}. 
%\textbf{I do not mention the $\sqrt{2}$ scaling of $W$ here.}
%\noindent
%{\bf MP-RW-LSH.}  
%We use the RW-LSH as described in Sect.~\ref{subsec:lsh-scheme} and MP-RW-LSH with multi-probe as described in Sect.~\ref{subsec:multi_probe_extension} for ANNS-$L_1$. 
%(\textbf{Huayi: I use a wide range instead of a certain number here, since $W$ of LSH is totally different on each datasets, it have to choose certain range for different datasets. Or we %can show the range of $W$ by combining all 7 datasets.}) 
%For RW-LSH, we tune the number of hash functions $M$ and bucket size $W$ in a wide range on all 7 datasets and find the best combination of parameters which appears to strike 
We use the combinations of $(M, W)$ for eight datasets
listed in Table~\ref{tab:dataset-stats} from top to bottom respectively:
$(12, 3144)$, $(12, 930)$, $(9, 122)$, $(16, 1728)$, $(8, 452)$, $(16, 1104)$, $(17, 424)$, $(14, 224)$. % \textbf{For Enron, we tune the parameters that strike the best tradeoff between query accuracy and  efficiency, and use the parameters as suggested by the authors of [cite: Huayi] for the other seven datasets.}
%The same value combinations are used for MP-BM-LSH.
% for Audio, MNIST, Trevi, GIST, GloVe, Deep10M and SIFT50M, respectively. 
%The recommendation from~\cite{lv2007multi} is to set $T$ between 30 and 100. 
We use $T=100$ and %strikes near-optimal tradeoffs between query time and query accuracy for all seven datasets \textbf{, so we fix $T=100$ for now. In Sect.\,\ref{sec:srscomp}, we test the tradeoff between query accuracy and query efficiency for various $T$ values.} For both RW-LSH and 
adjust $L$ to achieve a certain level of query accuracy for each dataset. 

% For simplicity, we refer multi-probe RW-based LSH as ``RW-MPLSH'' in the following sections.
%Since BM-LSH is statistically close to RW-LSH, we use the same set of parameters for MP-BM-LSH as in MP-RW-LSH, except that we divide the $W$ (bucket width) by a factor of $\sqrt{2}$ and round the result to integers, so they become $2223, 658, 86, 1222, 320, 781, 300, 158$ (in the same sequence as above). This is because each coordinate of all data and query points used by MP-RW-LSH is required to be even, so they are made two times of that used by MP-BM-LSH, so the difference of hash values $f(\mathbf{q}) - f(\mathbf{s})$ in MP-RW-LSH has a standard deviation (scaling parameter of Gaussian distribution) that is $\sqrt{2}$ times that of MP-BM-LSH. As a result, we scale the width of hash buckets correspondingly to compensate for this difference.

%\noindent
%{\bf MP-BM-LSH.}  For MP-BM-LSH, we use the same parameter settings of $M$ and $T$ as in MP-RW-LSH, because the two LSH functions (random walk and Brownian motion) are almost the same. For $W$ (bucket width), we divide the values for MP-RW-LSH by $\sqrt{2}$ and round it to the nearest integer for the following reasons. Since MP-BM-LSH requires the coordinates to be nonnegative numbers (instead of nonnegative even numbers as in MP-RW-LSH), MP-BM-LSH takes half as many steps as MP-RW-LSH, which results in a scaling of by $1/\sqrt{2}$ in the shape of the distribution, so we scale the bucket width $W$ for the same ratio to compensate.

\subsection{Compare MP-GRW-LSH with MP-RW-LSH}\label{subsec:comp_lsh}
In this section, we compare MP-GRW-LSH against MP-RW-LSH in terms of scalability and query efficiency.
%while configuring them to achieve similar query accuracy. 
In \autoref{tab:query}, we report the query times and the index sizes needed by both algorithms for achieving similar query accuracies on each dataset. %\textbf{We do not report the overall ratio for Enron, because all four algorithms fail to return $K=50$ candidates for some of the queries, and overall ratio is not well-defined if the number of returned candidates is less than $K$.}
%In order for such comparison, we set the number of hash tables in RW-MPLSH to achieve the best tradeoff between recall and query time on each dataset. 
%Then we tune the number of hash tables of RW-LSH and CP-LSH to match a similar recall value as RW-MPLSH on each dataset. dyadic simulation for Gaussian range-sumswith dyadic simulation,
We have run experiments on other query accuracy levels and observed similar results.
For this evaluation, the query time is 
broken down into two parts: (1) the amount of time it takes to compute the $L M$ hash values (of the query point $\vec{\mathbf{q}}$), denoted as $t_2$ (this 
computation involves $mLM$ table look-ups in the case of MP-RW-LSH and $mLM$ Gaussian-DST ``calls'' in the case of MP-GRW-LSH);  (2) the 
rest, which we denote as $t_1$.
Correspondingly, each query time entry of MP-RW-LSH and MP-GRW-LSH in \autoref{tab:query} is written as ``$t_1$ + $t_2$''.  
The index size of MP-RW-LSH is also broken down into two parts:  (1) the total size of the $L$ hash tables, which we denote as $v_1$; and (2) the total size of the precomputed tables, which we denote as $v_2$.  Hence, each query time entry of MP-RW-LSH in \autoref{tab:query} is written as ``$v_1$ + $v_2$''.  The index size of MP-GRW-LSH is only $v_1$, because  it does not need a precomputed table.

\begin{comment}
\begin{table*}[!htb]
	\caption{Query time (in milliseconds), recall, and index size (in megabytes) results.}\label{tab:query}
	\centering
	\begin{tabular} {@{}|c|c|c|c|c|c|c|c|c|@{\hspace{8pt}}c@{\hspace{8pt}}|@{}}
		\specialrule{.1em}{.05em}{.05em} 
		Algorithm & Metric& Audio & MNIST & Enron &  Trevi & GIST & GloVe & Deep10M & SIFT50M  \\ \specialrule{.1em}{.05em}{.05em} 
		\multirow{3}{*}{MP-RW-LSH}  & Time  & 3.8+0.4 & 11.0+0.6  & 39.3+4.8 & 55.9+4.6 & 353.6+0.7& 151.8+0.2 & 1044.9+0.1 & 5475.7+0.0 \\  \cline{2-10}
		& Recall & 0.9307 & 0.9333 & 0.9337 & 0.9187 & 0.9630 & 0.9766 & 0.9756 & 0.9807  \\  \cline{2-10}
		& Size& 65.6+3515.6 & 66.1+143.6 & 75.3+53389.7 & 50.3+191.3 & 94.5+173.1 & 100.4+304.8&  323.0+40.0 & 1192.4+5.2\\ \specialrule{.1em}{.05em}{.05em} 
		\multirow{3}{*}{MP-GRW-LSH} & Time   & 3.2+1.9 & 9.0+1.8 & 41.1+4.0 &73.2+21.1 &362.7+4.8 & 135.9+1.3& 1002.1+0.7 & 5339.8+0.5 \\  \cline{2-10}
		& Recall & 0.9264 & 0.9404 &   0.9355  & 0.9381 & 0.9617 &  0.9743 & 0.9688 & 0.9836 \\  \cline{2-10}
		& Size & 57.4 & 74.4 & 75.3 & 50.3 & 94.5 & 112.9 & 276.9 & 1192.4  \\ \specialrule{.1em}{.05em}{.05em} 
	\end{tabular}
\end{table*} 
\end{comment}

\begin{table}[!htb]
	\caption{Query time (in milliseconds), recall, and index size (in megabytes) results.}\label{tab:query}
	\centering
	\begin{tabular} {!{\vrule width 0.1em}c|c|c|c|c!{\vrule width 0.1em}}
		\specialrule{.1em}{.05em}{.05em} 
		Dataset & Algorithm & Query Time (ms) & Recall & Index Size (MB) \\ \specialrule{.1em}{.05em}{.05em} 
			\multirow{2}{*}{Audio}  & MP-RW-LSH & 3.8+0.4 & 0.9307 & 65.6+3515.6 \\\cline{2-5}
			& MP-GRW-LSH & 3.2+1.9 & 0.9264 & 57.4 \\\specialrule{.1em}{.05em}{.05em} 
			\multirow{2}{*}{MNIST}  & MP-RW-LSH & 11.0+0.6 & 0.9333 & 66.1+143.6 \\\cline{2-5}
			& MP-GRW-LSH &  9.0+1.8 &  0.9404  & 74.4 \\\specialrule{.1em}{.05em}{.05em} 
			\multirow{2}{*}{Enron}  & MP-RW-LSH & 39.3+4.8  & 0.9337  & 75.3+53389.7 \\\cline{2-5}
			& MP-GRW-LSH &  41.1+4.0 &  0.9355  & 75.3  \\\specialrule{.1em}{.05em}{.05em} 
			\multirow{2}{*}{Trevi}  & MP-RW-LSH & 55.9+4.6 & 0.9187 & 50.3+191.3 \\\cline{2-5}
			& MP-GRW-LSH &  73.2+21.1 &  0.9381  & 50.3 \\\specialrule{.1em}{.05em}{.05em} 
			\multirow{2}{*}{GIST}  & MP-RW-LSH & 353.6+0.7 & 0.9630 &  94.5+173.1  \\\cline{2-5}
			& MP-GRW-LSH &  362.7+4.8  &  0.9617  & 94.5 \\\specialrule{.1em}{.05em}{.05em} 
			\multirow{2}{*}{GloVe}  & MP-RW-LSH & 151.8+0.2 & 0.9766 & 100.4+304.8 \\\cline{2-5}
			& MP-GRW-LSH & 135.9+1.3 & 0.9743  & 112.9 \\\specialrule{.1em}{.05em}{.05em} 
			\multirow{2}{*}{DEEP10M}  & MP-RW-LSH & 1044.9+0.1 & 0.9756 & 323.0+32.7 \\\cline{2-5}
			& MP-GRW-LSH &  1002.1+0.7 & 0.9688  & 276.9 \\\specialrule{.1em}{.05em}{.05em} 
			\multirow{2}{*}{SIFT50M}  & MP-RW-LSH & 5475.7+0.0  & 0.9807  & 1192.4+5.2 \\\cline{2-5}
			& MP-GRW-LSH &  5339.8+0.5 & 0.9836  & 1192.4  \\\specialrule{.1em}{.05em}{.05em} 
	\end{tabular}
\end{table} 



\noindent
{\bf Scalability.} 
%We report the index sizes for reaching similar query accuracy of three classical LSH algorithms in Table~\ref{tab:query} on all 7 datasets.
Table~\ref{tab:query} shows that the $v_1$ (total size of hash tables) values of MP-RW-LSH and MP-GRW-LSH are similar 
across all 8 datasets.  This is because $v_1$ is proportional to $L$ (the number of hash tables used), and for each dataset, 
their $L$ values differ by at most $1$.  
As shown in Table~\ref{tab:query},
since MP-GRW-LSH 
does not pay for the cost of precomputed table ($v_2$),  
it has a significant index size advantage over MP-RW-LSH on 
all small and medium datasets, where $v_2$ is much larger than the corresponding $v_1$. 
%Although for the two large datasets, $v_2$ for MP-RW-LSH is only $12.4\%$ and $0.4\%$ of the corresponding $v_1$, 
%This significantly bloats the total index size $v_1 + v_2$.  
For example, for Enron, which has both a large data dimension $m$ and a large 
universe $U$, its $v_2 = \SI{53389.7}{MB}$ is $709$ times its $v_1 = \SI{75.3}{MB}$!  

%Therefore, by getting rid of $v_2$, MP-GRW-LSH has a much
%smaller total index size than MP-RW-LSH for these datasets.  

%To summarize, by getting rid of the precomputed table, MP-GRW-LSH is even more scalable than MP-RW-LSH.

%has almost the same query efficacy (query time needed to 
%achieve the same query accuracy) as MP-RW-LSH, without paying for a potentially large precomputed table.

%inherits the nice scalability (to large number of data points) 
%of MP-RW-LSH, , and furthermore has even better scalability than MP-RW-LSH to large data dimension $m$ and universe $U$ by replacing the precomputed table (of size $v_2 = O(LMmU)$) to some hash seeds of size $O(LMm\log U)$, which is negligible to $v_2$ when $U$ is very large.



\begin{comment}
%both MP-BM-LSH and MP-RW-LSH has much better scalability than both CP-LSH when $n$ (the number of points in the dataset) is large. On all eight datasets, the index sizes of both MP-BM-LSH and MP-RW-LSH are 11.1 to 53.3 smaller than those of CP-LSH. 
%The numbers of hash tables used in the MP-BM-LSH and MP-RW-LSH are also smaller than those used in CP-LSH and RW-LSH by the same ratios, since 
%this number is proportional to the index size in all three algorithms for the same dataset.

\textbf{Furthermore, MP-BM-LSH has much better scalability than MP-RM-LSH on datasets with large universe sizes $U$. Table?? (whether to merge?) shows that on some of the datasets (Audio and Enron) with large universe size $U$ and small dataset size $n$, the size of the precomputed tables of hash values (which is linear to $U$) can be tens or even hundreds of times larger than that of the index, which can easily become the memory bottleneck. On the contrary, since MP-BM-LSH uses dyadic simulation to compute the hash values, it does not require a precomputed table in memory for queries. (Although it does use a similar precomputed table to accelerate the indexing process, these memories can be safely freed after the index is built.) The space complexity of dyadic simulation is just a negligible $O(\log U)$, so MP-BM-LSH can easily scale to large $U$.}
, which is $O(LMU)$ space, 

\textcolor{teal}{
	Table~\ref{tab:query} clearly shows that MP-RW-LSH has much better scalability than both CP-LSH and RW-LSH.   
	On all seven datasets, the index sizes of MP-RW-LSH are 14.8 to 53.3 and 15.0 to 27.5 times smaller than those of CP-LSH and RW-LSH, respectively. 
	The numbers of hash tables used in the MP-RW-LSH are also smaller than those used in CP-LSH and RW-LSH by the same ratios, since 
	this number is proportional to the index size in all three algorithms for the same dataset.
	%Since for each dataset, a hash table is of the same size in all three algorithms, the number of hash tables used in   
	%The number of hash tables used in MP-RW-LSH is the same order smaller than those of CP-LSH and RW-LSH, respectively. This is because the index size of a classical LSH algorithm is proportional to its number of hash tables %on the same dataset. 
	Fig.\,\ref{fig:recall_time} shows the tradeoffs between
	% \textbf{Huayi: original is display here. }
	recall values achieved and the numbers of hash tables used by the three algorithms on two medium datasets
	GIST and GloVe.  Fig.\,\ref{fig:table_recall_gist} shows that for achieving the same recall value, CP-LSH and RW-LSH need to use roughly 18.2 to 20.1 and roughly 24.8 to 27.5 times more hash tables than MP-RW-LSH on GIST, respectively.
	Fig.\,\ref{fig:table_recall_glove} shows that for achieving the same recall value, CP-LSH and RW-LSH need to use roughly 20.1 to 29.2 and roughly 13.9 to 19.4 times more hash tables than MP-RW-LSH on GloVe, respectively.
	In fact, MP-RW-LSH can scale to the one-billion-point dataset SIFT1B (without sampling)~\cite{sift-gist} with an index size of roughly \SI{24}{GB}, whereas neither CP-LSH nor RW-LSH can 
	(using the \SI{128}{GB} memory the computer has)
	while achieving the same query accuracy as MP-RW-LSH. 
	% \textbf{Huayi: We need to mention for achieving the same query accuracy, since CP-LSH and RW-LSH can fit into the memory with small number of hash tables.}
	%MP-RW-LSH uses more than an order of magnitude less 
	%method reduces the number of hash tables required by the RW-LSH method by more than an order of magnitude. As CP-LSH needs similar number of hash tables as RW-LSH, the numbers of hash tables in MP-RW-LSH 
	%is smaller than those in CP-LSH by a significant factor. 
}
\end{comment}

\noindent
{\bf Query Efficiency.}  %Table~\ref{tab:query} reports the query time and the query accuracy of three classical LSH methods. 
As shown in Table~\ref{tab:query}, although GRW-LSH incurs a 
higher asymptotic time complexity (of $O(\log U)$) for  
evaluating each range-sum than RW-LSH (which incurs $O(1)$ using a precomputed table), 
it makes only a slight difference to the query efficiency of MP-GRW-LSH.
In all four small datasets except Trevi, for achieving similar (or better) query accuracies, the $t_2$ (computation time of hash values) of MP-GRW-LSH is at most $\SI{1.5}{ms}$ longer than that of MP-RW-LSH, which leads to at most $21.4\%$ longer overall query time ($t_1+ t_2$). %On Enron, the $t_2$ of MP-BM-LSH is even shorter than that of MP-RW-LSH, because the latter has to read from a very large \SI{53.3}{GB} procomputed table that only lies in DRAM. 
On Trevi, the $t_1+t_2$ of MP-GRW-LSH is  $56\%$ longer than that of MP-RW-LSH, because its data dimension $m$ is very large ($4096$) and this $t_2$ involves the computation of $LMm = 6 \times 16 \times 4096 =$ \SI{393216}{} range-sums. Although evaluating each range-sum takes only $\SI{53.7}{ns}$ on average, it is still slower than accessing the precomputed table in memory by a factor of $4.6$. %the complexity of evaluating the hash values is linear to $m$. 
The $t_1$ of MP-GRW-LSH is also slightly longer than that of MP-RW-LSH in this case, because a larger number of ANNS-$L_1$ candidates are found and processed
by MP-GRW-LSH as it uses one more hash table than MP-RW-LSH, which results in it having a higher recall than MP-RW-LSH. 
% clearly shows that MP-RW-LSH significantly outperforms RW-LSH ($4^{th}$ column):
%MP-BM-LSH has  query times on Trevi only, On all other seven datasets, MP-BM-LSH achieves similar query times compared with MP-RW-LSH (whose hash computation is just looking up an entry in the precomputed tables). 
On all four medium and large datasets, MP-GRW-LSH has similar or even slightly shorter total query times than MP-RW-LSH to achieve similar query accuracies, because the slightly longer $t_2$ is only a negligible fraction of $t_1$ in these datasets.

To summarize, although MP-GRW-LSH has a slightly higher asymptotic time complexity of $O(LMm\log U)$ than MP-RW-LSH (which is $O(LMm)$) in computing hash values, this only slightly impacts the query efficiency of MP-GRW-LSH, because $t_2$ is dominated by $t_1$ in most cases.
Overall, it is fair to say that MP-GRW-LSH achieves a much better tradeoff between scalability and query efficiency than MP-RW-LSH.





\begin{comment}

\begin{table*}[!htb]
	\caption{Experiment results overview.}\label{tab:query}
	\centering
	\begin{tabular} {@{}|c|c|c|c|c|@{\hspace{8pt}}c@{\hspace{8pt}}|@{}}
		\specialrule{.1em}{.05em}{.05em} 
		\multicolumn{1}{|c}{} && \textbf{MP-RW-LSH} & \textbf{CP-LSH} & \textbf{MP-BM-LSH} &  \textbf{SRS}  \\ \specialrule{.1em}{.05em}{.05em} 
		\multirow{4}{*}{Audio}  & Query Time (ms)  & 4.2 & 2.4  & 3.2 + 1.9 & 18.0  \\  \cline{2-6}
		& Recall & 0.9307 & 0.9298 & 0.9264 & 0.9140  \\  \cline{2-6}
		& Overall Ratio  & 1.0032& 1.0033 & 1.0037 & 1.0050 \\ \cline{2-6}
		& Index Size (MB) & 65.6 & 968.0 & 57.4 & 3.0  \\ \specialrule{.1em}{.05em}{.05em} 
		\multirow{4}{*}{MNIST} & Query Time (ms)  & 11.6 & 5.6 & 9.0 + 1.8 & 47.7 \\  \cline{2-6}
		& Recall & 0.9333 & 0.9309 & 0.9404 & 0.9314  \\  \cline{2-6}
		& Overall Ratio  & 1.0046 & 1.0048 & 1.0042 & 1.0070  \\ \cline{2-6}
		& Index Size (MB) & 66.1 & 2644.2 & 74.4 & 3.8  \\ \specialrule{.1em}{.05em}{.05em} 
		\multirow{4}{*}{Enron}  & Query Time (ms) &  44.2 & 40.8 &41.1 + 4.0 & 64.9 \\  \cline{2-6}
		& Recall &  0.9337 &  0.9376 & 0.9355 & 0.9323  \\  \cline{2-6}
		& Overall Ratio  &  - &  - &  - &  -\\  \cline{2-6}
		&Index Size (MB)   & 75.3 & 836.2  & 75.3 & 5.4
		\\ \specialrule{.1em}{.05em}{.05em} 
		\multirow{4}{*}{Trevi}  & Query Time (ms)  & 60.5 & 40.4 & 73.2 + 21.1 & 86.8  \\  \cline{2-6}
		& Recall & 0.9187 & 0.9162 & 0.9381 & 0.9144  \\  \cline{2-6}
		& Overall Ratio  & 1.0035 & 1.0038 & 1.0022 & 1.0042  \\  \cline{2-6}
		&Index Size (MB)  & 50.3 & 2681.9  &  50.3 & 5.7  \\ \specialrule{.1em}{.05em}{.05em} 
		\multirow{4}{*}{GIST}   & Query Time (ms)  & 354.3 & 247.0 & 362.7 + 4.8 & 1045.8  \\  \cline{2-6}
		& Recall & 0.9630 & 0.9576 & 0.9617 & 0.9602  \\  \cline{2-6}
		& Overall Ratio  & 1.0009 & 1.0010 & 1.0009 & 1.0010  \\  \cline{2-6}
		& Index Size (MB)  & 94.5 & 1417.8 & 94.5  & 52.6  \\ \specialrule{.1em}{.05em}{.05em} 
		\multirow{4}{*}{GloVe}  & Query Time (ms)  & 152.0 & 119.2 & 135.9 + 1.3 & 557.1  \\  \cline{2-6}
		& Recall & 0.9766 & 0.9753 & 0.9743	 & 0.9648  \\  \cline{2-6}
		& Overall Ratio  & 1.0006 & 1.0007 & 1.0006 & 1.0010  \\  \cline{2-6}
		& Index Size (MB)  & 100.4  & 3764.7  & 112.9  & 52.6  \\ \specialrule{.1em}{.05em}{.05em} 
		\multirow{4}{*}{Deep10M}  & Query Time (ms)  & 1045.0 & 560.8 & 1002.1 + 0.7 & 5338.8 \\ \cline{2-6}
		& Recall & 0.9756 & 0.9758 & 0.9688 & 0.9565  \\  \cline{2-6}
		& Overall Ratio  & 1.0008 & 1.0007 & 1.0010 & 1.0017 \\ \cline{2-6}
		& Index Size (MB)  & 323.0 & 6922.0 & 276.9 & 525.2  \\ \specialrule{.1em}{.05em}{.05em}  
		\multirow{4}{*}{SIFT50M}  & Query Time (ms)  & 5475.7 & 2445.0 & 5339.8 + 0.5 & 28302.9  \\  \cline{2-6}
		& Recall & 0.9807 & 0.9809 & 0.9836 & 0.9595 \\  \cline{2-6}
		& Overall Ratio & 1.0006 & 1.0005 & 1.0005 & 1.0017  \\ \cline{2-6}
		& Index Size (MB) & 1192.4 & 19873.5 & 1192.4 & 2656.8  \\ \specialrule{.1em}{.05em}{.05em} 
	\end{tabular}
\end{table*} 

\begin{table}[!htb]
	\caption{Size of precomputed tables.}\label{tab:precomputesize}
	\centering
	\begin{tabular} {@{}c c c@{}}
		\specialrule{.1em}{.05em}{.05em} 
		Dataset & Size of precomputed tables (MB) & Ratio over index size \\\specialrule{.1em}{.05em}{.05em} 
		Audio &   3515.6 & 53.6\\
		MNIST & 143.6 & 2.17\\
		Enron & 53389.7 &  709.4\\
		Trevi & 191.3 & 3.80\\
		GIST & 173.1 & 1.83\\
		GloVe & 304.8 & 3.04\\
		Deep10M & 40.0 & 0.124\\
		SIFT50M & 5.2 & 0.004    \\
		\specialrule{.1em}{.05em}{.05em} 
	\end{tabular}
\end{table} \end{comment}

%dyadic times
%audio 5.1
%MNIST 10.7
%enron 45.1
%Trevi 94.4
%GIST 367.5
%glove 137.2
%deep 1002.8
%sift 5340.3
% sizes per hash table
% audio 8.204 8 7
% MNIST 8.263 8 9 
% Enron 8.362 9 9 100
% Trevi 8.381 6 6
% GIST 11.815 8 8
% GloVe 12.549 8 9
% deep10M 46.147 7 6
% sift50M 198.73 6 6
% Due to our significant advantages on scalability, our RW-MPLSH could scale to 
% More hash tables in classical LSH generally predicts longer indexing time. Although the construction time of each hash table in MP-RW-LSH is higher than CP-LSH, since RW-MPLSH has a precomputed time cost as described in Sect.\ref{subsec:rw_lsh_issue}, however since the number of hash stables in RW-MPLSH is significantly smaller than CP-LSH, indexing time of MP-RW-LSH is still smaller than CP-LSH. Our measurement of the indexing times for three classical LSH methods has confirmed that. For example, on Deep10M, it takes MP-RW-LSH, CP-LSH and RW-LSH 364.4s, 615.1s and 6421.6s to build their indices respectively. 

%\begin{figure*}
%	\centering
%	\includegraphics[width=\textwidth]{figures/mp1}
%	\caption{Query time under different recalls.}\label{fig:recall_time}
%\end{figure*}
\begin{comment}
some figures

\begin{figure}[htb]
$ \centering
\begin{subfigure}[t]{0.5\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/gist_v4}
\caption{GIST}\label{fig:table_recall_gist}
\end{subfigure}%
\begin{subfigure}[t]{0.5\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/glove_v4}
\caption{GloVe} \label{fig:table_recall_glove}
\end{subfigure}
\caption{Number of hash tables vs. recall.}\label{fig:table_recall}
\end{figure} $
\end{comment}



\section{Empirical Independence of Underlying RVs}\label{sec:kstest}

In this section, we show that the underlying RVs generated from our RW-DSTs and Gaussian-DSTs are empirically independent for ANNS-$L_1$. Recall from \autoref{sec:ann} that performances of MP-RW-LSH and the more efficient MP-GRW-LSH are theoretically guaranteed by the following property: The distribution of the difference in raw hash values $f(s)-f(q)$ on one coordinate %LSH requires that the range-sum $S[s, t)$ 
is a $|s-q|$-step random walk (or Gaussian random walk). We empirically show this is the case on three groups of different values of $|s-q|$, \ie small ($|\SI{623490}{}-\SI{623390}|=100$), medium ($|\SI{690830}{}-\SI{689808}|=\SI{1022}{}$) and large ($|\SI{844567}{}-\SI{834491}|=\SI{10076}{}$), to represent the possible distances between the query point and its nearest neighbor in different scenarios. In each case, we generate \SI{10000}{} samples of range-sums from  independent RW-DSTs for RW-LSH or Gaussian-DSTs for GRW-LSH, both of which are implemented with \texttt{wyhash}~\cite{wyhash} and parameterized by the universe size $U=2^{20}$, and compare their empirical cdfs with the standard cdfs in \autoref{fig:rw_ann} and \autoref{fig:gaussian_ann}, respectively. We also compare the EH3-based RW-LSH scheme~\cite{feigenbaum} against the standard cdf of random walks in \autoref{fig:feigen_ann}.

These figures shows that although \texttt{wyhash} cannot guarantee perfect independence, the empirical cdfs of two dyadic simulation schemes match the standard cdfs without any observable difference, so it is safe to empirically ``believe'' that the difference in raw hash values distribute as a strict (Gaussian) random walk that consists of mutually independent underlying RVs. However, the difference in raw hash values of the EH3-based random walk have a very different distribution, as its empirical cdf greatly deviates from the standard cdf, especially on the tails and near $x=\pm 30$ in the medium distance case. Therefore, the EH3-based random walk cannot provide good empirical guarantees as required by RW-LSH.

\begin{comment}For both applications, we construct some practical ``workloads'' and generate a large number of sample range-sums from independent DSTs. We compare the distributions of the raw statistics, which are the final values of the accumulators for data streaming and the difference in raw hash values $f(s)-f(q)$ on one coordinate for ANNS, with those in the ``ideal'' case where the singletons are i.i.d. 
For the data streaming application, we create a simulated data stream consisting of $100,000$ intervals on a universe $0, 1, \cdots, 2^{32}-1$. To generate each interval in stream, we first generate the length $b_t - a_t$ from a power-law distribution whose pdf is $f(x) \propto x^{-2}$ on range $[2^{10}, 2^{32}]$ and round it to integers, and then uniformly generate the starting point $a_t$ conditioning on $a_t \geq 0$ and $b_t \leq 2^{32}$. For $F_0$ estimation, the increment $\delta_t$ is always $1$ as in \autoref{sec:datastreaming}, and  for $L_1$ and $L_2$ estimation, $\delta_t$ is inversely proportional to the length of each interval, i.e. $\delta_t = \lfloor 2^{32} / (b_t-a_t) \rfloor$, so that each interval update has similar $L_1$ norms. $3/4$ of the increments are assigned a plus sign, and the remaining $1/4$ are assigned a minus sign, so that the overall effect of the stream is biased to the positive direction.  This design simulates a ``tough'' data streaming case, which contains both short and abrupt intervals (impulses) and long but insignificant intervals (backgrounds). This particular interval stream has a ground truth $F_0$ moment %(disregarding cancellation of plus and minus increments)
 of $1.030\times 10^{9}$, an $L_1$ norm of $4.220\times 10^{14}$ and an $L_2$ norm of $3.016\times 10^{10}$. We calculate the sketch value $A$ with three versions of the streaming algorithm (exponential for $F_0$, Cauchy for $L_1$ and Gaussian for $L_2$) in \autoref{sec:datastreaming} with $10,000$ independent DSTs, and plot the empirical cdf (from these samples) against the standard cdf (in the ideal case parameterized by the ground truth) in \autoref{fig:stream_cdf}.

\begin{figure*}
	\centering
	%\begin{subfigure}[b]{0.33\textwidth}
	%	\centering
	%	\includegraphics[width=\textwidth]{figures/exponential}
	%	\label{fig:exp_stream}
%	\end{subfigure}
	\begin{subfigure}[b]{0.33\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/cauchy}
		\label{fig:cau-stream}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.33\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/gau_stream}
		\label{fig:gau-stream}
	\end{subfigure}
	\caption{Comparisons of empirical cdf with standard cdf (calculated from ground truth).}
	\label{fig:stream_cdf}
\end{figure*}
\end{comment}



\begin{figure*}[!ht]
	\centering
	\includegraphics[width=\textwidth]{figures/randwalk}
	\caption{Random walk from RW-DST.}
	\label{fig:rw_ann}
\end{figure*}
\begin{figure*}[!ht]
	\centering
	\includegraphics[width=\textwidth]{figures/feigenbaum}
	\caption{Random walk from EH3~\cite{feigenbaum}.}
	\label{fig:feigen_ann}
\end{figure*}
\begin{figure*}[!ht]
	\centering
	\includegraphics[width=\textwidth]{figures/gau_ann}
	\caption{Gaussian random walk from Gaussian-DST.}
	\label{fig:gaussian_ann}
\end{figure*}

%In this testing, we show that the empirical cdfs of all raw statistics from dyadic simulation match the corresponding standard cdf, but 


==> sections/glibert-paragraphs.tex <==
========= The Gilbert paragraphs are all here below

The values of its vertices are defined in a``top-down'' approach, \textbf{as proposed by \etal{Gilbert} in~\cite{dyahist}}. We first define the value of the root as a random variable from the distribution $X^{*U}$, and for every non-leaf vertex $\alpha$ in the simulation tree, we recursively define the value of its two children $S_{\alpha0}$ and $S_{\alpha1}$ from a specially designed operation that ``splits'' $S_\alpha$ into $S_{\alpha0}$ and $S_{\alpha1}$ while satisfying the invariant $S_\alpha = S_{\alpha0} + S_{\alpha1}$.
 As an example, we describe how the range-sum $S_{100*}$ of dyadic interval $[8, 10)$ is generated (the universe is still $[0, 16)$). Instead of defining $S[8, 10) \triangleq X_8 + X_9$ as in the naive ``bottom-up'' approach, $S_{100*}$ is defined by splitting its parent $S_{10*}$, which is in turn split from the grandparent $S_{1*}$,  and in the end, derived from the sum of universe $S_{*}$, which is generated directly from $X^{*16}$ disregarding the singletons. %Generally, the range-sum of a dyadic interval $\alpha$ can be defined in $|\alpha|$ (the length of the prefix $\alpha$) splits, which is at most $\log_2 U$ splits for any $\alpha$ in the simulation tree. 
This ``top-down'' approach has an advantage that the value of each vertex is defined by $O(\log U)$ splits from the top instead of $O(U)$ singletons from the bottom, so it can be efficiently computed by applying these $O(\log U)$ splits even if we store only a single value $S_{*}$ in memory.
%By splitting the range-sum of the parent into two, we can guarantee the same invariant that the range-sums of two children add to the parent one. 
The computed value is consistently the same if the split on each vertex consistently returns the same pair of children values, which behavior fixes an instance (and the values of all singletons) of a simulation tree.

\textcolor{purple}{(unused: why call it dyadic simulation)
1. In this section, we briefly describe the general framework by \etal{Gilbert} \cite{dyahist}. We will use the summation operation as a example, although the general idea also works with minimization. The name \emph{dyadic simulation} comes from two of its features as follows.1) The universe is divided into levels of \emph{dyadic intervals} that form a small size partition of any input interval. 2) The range-sum of each such dyadic interval is computed by a top-down sampling mechanism that simulates the process of range-summation in the inverse direction. We will start with the definition of dyadic intervals before specifying the rationales of this design. In this sequence, we refer to the number of integer points in an interval as the \emph{size} of the interval. For example, the size of $[a, b)$ ($b\geq a$) is $b-a$.
}

\etal{Gilbert} only mentioned the idea of a top-down simulation tree but did not work out (publish) the details of designing and implementing the actual splitting operation (the core of dyadic simulation). The suggested solutions they gave (using inverse transform method for splitting Cauchy random variables) have theoretical bounds, but are not efficient in practice. Furthermore, there has been no follow-up works on this topic ever since, perhaps because of a belief that dyadic simulation is only a technique of theoretical interest, but not practical for applications. In Section\,\ref{sec:overview}, we recap the simulation tree and showing the general principle of designing the splitting mechanism for all target distributions and then work out the practically implementable splitting operations for Gaussian, Cauchy, exponential (range-minimizable), and random walks in \autoref{sec:gauss} through \autoref{sec:randw}.



====

A sketchy idea of \emph{dyadic simulation} and how it can be used for efficiently computing the range sum of i.i.d. Cauchy and Gaussian RVs were proposed, in a few
sentences, in~\cite{dyahist}.   The focus of~\cite{dyahist} is, however, on a data streaming problem called histogram maintenance, of which the ERS 
problem is a small part of.  Hence, although~\cite{dyahist}
has since been cited hundreds of times, but to the best of our knowledge never for ERS.  

{\bf JFM:} \cite{dyahist} suggested that a random
variable (which we denote as $L$) 
that lies at the center of each aforementioned binary-split operation should be generated by a particular conditional distribution, but did not provide detailed and efficient techniques on how to sample from this conditional distribution.   For example, we will explain in \autoref{sec:dyasim} that, for Cauchy distribution, the inverse 
transform method suggested in~\cite{dyahist} is not efficient.   

{\color{red} It was suggested in \cite{dyahist} that inverse transform is to be used for generating a random
variable (which we denote as $L$) 
that lies at the center of each aforementioned binary-split operation.   However, we will explain in \autoref{sec:dyasim} that, in both cases of Cauchy and Gaussian, the inverse 
transform method is not efficient.  Instead, we propose efficient techniques for generating this $L$ in both cases that takes only nanoseconds.  
}



A very sketchy idea of \emph{dyadic simulation} was proposed, in a few
sentences, in a theory paper~\cite{dyahist}.   
Although it was stated in~\cite{dyahist} that dyadic simulation can possibly be used for the ERS of Gaussian and Cauchy RVs, 
no specific technique was prescribed for binary-splitting a Gaussian RV,
and the suggested technique for binary-splitting a Cauchy RV is not computationally efficient as we will elaborate in \autoref{sec:cauchy}.
The ``footprint'' of the dyadic simulation idea is tiny in~\cite{dyahist}, since the focus of~\cite{dyahist} is on a very different problem in data streaming and sketching 
called space-efficient histogram maintenance (SEHM), of which ERS is only a tiny building block.  
Likely for this reason, although~\cite{dyahist}
has been cited hundreds of times for SEHM, to the best of our knowledge, 
%it has never been cited for the (seminal) contributions to ERS and 
the dyadic simulation idea has never been cited, or followed up, for ERS. 
% work on the idea exists.  

%Also, like many other theory papers, no or little detail is provided 

Our work substantiates and significantly extends the dyadic simulation 
idea in two aspects.  First, we propose computationally efficient statistical techniques in sufficient detail (for reproducibility) for binary-splitting not only Gaussian and Cauchy, but also random walk and exponential RVs.  
Second, since to guarantee the strict independence among the $U$ underlying RVs requires remembering (storing) the random seed values generated 
(but fixed after their generations) during the binary splits, which we will explain can incur a prohibitively high storage cost, we propose three broad classes of 
generalized hash-based solutions (with Nisan's PRNG as the ``luxury'' class) 
that can guarantee, besides empirical independence as the bottomline, varying degrees of provable independence among the underlying RVs. 
In comparison, ``using Nisan's PRNG'' was the only detail provided in~\cite{dyahist} in this regard.  


%recognizing that we generally cannot afford to remember (store) the values of the RVs involved in the binary splits, we propose, prove, and otherwise validate a host of 
%generalized hash-based solutions (including those using Nisan's PRNG) that can provide varying degrees of provable independence while all providing empirical independence.  


No specific technique was prescribed for binary-splitting a Gaussian RV, with ``using standard techniques'' as the only detail provided.    



In comparison, (only for Gaussian and Cauchy), and
the only such statement or information provided in~\cite{dyahist} is that ``standard techniques" shall be used for binary-splitting a Gaussian random variable, and ``inverse transform", 
which we will show is much less computationally efficient than our rejection-sampling-based technique, shall be used for binary-splitting a Cauchy random variable.  

{\bf [JX: to revise accordingly]}
In \cite{dyahist}, the authors (\etal{Gilbert}) suggested to use inverse transform to sample from the pdf above. In order to generate a random variable $X$ with cdf $F_X(x)$, the inverse transform method first generates $Y$ from uniform distribution on $[0,1]$ and then performs the inverse transform $X= F^{-1}(Y)$, where $F^{-1}_X(\cdot)$ is the inverse function of $F_X(x)$. However, we note that inverse transform is not very efficient for the following reasons. Firstly, in the inverse transform method, we need to solve the nonlinear equation $\int_{-\infty}^{S_{\alpha0}} \phi_{n,z}(x)\mathrm{d}x  = Y$ for $S_{\alpha0}$ from a randomly generated $W_{\alpha}\in [0, 1]$, which cannot be solved efficiently with numerical methods. \textbf{Is that true?}. Secondly, even if precomputed tables can be used for storing the answers of the equation above, it will be inefficient in space, because the a posteriori pdf function $f_z(x)$ is dependent on both $n$ (size of $\alpha$, or level on the tree) and $z$. The precomputed table will be three dimensional to work for all possible combinations of $n$, $z$ and $Y$ \textbf{and will be too big to fit in fast memory.}




[to compare with earlier ERS work]  To the best of our knowledge, our work is the first study of the deep connection between ERS and LSH.  


=======

It was suggested in \cite{dyahist} that inverse transform is to be used for generating a random
variable (which we denote as $L$) 
that lies at the center of each aforementioned binary-split operation.   However, we will explain in Section \autoref{sec:cauchy} that, in both cases of Cauchy and {\bf Gaussian}, the inverse 
transform method is not efficient.  Instead, we propose efficient techniques for generating this $L$ in both cases that takes only nanoseconds.  


The core idea of dyadic simulation was originally proposed in~\cite{dyahist} in a very sketchy manner.  
However, since the focus of~\cite{dyahist} is on a now classical data streaming problem called space-efficient 
histogram maintenance (SEHM), and the dyadic simulation was suggested as a solution approach to an ERS subproblem that arises in SEHM.    





In \cite{dyahist}, \etal{Gilbert} proposed the idea of dyadic simulation, which efficiently generates the dyadic components with the structural consistency guarantee by using the Bayes's law to reverse the dependency of the parent on its children. Instead of generating the children-sums and take the summation, dyadic simulation generates the parent-sum $Z$ first and then split it into two i.i.d. children-sums $X$ and $Y$ (that sum up to the parent range-sum). This is the second feature of dyadic simulation: a top-down derandomization of the inverse process of range-summation, which simulation scheme works perfectly well with the top-down recursion of enumerating the minimal dyadic cover, so we do not need to compute or store any range-sum that is a finer component of the minimal dyadic cover. The \emph{splitting mechanism} requires one random sample for each split (because one parent-sum can be possibly split to many combinations of children-sums). The children range-sums $X$ and $Y$ should be independent of each other and follow the marginal distribution of the range-sum, which is determined by the target distribution and size of the range and whose pdf is denoted as $g(x)$. These two arguments guarantee that the leaves (the termination of splitting) will have the target distribution. 

[duplicated above]
The idea of dyadic simulation was originally proposed by \etal{Gilbert}~\cite{dyahist} (back in 2002) for the ERS problem. However,  \etal{Gilbert} only mentioned the idea of a top-down simulation tree but did not work out (publish) the details of designing and implementing the actual splitting operation (the core of dyadic simulation). The suggested solutions they gave (using inverse transform method for splitting Cauchy random variables) have theoretical bounds, but are not efficient in practice. Furthermore, there has been no follow-up works on this topic ever since, perhaps because of a belief that dyadic simulation is only a technique of theoretical interest, but not practical for applications. In Section\,\ref{sec:overview}, we recap the simulation tree and showing the general principle of designing the splitting mechanism for all target distributions and then work out the practically implementable splitting operations for Gaussian, Cauchy, exponential (range-minimizable), and random walks in \autoref{sec:gauss} through \autoref{sec:randw}.

========= The Gilbert paragraphs are all here above





==> sections/lsh-conflict.tex <==
\color{black}
\section{ANNS-$L_1$ Application}\label{sec:ann}
% NOTE: organization of paper       we may need to move the backgrounds of ANN forward and add some contents in introduction.

%[background on ANNS and LSH]





%LSH~\cite{Indyk_ANN_1998} is one of the most popular ANNS solution approaches. 
%In LSH, the key intellectual component of an LSH scheme is its hash function family 
%$\mathcal{H}$.
%Any function $h$ sampled uniformly at random from $\mathcal{H}$ has the following 
%nice collision property:  It maps two distinct points in $\mathcal{D}$ to the same hash %value with probability $p_1$
%if they are close to each other (say no more than distance $r_1$ apart) and with probability $p_2 < p_1$ if they are far apart (say more than $r_2 > r_1$ apart), respectively. 

%In this section, we introduce MP-GRW-LSH, the application of dyadic simulation on ANNS-$L_1$ that improves MP-RW-LSH~\cite{mprwlsh} by scaling highly efficient ANNS queries to huge universes without having to store a large precomputed table. We also show that dyadic simulation is the preferred option over existing range-summable schemes such as EH3~\cite{feigenbaum} on ANNS, because the performance of ANNS is determined by the distribution of the generated range-sums. 
%While the former has a theoretical guarantee on this, the latter does not and can have degraded performances for worst-case queries.


In this section, we first describe an ERS 
problem that arises in MP-RW-LSH, the aforementioned multi-probe LSH solution
for ANNS-$L_1$ proposed in~\cite{mprwlsh}.  Then we study why this problem cannot be robustly
solved using an existing ERS solution called EH3~\cite{feigenbaum}.  Finally, we describe MP-GRW-LSH, a slight variant of MP-RW-LSH that 
can cleanly and robustly solve this problem using our Gaussian-DST.
% Gaussian-DST and
%has nearly identical query efficacy and better efficiency as 
%MP-RW-LSH.





%[change s to vector t, q to vector q]
In ANNS-$L_1$, given a query point $\vec{\mathbf{q}}$, 
we search in a massive dataset $\mathcal{D}$, which lies in a space of high dimensionality (say $m$),  
for one or more points $\mathbf{s}$ in $\mathcal{D}$ that are \emph{among the closest} to $\vec{\mathbf{q}}$ according to the $L_1$ distance.  
Here the $L_1$ distance between any two $m$-dimensional points $\vec{\mathbf{s}}= \langle s_1, s_2, \cdots, s_m\rangle$ and $\vec{\mathbf{q}} = \langle q_1, q_2, \cdots, q_m\rangle$, denoted as $  \|\vec{\mathbf{q}} - \vec{\mathbf{s}}\|_1$, 
is defined as  $\sum_{j=1}^m |q_j - s_j|$.

%\subsection{Locality-Sensitive Hashing (LSH)}d(\mathbf{q}, \mathbf{s})=
\subsection{The RW-LSH Algorithm}

LSH~\cite{Indyk_ANN_1998} is one of the most popular ANNS solution approaches. 
%JFM-1 (new) We first describe RW-LSH, % (Random Walk LSH), 
% and then show how to use dyadic simulation to efficiently implement our ERS-based variant called BM-LSH.(an $m$-dimensional dataset) 
In an LSH scheme, typically a vector of $M > 1$ LSH functions $\vec{\mathbf{g}} = \langle g_1$, $g_2$, $\cdots$, $g_M\rangle$ 
are used to map each point $\vec{\mathbf{s}}$ in $\mathcal{D}$ to an $M$-dimensional vector of independent hash values 
${\overrightarrow{\mathbf{g}(\mathbf{s})}} = \langle g_1(\vec{\mathbf{s}}), g_2(\vec{\mathbf{s}}), \cdots, g_M(\vec{\mathbf{s}})\rangle$.  
This point $\vec{\mathbf{s}}$ is to be stored in a hash bucket indexed 
% \textbf{Jingfan: We do not need to mention $g(\cdot)$ since use hash vector as index in hash table is common sense for readers and our iDEC also write as ``vector as hash key''.}
%({\color{red} say using a conventional hash function $g(\cdot)$}) 
by the vector ${\overrightarrow{\mathbf{g}(\mathbf{s})}}$;
hence we identify this hash bucket as ${\overrightarrow{\mathbf{g}(\mathbf{s})}}$. 
% \textbf{Huayi: I think we need the following sentence to explain each hash table needs one LSH function vector and the meaning of $n$.}
%{\color{red} These $n$ points in $\mathcal{D}$ are 
%stored in a hash table
%using their corresponding vectors as hash keys.}
%({\it e.g.}, the point $\beta$ is to be stored in hash bucket %
%$g(\langle h_1(\beta), h_2(\beta), \cdots, h_k(\beta)\rangle)$.  
Then given a query point $\vec{\mathbf{q}}$, the search procedure, in a standard LSH solution, is to
probe all points in the \emph{epicenter bucket} ${\overrightarrow{\mathbf{g}(\mathbf{q})}}$
%bin 
%that the vector $\langle h_1(\alpha), h_2(\alpha), \cdots, h_k(\alpha)\rangle$ would be inserted into, 
in the hope that 
some nearest neighbors of $\vec{\mathbf{q}}$ are mapped to the same vector (bucket). %bin.
%We regard this search procedure as hard-decision decoding, since 
%the query point $\alpha$ is ``decoded'' to precisely the vector 
%$\langle h_1(\alpha), h_2(\alpha), \cdots, h_k(\alpha)\rangle$ and only the corresponding bucket is probed. 
%$\mathbf{s}\in\mathbb{Z}^{m\smash[t]{\mathstrut}}_{\geq 0}$ is a data or query point,

%A standard LSH solution is one in which only a single hash bucket is searched in each hash table.   is one in which the algorithm(as in standard LSH)


Unlike a standard LSH solution,
a multi-probe LSH solution probes not only the epicenter bucket, but also 
$T > 0$ other nearby buckets whose success probabilities (of containing a nearest neighbor) are among the highest.
%$T$  (excluding the epicenter bucket).
Among LSH solutions, a multi-probe one, if it can be found, is arguably the most desirable one because its index size for achieving the 
same query accuracy is much smaller than that of a standard LSH solution~\cite{mprwlsh}.  


%We now describe what 

{\color{blue} (Add by Huayi) To simplify notation, we focus on only one hash function $g(\vec{\mathbf{s}})$ and drop its subscript in the sequel.}
An LSH function $g(\vec{\mathbf{s}})$ in RW-LSH~\cite{mprwlsh}
%the first multi-probe solution for ANNS-$L_1$. % and in BM-LSH, our ERS-based variant of RW-LSH that has an efficient implementation with dyadic simulation. 
%To simplify notation, we focus on only one hash function $g(\mathbf{s})$ and drop its subscript in the sequel. 
%l, with the understanding that each $g_j(\mathbf{s})$, $j=1,2,\cdots, M$, is an independent instance of $g(\mathbf{s})$.
%In both LSH schemes, same
takes the  following form:  
$g(\vec{\mathbf{s}}) \triangleq  \left\lfloor (f(\vec{\mathbf{s}}) + B)/W \right\rfloor$, 
where  $W > 0$ is a constant and $B$ is a RV (fixed after generation) uniformly distributed in $[0, W]$.
Here $f(\vec{\mathbf{s}})$ is called the \emph{raw hash value} of $\vec{\mathbf{s}}$. 


Before we describe such an $f(\cdot)$, we need to introduce some notations.
Let $\tau$ be a sequence of independent RVs $X_0$, $X_1$, $X_2$, $\cdots$ 
%{\bf [add superscript $\tau$ to them ]  JFM: maybe not} 
that each has a single-step random walk distribution.
When necessary, we call $\tau$ a {\it strict} random walk sequence to emphasize the (strict) independence among its steps.
% {\bf[delete?] and to highlight its difference with  
%a random walk (sequence) whose steps are strongly correlated. } 
Let $q$ and $s$ be two nonnegative integers such that $q \le s$.  
We define $S^{\tau}[q, s)$ as the $(s-q)$-step random walk $X_q+ X_{q+1} + \cdots + X_{s-1}$.  
Clearly, $S^{\tau}[q, s)$ is also a range-sum, with the underlying RVs being the sequence $\tau$.  
For notation convenience in the following, we also define the value of $S^{\tau}[s, q)$ as $-S^{\tau}[q, s)$.

In RW-LSH, the raw hash value function $f(\cdot)$ is parameterized by a vector of $m$ (which is also the dimension of the dataset $\mathcal{D}$) 
such strict random walk sequences $\vec{\bm{\tau}} = \langle \tau_1, \tau_2, \cdots, \tau_m \rangle$ that 
are  independent.
%Each $\tau_j$ is a sequence of single-step random walks that are mutually independent. 
%i.i.d. random variables, each of which takes value $1$ or $-1$ with equal probability $1/2$;  the value of each random variable is fixed 
%once it is generated. %, just as the computational model in \autoref{sec:overview}.  
%\textbf{In the sequel, we refer to such a random walk with mutually independent steps as a ``real'' random walk, in contrast to other instances that does not guarantee mutual %independent steps.}
Given a data point $\vec{\mathbf{s}} = \langle s_1, s_2, \cdots, s_m \rangle$, the raw hash value $f(\vec{\mathbf{s}})$ is defined as $\sum_{j=1}^m S^{\tau_j}[0, s_j)$.
In other words, $f(\vec{\mathbf{s}})$ is the result of randomly walking $s_1$ steps along sequence $\tau_1$, $s_2$ steps along $\tau_2$, $\cdots$, and $s_m$ steps along $\tau_m$.
RW-LSH requires that each $s_j$, $j = 1, 2,\cdots, m$, be a nonnegative even integer.  

%This requirement is imposed on all data points in $\mathcal{D}$  
%and all query points, to guarantee a monotonocity condition that, as we will explain shortly, qualifies a hash function family as LSH.  

We now fix a query point $\vec{\mathbf{q}}$ and a point $\vec{\mathbf{s}}$ in the dataset $\mathcal{D}$.  
We now state some facts that will be used both next and soon {\color{red} in~\autoref{sec:grwlsh}}.
Let $d_1$ be the $L_1$ distance between $\vec{\mathbf{q}}$ and $\vec{\mathbf{s}}$, that is, $d_1 = \sum_{j=1}^m |s_j-q_j|$.
%$d_1$ is a nonnegative integer since every $s_j$ and $q_j$ is.
%The performance of LSH heavily relies on the distribution of 
Then, $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})= \sum_{j=1}^m\left(S^{\tau_j}[0, s_j) -S^{\tau_j}[0, q_j) \right) =  \sum_{j=1}^mS^{\tau_j}[q_j, s_j)$~\cite{mprwlsh}. 
%Here, we have to clarify a subtle issue on notation. We have
%defined the range-sum $S^{\tau_j}[q_j, s_j)$ only when $q_j\leq s_j$, but it might be $q_j > s_j$, in which case we define $S^{\tau_j}[q_j, s_j) \triangleq -S^{\tau_j}[s_j, q_j)$.
%Since $f(\mathbf{s})  - f(\mathbf{q})$  .
%the random walks   $\langle \tau_1, \tau_2, \cdots, \tau_m \rangle$ are mutually independent, and because$f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$ has the same distribution as a  
%each   has the distribution of $d_1$-step random walk, because it is the sum of $m$ independent range-sums,
Note that each range-sum $S^{\tau_j}[q_j, s_j)$ has the distribution of a $|s_j - q_j|$-step random walk 
whether $q_j\leq s_j$ or $q_j> s_j$, since (the pdf of) every underlying single-step random walk is symmetric about $0$.
Since the random walks $S^{\tau_j}[q_j, s_j)$, $j = 1, 2, \cdots, m$, are independent (as they are along independent sequences), $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$
has the distribution of a $d_1$-step random walk, and hence is parameterized only by  $d_1$.
When $d_1$ is not small (say when $d_1 > 25$), this distribution can be closely approximated as $\mathcal{N}(0, d_1)$.
It has been shown in~\cite{mprwlsh} that this distribution being approximately Gaussian leads to every nice property of RW-LSH and its multi-probe 
extension MP-RW-LSH.

%highly efficient (w.r.t. query time) and
%effective (w.r.t. query accuracy).

 %(thanks to sin$|q_j - s_j|$-step random walk gle-step random walk has a symmetric distribution about 0).the number of steps
% Here we need to use a property of  (and the same for Gaussian distribution $X$): and, it because, the distribution of the range-sum of $|s_j-q_j|$ i.i.d. steps,
 %$S^{\tau_j}[s_j, q_j)$ is symmetric about $0$, or in other words $S^{\tau_j}[s_j, q_j)$ and $-S^{\tau_j}[s_j, q_j)$ have the same distribution, because
%the underlying RV $X$ at each step is symmetric about $0$.

%[JFM] Recall that the performance of (standard or multi-probe) LSH relies on the distribution of 

\begin{comment}
Now we are ready to derive the pdf of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$.

 which we already know is the sum of $m$ independent range-sums $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality), so it is important that each $S^{\tau}[q, s)$ is the range-sum of a \emph{strict} random walk. Under this condition,  $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$  is a strict random walk of $d_1$ i.i.d. steps, which is  parameterized only by  $d_1$.
When $d_1$ is not small, the distribution of a $d_1$-step random walk can be very closely approximated as the Gaussian distribution $\mathcal{N}(0, d_1)$.
It has been shown in~\cite{mprwlsh} that this Gaussian distribution alone makes MP-RW-LSH highly efficient (w.r.t. query time) and
effective (w.r.t. query accuracy).


%It is not hard to show that , is a  this $d_1$-step random walk.  Therefore,  , which is JFM] Since  if the random walks are strict, and in general relies onthe distribution of each range-sum .[], $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$ is a deterministic function of $d_1$


[duplicated] When $d_1$ is not small, the distribution of $d_1$-step random walk can be very closely approximated as the Gaussian distribution $\mathcal{N}(0, d_1)$.
It has been shown in~\cite{mprwlsh} that this Gaussian distribution alone that makes MP-RW-LSH highly efficient (w.r.t. query time) and
effective (w.r.t. query accuracy).
It is not hard to show that $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$, the marginal 
(collision) probability for $\vec{\mathbf{s}}$ to have the same LSH value (by the LSH function $g()$) as the query point $\vec{\mathbf{q}}$, is a (deterministic) linear functional of the pdf of this $d_1$-step random walk.  Therefore, the performance guarantee of LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality), which is a deterministic function of $d_1$ (parameterized by $W$ used  {\color{red}in $g(\vec{\mathbf{s}})$ }) if the random walks are strict.
\end{comment}

%(the total number of $f(\cdot)$ functions)as large as hundreds to

Recall that 
In the MP-RW-LSH scheme, given a query point $\vec{\mathbf{q}}= \langle q_1, q_2, \cdots, q_m \rangle$, we need to compute the raw hash value $f(\vec{\mathbf{q}}) 
= \sum_{j=1}^m S^{\tau_j}[0, q_j)$
for $L M$ ($L$ hash tables each using a vector 
of $M$ hash functions) such ($f$)'s.
Computing these range-sums one (random walk) step at a time is a relatively computationally heavy task, since
%is to compute, given a query point $\vec{\mathbf{q}}= \langle q_1, q_2, \cdots, q_m \rangle$,
%$L M$ ($L$ hash tables each using a vector 
%of $M$ hash functions) such raw hash values of $\vec{\mathbf{q}}$.  
although each step takes only nanoseconds to compute, there
are simply too many of them:
There are a total of $O(LMmU)$ steps, where $LM$  is typically in hundreds, 
the data dimension $m$ can be in thousands, and the maximum possible number of steps $U$ to walk along 
each random walk sequence $\tau$ can be hundreds of thousands.   As a result, it is not uncommon for $LMmU$ to be on the
order of $10^{10}$ or $10^{11}$.  This translates into tens of seconds of or minutes of computation time just for the raw hash values
of $\vec{\mathbf{q}}$.  In contrast, the rest of the ANNS query can often be done in tens of milliseconds.  
To reduce the time of computing these range-sums, RW-LSH precomputes and stores all $S^{\tau_j}[0, q_j)$ values for $q_j = 0, 1, 2,\cdots, U$ and for each random walk 
sequence $\tau_j$.  This reduces the time complexity to $O(LMm)$ but bloats the total size of pre-computation tables to $O(LMmU)$, which can translate into 
tens of gigabytes of storage as will be shown in~\autoref{sec:eva}.
%The ERS solutions that we will describe soon achieve the better of both worlds: It does not need precomputed tables, and the complexities in both space and evaluation time are as low as $O(LMm\log U)$.
% for each range-sum $S^{\tau}[0, q)$ achieves
\begin{comment}
To reduce the time of evaluating $f(\mathbf{s})$, the baseline solution of RW-LSH precomputes and stores each  $S^{\tau_j}[0, s_j)$ for $t = 2, 4, 6, \cdots, U_j$ where $U_j$ is the maximum possible (even) 
value for the $j^{th}$ coordinate of a data point.  For any random walk $\tau_j$, the baseline RW-LSH needs $U_j$ bytes for storing the precomputed table. Although
the storage cost of each precomputed table, which is roughly $O(mMU)$, supposing $U$ is the maximum value among $U_j$, is small relative to the size of each hash table, which is $O(n_d)$ and  $n_d$ is the size of the dataset, for large datasets, this cost can increase the total index size by several hundred times, for some smaller datasets where both $m$ and $U_j$ are very large (relative to the dataset size), 
as we will show in~\autoref{sec:eva}. 
\end{comment}

%We will explain shortly why this assumption is not 
%overly restrictive for real-world applications. 




%To reduce the storage cost of precomputed tables, the authors of \cite{mprwlsh} proposes ``long jump'', which reduces the storage cost by $32l$ times by paying $l$ CPU instructions for evaluating each range-sum $S^{\tau_j}[0, t)$. Even with this solution, the product of space and time complexities of RW-LSH is still $O(U_j)$ for each random walk, which is not scalable for future databases where $U_j$ might be gigantic.

%efficient range-summable (ERS) algorithms  to save the space of the precompute table
% ERS solutions, which only takes a small space and poly-logarithmic time. We can indeed use dyadic simulation to implement RW-LSH by generating range-summable single-step random walks , but %generate , but a better solution is to generate Gaussian random variables instead, because the latter can be  since it does not require rejection sampling. In BM-LSH, by changing the distribution of each step from a single-step random walk to a standard Gaussian random variable, we reformulate the random walk in RW-LSH to a discrete time Brownian motion. This reformulation is justified because a random walk is statistically close to a Brownian motion when $n$ (the number of steps) is large.
 

 %Since the evaluation of RW-LSH resolves to the ERS problem, 
 %Readers may wonder if
%{\bf no BCH3 anymore} 
We have considered whether EH3~\cite{feigenbaum}, an ERS scheme for single-step random walks, can be used to generate these range-sums for RW-LSH.  
The answer is ``no'' for the following reason.
  %One possible option is  which is shown by~\cite{rusu-jour} as the fastest range-summable scheme that has both theoretical guarantee (approximate $4$-wise independence) and good empirical performance (when estimating the size of joins). However, we show that EH3 is not very suitable for ANNS-$L_1$, for the following reasons.or BCH3~\cite{rusu-jour}
%   Recall that the efficacy of RW-LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ to be of a strict random walk.
  Although every underlying RV generated by EH3 has the  %EH3 scheme in \etal{Feigenbaum}~\cite{feigenbaum} generates range-summable random variables whosebe used to and BCH3of   matches that of
  marginal distribution of a single-step random walk, these %is highly ordered (deterministic)  (as required they only preserves the three-wise independence among  andir generated random variables
RVs are strongly correlated, since as explained earlier EH3 achieves ERS by systematically destroying all independence beyond $4$-wise among the underlying RVs.  
Hence the resulting range-sum $S^\tau[q, s)$ (where $\tau$ is generated by EH3)
%guaranteed to have the same standard deviation as those from an authentic 
%random walk, they may structure when more than three consecutive random variables are concerned. generated are  Thereforefollow a very different distribution than that of
behave very differently from a $(s - q)$-step random walk. %For example, when $[q, s)$ is a dyadic interval of width $2^l$ 
%{\bf JFM: I think $l$ is best. (DO WE WANT TO USE l here?)}, %the range-sum $S^\tau[q, s)$ generated by BCH3 is equal to $0$ with probability $1-2^{-l}$, 
%and has absolute value $2^l$ with probability $2^{-l}$~\cite{rusu-jour}.
%This distortion seriously impacts the distribution of $f(\mathbf{s})  - f(\mathbf{q})$ and the accuracy of RW-LSH.
%EH3 has a slightly better distribution of range-sums than BCH3 that is no longer 0 with high probability, but that is still far from that of a strict random walk.
%Although EH3 has a slightly stronger guarantee than BCH3 of approximate four-wise independence, so it has theoretical guarantees in the accuracy of estimating the $L_2$ moment in data streams in its proposed application, but it suffers from the same problem as above. %the generated range-sums still follow a very different distribution from
% is, its detailed distribution may be very different from the latter.$S^{\tau}[0, 10^6)$ 
For example, when $[q, s)$ is a dyadic interval and  $s - q = 4^l$, the range-sum $S^\tau[q, s)$ 
%generated by EH3 
takes values $2^l$ and $-2^l$ each with probability 1/2.
%follows uniform distribution in $\{2^l, -2^l\}$~\cite{rusu-jour}, so its absolute value is always $2^l$! 

\begin{comment}
\autoref{fig:distcomp} shows another example in which $[a, b)$ is  $[0, 10^6)$, which is not a dyadic interval. The histogram at the top is plotted from one million range-sums $S^{\tau}[0, 10^6)$ generated from EH3 with different seeds, and that at the bottom is from %one million range-sums of the same range from , which
a ``real'' random walk with empirically independent steps is generated by the built-in \texttt{mt19937} PRNG (not range-summable) in C++.%, and plot its distribution histogram at the top of \autoref{fig:distcomp}. at the bottom
%plot the histogram of the range-sum  generated from EH3 with one million different seeds  from  (not range-summable) 
%As a reference, we also plot the histogram of $S^{\tau}[0, 10^6)$ in 
 \begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{figures/histogram.eps}
	\caption{Distribution of generated random walks (Y axis normalized to probability density).}\label{fig:distcomp}
\end{figure}
From \autoref{fig:distcomp}, the distribution of range-sums generated by EH3 is far from that of the ``real'' random walk below, but concentrates at some special points near $1000$ (its standard deviation) and $-1000$. 
\end{comment}
%In contrast, the distribution of the range-sums generated by dyadic simulation % and of the independent non-range-summable random walk are distributed
%is close to the reference Gaussian distribution. This shows dyadic simulation is more suitable to ANN applications where the distribution of range-sums is crucial to the performance.
%In an even more extreme example, 
%Therefore, the performance of applying EH3 to MP-RW-LSH leads to unstable performance and significant degradation for some special queries on which the distribution of the produced range-sums is far from that of random walks. This will be illustrated by simulations in \autoref{sec:feigen_sim}.

 %preserves the independence between %different steps of the Brownian motion with the use of $O(\log U)$ two-wise independent hash functions (to be explained in ??) %if a two-wise independent hash function is used on each level of the simulation tree (to be explained later), 
%, so it is better suited for this application. of this distribution onof the distribution of range-sums , corresponding to recalls changes with $d_1$


%It has been shown in~\cite{stablelsh} that the performance guarantee of standard 
A key metric for measuring the quality of any LSH function family is $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$, the 
(collision) probability for $\vec{\mathbf{s}}$ to have the same LSH value (by the LSH function $g(\cdot)$) as the query point $\vec{\mathbf{q}}$.
%(so that $\vec{\mathbf{s}}$ can be found by the ANNS query in case it is a nearest neighbor of $\vec{\mathbf{q}}$).
In RW-LSH, this probability is a (deterministic) linear functional of the pdf of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}}) = \sum_{j=1}^mS^{\tau_j}[q_j, s_j)$.
%It as shown in~\cite{} that this pdf leads to virtually every nice property of RW-LSH.
% can be derived from the pdf of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$.
%(parameterized by $W$ {\color{red} used in $g(\vec{\mathbf{s}})$}). For a similar reason, the performance guarantee of multi-probe LSH also relies on the distribution of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$~\cite{mprwlsh}.
We now study how the use of EH3 for generating the sequences $\tau_j$, $j = 1,2, \cdots, m$, impacts 
%the damaging effect of this strong correlation among the random walk steps on 
the collision probability $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$ by distorting the range sums $S^{\tau_j}[q_j, s_j)$, $j=1,2, \cdots, m$.
We do so by zooming in on its damaging effect on a single sequence $\tau_1$ as follows:
%To isolate the effect of a single EH3-generated random walk sequence on the corresponding range sum, 
%$S^\tau[q, s)$ affects the collision probability, we now place further restrictions on these two points while keeping them $d_1$ apart in $L_1$ distance.
We let $\vec{\mathbf{q}} = \vec{\mathbf{s}}$ in every coordinate except the first, where $s_1 = 0$ and $q_1 = D$, so that $d_1 =  \sum_{j=1}^m |s_j-q_j| = D$.  
This way the value $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}}) = S^{\tau_1}[0, s_1)$, and hence the collision probability, is affected by only $\tau_1$.
%When the single-step random walks in the sequence $\tau_1$ is  independent,
%$f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}}) $ is a strict random walk with $d$ steps.  

In \autoref{fig:coll_prob}, we compare this collision probability ($y$-axis), which is a function of $D$ ($x$-axis), in two cases:  (1) \emph{original},
when $\tau_1$ is a strict random walk;  (2) \emph{EH3-augmented}, when $\tau_1$ is generated by EH3.
In case (1), this probability is monotonically decreasing as $D$ increases.
This monotonicity property has been widely used as a litmus test for an ``aspiring'' LSH function family~\cite{Indyk_ANN_1998}.
%qualifying requirement 
% for a (hash) function family to become a legitimate LSH function family [?] {\bf talk with Huayi}.
In contrast, in case (2), the collision probability jumps up and down when $D$ becomes larger.
%The obvious oscillation of the blue line in \autoref{fig:coll_prob} shows that the distortion of the distribution %of range-sums by EH3 shown in \autoref{fig:distcomp} against the ideal case with independent steps. 
%This phenomenon is extreme
This behavior automatically disqualifies the ``EH3-augmented'' RW-LSH, as an LSH function family.  
Furthermore, when the distance $D$ between \SI{16000}{} and \SI{17000}{} happens to cause the collision probability (curve) to fall into a ``valley'', 
%the collision probability becomes close to 0.
%As a result, 
the (success) probability for $\vec{\mathbf{q}}$ to be hashed into the epicenter bucket and be found by the ANNS query becomes very close to 0.
In this case, the query accuracy can be very low, 
%It can be shown that this probability remains low 
even when multi-probe is used, as we will show next to some extent.  
%has a significant influence on the collision probability  against ideal RW-LSH, especially in the ``valleys'' in which it is impossible to find the data point in the epicenter bucket! 
%(The first two valleys occur at distance $16384$ and $49152$.) 
%As a result, it is difficult to guarantee robust performance when EH3 is used to implement RW-LSH.  

\begin{comment}
[added]
To further verify 
We have evaluated the ANNS-$L_1$ query accuracy of MP-RW-LSH using EH3 on the Enron dataset (see ???), when the distance of the nearest neighbor to a query point
We have found that its recall value is an order of and that of MP-RW-LSH using precomputed tables.
show 
%tune the parameter for the ANNS with EH3
%which may lead to significant performance degradation in some bad cases. 


%[maybe still useful]
%When the single-step random walks in the sequence $\tau_1$ is mutually indepdent,
%$f(...) - f(...)$ is an authentic random walk with $d$ steps.  


[duplicate]
When the single-step random walks in the sequence $\tau_1$ is mutually indepdent,
$f(...) - f(...)$ is an authentic random walk with $d$ steps.  






[duplicate]
it is the sum of $m$ independent range-sums, and the range-sum on the $j^{th}$ coordinate is a $|q_j - s_j|$-step random walk. Therefore, the performance guarantee of LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality).

[mostly spent]
hashed by a single LSH function $g$.  
in the following (overly simple) simulation, we set the LSH bucket width $W=122$ (same as the simulation below) and regard the range-sum $S^\tau[0, d)$ as the difference of the raw hash values $f(\mathbf{s}) - f(\mathbf{q})$, corresponding to the case where %$m=1$, $\mathbf{s}=\langle 0\rangle$, and $\mathbf{q}=\langle d\rangle$. 
$\mathbf{s}$ and $\mathbf{q}$ differ only at the $j^{th}$ coordinate, with $s_j=0$ and $q_j=d$. We plot the frequency of hash collisions (\ie $g(\mathbf{s}) = g(\mathbf{q})$) in one million runs for each $d$ on a wide range in \autoref{fig:coll_prob}, against ideal RW-LSH. %(directly computed from the property that $f(\mat

[duplicate]In this section, we show why existing range-summable generation schemes, such as EH3~\cite{feigenbaum}, is not suitable for ANNS.  In particular, we show by simulation that the dependency between the components of the EH3 scheme interferes the distribution of the difference of raw hash values $f(\mathbf{s})  - f(\mathbf{q})$, making it far from Gaussian.

\end{comment}
% samplesThe distribution of the final position shold$To compare the distribution of range-sums, we generate $1$ million range-sums of 1 million standard gaussian random variables from existing range-summable sketches for $L_1$ \cite{feigenbaum} and dyadic simulation and plot the histograms as \autoref{fig:distcomp} against the distribution of one-million step random walks and reference Gaussian $\mathcal{N}(0, 10^6)$. Ideally, the range-sums should follow Gaussian distribution with mean $0$ and standard deviation $1000$ (bottom figure). 



%[maybe still useful]
%it is the sum of $m$ independent range-sums, and the range-sum on the $j^{th}$ coordinate is a $|q_j - s_j|$-step random walk. Therefore, the performance guarantee of LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality).

%[mostly spent]
%hashed by a single LSH function $g$.  
%in the following (overly simple) simulation, we set the LSH bucket width $W=122$ (same as the simulation below) and regard the range-sum $S^\tau[0, d)$ as the difference of the raw hash values $f(\mathbf{s}) - f(\mathbf{q})$, corresponding to the case where %$m=1$, $\mathbf{s}=\langle 0\rangle$, and $\mathbf{q}=\langle d\rangle$. 
%$\mathbf{s}$ and $\mathbf{q}$ differ only at the $j^{th}$ coordinate, with $s_j=0$ and $q_j=d$. We plot the frequency of hash collisions (\ie $g(\mathbf{s}) = g(\mathbf{q})$) in one million runs for each $d$ on a wide range in \autoref{fig:coll_prob}, against ideal RW-LSH. %(directly computed from the property that $f(\mathbf{s}) - f(\mathbf{q})$ is $\mathcal{N}(0, d)$, the approximation of a $d$-step random walk).
%especially the collision probability (of having the same hash value) of RW-LSH. We draw   with a varying number of steps generated by EH3 similarly to the simulation above. % The following simulation provides a more intuitive view on how the distribution of the random walk (of the difference of raw hash values) influence the performance of ANNS. 
%In this   %fix the query point at $0$, and increase the first coordinate of the nearest neighbor while fixing the other coordinates at $0$.  (equivalent to the case when data and query points are one-dimensional, the query points is $0$, and the data point $d$ is moving).
%\autoref{fig:coll_prob} shows the  of EH3 against 
%

\begin{figure}[!ht]
	\centering
	\caption{Comparison of collision probabilities, $W=122$.}\label{fig:coll_prob}
	\includegraphics[width=0.51\textwidth]{figures/collprob.eps}
\end{figure}

% Figure.\, \ref{fig:coll_prob} gives an example in which the dependence of ETH3 significantly affect the collision probability (of finding a nearest neighbor in the same bucket). %Therefore, the generated sequence is not a real random walk, so $f(\mathbf{s}) - f(\mathbf{t})$ will not always converge to Gaussian distribution as required by the LSH function and is very sensitive to input. 
%We will show in ??? that the range-summable ``random-walk'' scheme by~\cite{feigenbaum} is not suitable for ANNS-$L_1$.


%\textbf{The probability of $|g(\mathbf{s}) - g(\mathbf{q})|=1$ also oscillates in a similar manner, so the probability of finding $\mathbf{s}$ even with multi-probe used is not stable. Note that the numbers in \autoref{fig:coll_prob} do not directly explain the next experiment, because the collision probability depends on the nearest neighbor $\mathbf{s}$, which is no longer $\langle 0\rangle$ in real datasets. }

%In comparison, dyadic simulation can generate range-summable random variables that are nearly perfectly independent, so it is better suited for the ANNS-$L_1$ application. We can indeed use dyadic simulation to generate empirically independent range-summable single-step random walks as in \autoref{sec:randw}, but a better solution is to generate Gaussian random variables instead, because the latter can be generated four times as fast as random walks since it does not require rejection sampling. In BM-LSH, by changing the distribution of each step from a single-step random walk to a standard Gaussian random variable, we reformulate the random walk in RW-LSH to a discrete time Brownian motion. This reformulation is justified because a random walk is statistically close to a Brownian motion when $n$ (the number of steps) is large.

%Since the range-sum of  we may use (rounded) Gaussian distribution approximation in rejection sampling. However, we think it might be better to just take the easy step: to use the range-summable scheme for Gaussian distribution in this application. For this purpose
%We reformulate RW-LSH to a closely related stochastic process, a discrete time Brownian motion. 







\begin{comment}
\textcolor{teal}{
How to efficiently search for similarity on large (large element number, high dimension) databases? 
(definition of c-ANN)
We focus on $l_1$ distance, because it is important (robust to outliers) and underexplored.
A thread of high performance ANN by Locality Sensitive Hashing (LSH) indices. For similar pairs of (data and query) points that are closer under $l_1$ metric (than a certain threshold), the LSH function maps them to the same bucket with higher probability. But for dissimilar pairs of points, this LSH function maps them to the same bucket with very low probability.(definition of LSH)
% One basic LSH is constructed with stable distribution, which is generic for $l_p$ distance with $1\leq p\leq 2$. 
In addition to the ``hard decoding" schemes that works only when the data and query are in the same bucket, researchers have put forward ``soft decoding" schemes, such as SRS and multiprobe \cite{multiprobe}, which also search nearby buckets for data candidates. These schemes achieve higher memory efficiency, but they require the distribution of the difference of hash values $f(\mathbf{x})-f(\mathbf{q})$ to be concentrated so that near neighbors will always be hashed close to the query.  However, the only? $l_1$ LSH function $f$ till now is based on stable distributions \cite{stablelsh}, under which the distribution of $f(\mathbf{x})-f(\mathbf{q})$ follows the corresponding stable distribution for $l_p$ norm with $1\leq p\leq 2$. Although Gaussian distribution (stable for $l_2$) is nicely concentrated, Cauchy distribution (stable for $l_1$) has a heavy tail. As a result, a large proportion of data points may be hashed far away from the query point under the Cauchy scheme, which is why multiprobing performs well on $l_2$ but is less effective on $l_1$. 
}\end{comment}
 
% \subsection{Comparison with EH3 Scheme}\label{sec:feigen_sim}
 %However, no existing range-summable scheme maintains the distribution of the range-sum as perfect Gaussian as required by the LSH propery (and multiprobing). 
%[duplicate]In this section, we show why existing range-summable generation schemes, such as EH3~\cite{feigenbaum}, is not suitable for ANNS.  In particular, we show by simulation that the dependency between the components of the EH3 scheme interferes the distribution of the difference of raw hash values $f(\mathbf{s})  - f(\mathbf{q})$, making it far from Gaussian.
 
%[duplicate]At first, we compare the distribution of generated range-sums from simulation. In each run of the simulation, we generate the final position of a random walk or a Brownian motion with the following three schemes. \textbf{Sequence of schemes?} The first one is dyadic simulation for standard Gaussian target distribution, which generates the final position of a Brownian motion $S^{\zeta}[0, 10^6)$. The second scheme is EH3, which generates the final position of a ``random walk'' $S^{\tau}[0, 10^6)$ with the same number of steps. The third scheme is a ``real'' random walk $S^{\tau}[0, 10^6)$ from empirically independently steps (not range-summable) generated by the built-in \texttt{mt19937} PRNG in C++. %The third scheme is to use range-summable  to generate a random walk for the same $\tau(t)$ at $t=10^6$. 
%For all three schemes above, we draw the histogram (normalized to probability density) from one million independent runs and show at the bottom of \autoref{fig:distcomp} the reference Gaussian distribution $\mathcal{N}(0, 10^6)$ , %draw the histogram for the distribution of the final position, 
%to which all of the top three figures should converge. %is the distribution should all converge to with mean $0$ and standard deviation $1000$ (bottom figure). 

% samplesThe distribution of the final position shold$To compare the distribution of range-sums, we generate $1$ million range-sums of 1 million standard gaussian random variables from existing range-summable sketches for $L_1$ \cite{feigenbaum} and dyadic simulation and plot the histograms as \autoref{fig:distcomp} against the distribution of one-million step random walks and reference Gaussian $\mathcal{N}(0, 10^6)$. Ideally, the range-sums should follow Gaussian distribution with mean $0$ and standard deviation $1000$ (bottom figure). 
 

 
%[duplicate] From \autoref{fig:distcomp}, the distribution of range-sums generated by EH3 is far from that of the ``real'' random walk, but concentrates at some special points near $\pm1000$ (in order to have $0$ mean and $1000$ standard deviation). In contrast, the distribution of the range-sums generated by dyadic simulation % and of the independent non-range-summable random walk are distributed
%is close to the reference Gaussian distribution. This shows dyadic simulation is more suitable to ANN applications where the distribution of range-sums is crucial to the performance.
% \textcolor{teal}{However, no existing range-summable scheme maintains the distribution of the range-sum as perfect Gaussian as required by the LSH propery (and multiprobing). For example, the scheme in \cite{feigenbaum} can only guarantee approximate four-wise independence, which sacrifices all higher orders of independence in return for range-summability, and although \cite{rusu-jour} described several range-summable schemes with a higher degree of independence, the time complexity of these schemes is too high. }%Four-wise independence is sufficient for bounding the variance of the estimator in the streaming application, but for ANN, 
%To intuitively show  the impact of this distribution on the performance of ANNS, especially the collision probability (of having the same hash value) of RW-LSH. We draw \autoref{fig:coll_prob}  with a varying number of steps generated by EH3 similarly to the simulation above. % The following simulation provides a more intuitive view on how the distribution of the random walk (of the difference of raw hash values) influence the performance of ANNS. 
%In this (overly simple) simulation, we set the LSH bucket width $W=100$ and regard the range-sum $S^\tau[0, d)$ as the difference of the raw hash values $f(s) - f(q)$, corresponding to the case where $m=1$ and $s=\langle 0\rangle$. %fix the query point at $0$, and increase the first coordinate of the nearest neighbor while fixing the other coordinates at $0$.  (equivalent to the case when data and query points are one-dimensional, the query points is $0$, and the data point $d$ is moving).
%\autoref{fig:coll_prob} shows the ratio of hash collisions in one million runs for each $d$ of EH3 against ideal RW-LSH (directly computed from the property that $f(s) - f(q)$ is $\mathcal{N}(0, d)$, the approximation of a $d$-step random walk).
 %\begin{figure}
 %	\centering
 %	\includegraphics[width=0.48\textwidth]{figures/coll_prob_100.png}
 %	\caption{Comparison of collision probabilities.}\label{fig:coll_prob}
 %\end{figure}
% Figure.\, \ref{fig:coll_prob} gives an example in which the dependence of ETH3 significantly affect the collision probability (of finding a nearest neighbor in the same bucket). %Therefore, the generated sequence is not a real random walk, so $f(\mathbf{s}) - f(\mathbf{t})$ will not always converge to Gaussian distribution as required by the LSH function and is very sensitive to input. 
 %We will show in ??? that the range-summable ``random-walk'' scheme by~\cite{feigenbaum} is not suitable for ANNS-$L_1$.
%The obvious oscillation of the blue line in \autoref{fig:coll_prob} shows that the distortion of the distribution of range-sums by EH3 shown in \autoref{fig:distcomp} has a significant influence on the collision probability  of RW-LSH against the ideal case with independent steps. This phenomenon is extreme in the ``valleys'' in which it is impossible to find the data point in the epicenter bucket! (The first two valleys occur at distance $16384$ and $49152$.) As a result, it is difficult to guarantee consistent performance when EH3 is used to implement RW-LSH, %tune the parameter for the ANNS with EH3
%which may lead to significant performance degradation in some bad cases.
%\subsection{Comparison between Feigenbaum and Dyadic}
% \begin{table}[!htb]
% 	\caption{Comparison between MP-BM-LSH and MP-RW-LSH(EH3) on synthetic dataset. $M=7$, $W=100$}\label{tab:feigen_vs_dyadic}
% 	\centering
% 	\begin{tabular} {@{}c c c c c@{}}
% 		\specialrule{.1em}{.05em}{.05em} 
% 	\multirow{2}{*}{$L$} & \multicolumn{2}{c}{MP-BM-LSH}  & \multicolumn{2}{c}{MP-RW-LSH (EH3)} \\\cline{2-5}
% 	& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
% 	6  & 0.0820 & 1.0878 & 0.0065 & 0.9088\\
% 	10 & 0.1287 & 1.7429 & 0.0129 & 1.4614  \\
% 	20 & 0.2402 & 3.3721 & 0.0228 & 2.8278  \\
% 	40 & 0.4201 & 6.7092 & 0.0442 & 5.5682\\
% 		\specialrule{.1em}{.05em}{.05em} 
% 	\end{tabular}
% \end{table} 
\begin{comment}
\begin{table}[!htb]
	\caption{Comparison between MP-BM-LSH and MP-RW-LSH(EH3) on synthetic dataset. $M=7$, $W=100$}\label{tab:feigen_vs_dyadic}
	\centering
	\begin{tabular} {@{}c c c c c@{}}
		\specialrule{.1em}{.05em}{.05em} 
		\multirow{2}{*}{$L$} & \multicolumn{2}{c}{MP-BM-LSH}  & \multicolumn{2}{c}{MP-RW-LSH (EH3)} \\\cline{2-5}
		& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
		6  & 0.0820 & 1.03+0.06 & 0.0065 & 0.85+0.06\\
		10 & 0.1287 & 1.65+0.10 & 0.0129 & 1.37+0.10  \\
		20 & 0.2402 & 3.17+0.20 & 0.0228 & 2.64+0.19  \\
		40 & 0.4201 & 6.26+0.45 & 0.0442 & 5.18+0.40\\
		\specialrule{.1em}{.05em}{.05em} 
	\end{tabular}MP-RW-LSH (precomputed) and MP-RW-LSH (EH3) on synthetic Enron dataseComparison between two different MP-RW-LSH
\end{table}\end{comment}
\begin{table}[!htb]
\caption{Original vs EH3-augmented. }\label{tab:feigen_vs_dyadic_another}
\centering
%\begin{tabular} {@{}c c c c c@{}}
%\specialrule{.1em}{.05em}{.05em} 
%\multirow{2}{*}{$L$} & \multicolumn{2}{c}{Precomputed}  & \multicolumn{2}{c}{EH3} \\\cline{2-5}
%& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
%10 & 0.1111 & 2.64+2.42 & 0.0100 & 0.64+1.12  \\
%15 & 0.1647	& 4.09+4.98 & 0.0147 & 1.05+1.64 \\
%20 & 0.2080	& 4.70+8.21 & 0.0180 & 1.25+2.16  \\
%\specialrule{.1em}{.05em}{.05em} 
%\end{tabular}
\begin{tabular} {@{}c | c c c c@{}}
	\specialrule{.1em}{.05em}{.05em} 
	 \multicolumn{2}{c} {$L$ } & 10 & 15 & 20 \\
	\specialrule{.1em}{.05em}{.05em} 
	  \multirow{2}{*}{Recall} &original & 0.1111 & 0.1647 & 0.2080\\\cline{2-5}
 &EH3-augmented& 0.0100& 0.0147 & 0.0180	\\
	\specialrule{.1em}{.05em}{.05em} 
\end{tabular}
\end{table}  
% \begin{table}[!htb]
% 	\caption{Comparison results on Enron dataset with synthetic queries. }\label{tab:feigen_vs_dyadic_another}
% 	\centering
% 	\begin{tabular} {@{}c c c c c@{}}
% 		\specialrule{.1em}{.05em}{.05em} 
% 		\multirow{2}{*}{$d$ } & \multicolumn{2}{c}{Precomputed}  & \multicolumn{2}{c}{EH3} \\\cline{2-5}
% 		& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
% 		6400  & 0.5880 & 10.58+2.77 & 0.4321 & 6.41+1.01 \\
% 		8400 & 0.1709 & 6.68+2.35 & 0.1109 & 3.25+1.01  \\
% 		13300 & 0.0208	& 2.44+2.14 & 0.0019 & 0.65+1.01  \\
% 		16600 & 0.0084	& 1.33+2.10 & 0.0001 & 0.20+1.02 \\
% 		\specialrule{.1em}{.05em}{.05em} 
% 	\end{tabular}
% \end{table} 
% in the worst casethe Audio dataset (to define in \autoref{subsec:exp_set}). Each query is generated by conduct the following experiment in in the worst cases
%$M=9$, $W=122$between MP-GRW-LSH and MP-RW-LSH(EH3)

\begin{comment}
Description for varying distance: To show how the performance of EH3-based MP-RW-LSH degrades, we compare it  with the vanilla MP-RW-LSH with precomputed tables~\cite{mprwlsh}. %on the  dataset . 
In the experiments, we use Enron (see \autoref{tab:dataset-stats}) as the dataset $\mathcal{D}$, and generate \SI{10000} synthetic queries from the following procedure for each $d$. First, we randomly sample one point from the Enron database. Then, we generate the query point from randomly choosing one coordinate of the sampled data point and adding $d$ while keeping other coordinates unchanged, similar to the restriction above. %which is a variable parameter reflecting how far the query is from its neareat neighborroughly the position of the first ``valley'' in \autoref{fig:coll_prob}, to this coordinate value. MP-BM-LSH (from dyadic simulation) and MP-RW-LSH (from EH3) with different number of hash tables 
For different distance value $d$, the recalls and query times of both algorithms reported in~\autoref{tab:feigen_vs_dyadic} are averaged for these \SI{10000} queries.
We use the same index structure (hash tables) as in \autoref{sec:eva}, with the same set of parameters $M=9$, $T=100$, $W=122$. We show how recall and query time (written as $t_1+t_2$) change when  $d$ increases.\end{comment}

%As an example of the worst case, we generate the distance between the data and query points areplease refer to \autoref{subsec:ann-comp-algorithmsfor the meaning of these parameters)



%\textbf{Huayi Paragraph for the generation of synthetic dataset: \autoref{fig:distcomp} clearly shows that the success probability of EH3-based LSH is close to 0 for distance equal to 17600 when hash bucket width $W=100$. Based on this fact, we generate synthetic dataset where the distance of each query point to its corresponding nearest neighbor is 17600. More precisely, we first randomly sample one point from database. Then we generate the query point from randomly choosing one coordinate of the sampling point and adding 17600 on the coordinate value of this point. We use such generation process in order to achieve the similar success probability value as shown in \autoref{fig:distcomp}. We generate 1000 different query points and report the query performance of Feigenbaum and Dyadic on the synthetic dataset with different number of hash tables in~\autoref{tab:feigen_vs_dyadic}.}$M=9$, $W=122$index structure (hash tables) , with the same, which is roughly the position of the first ``valley'' in \autoref{fig:coll_prob},

We illustrate this ``fall into the valley'' effect by performing the following controlled ANNS-query experiment involving both 
the original and the  EH3-augmented MP-RW-LSH.  
%To show how the performances of EH3-based MP-RW-LSH (EH3-based for short in the sequel) degrades, we compare it  with the original MP-RW-LSH with precomputed tables~\cite{mprwlsh} (Precomputed for short).
In this experiment, we use Enron (see \autoref{tab:dataset-stats}) as the dataset $\mathcal{D}$ and generate \SI{10000}{} synthetic queries that target a ``fall'' distance
$D$ = \SI{13300}{} (the first ``valley'' shown \autoref{fig:coll_prob}).  
Each query is generated as follows.  First, we randomly sample a point $\vec{\mathbf{s}}$ from $\mathcal{D}$.  Then, we pick a dimension $j$ uniformly at
random (out of the $m$ dimensions), and set the query point $\vec{\mathbf{q}}$ such that $\vec{\mathbf{q}}$ is identical to $\vec{\mathbf{s}}$ in every dimension except the $j^{th}$, where $q_j = s_j + D$.
Note that despite our ``targeted push'', 
only a small percentage of query points actually ``fall into the valley'', because, even when $D$ is fixed, the value of an EH3-generated range-sum 
$S^{\tau_j}[s_j, s_j + D]$, and hence the shape of the corresponding collision probability curve (\autoref{fig:coll_prob} shows only that for $s_j = 0$), varies when $s_j$ varies (as 
it does in this experiment);  
hence we are not overly ``exaggerating'' EH3's damaging effect here.
%generate the query point from randomly choosing one coordinate of the sampled data point and adding \SI{13300}{} to this coordinate value while keeping other coordinates %unchanged, similar to the restriction above. 
For both the original and the EH3-augmented, we use the same set of parameters $M=9$, $T=100$, $W=122$ as in~\autoref{sec:eva}, and report their average 
recalls (over these \SI{10000}{} queries)
under the same set of $L$ (number of hash tables) values.
\autoref{tab:feigen_vs_dyadic_another} shows that recall values of the original are between $11.1$ and $11.6$ times larger than those of EH3-augmented. 

%Note that here the recalls are lower than those in~\autoref{sec:eva}, because $d$, the distance between the query point and its nearest neighbor is \SI{13300}{}, which corresponds with the ``valley'' in \autoref{fig:coll_prob}, are ??? times of those typical in ~\autoref{sec:eva}. Under such a large distance, the recalls of EH3-based is approximately equal to $0$ while Precomputed still have recalls around $0.1$. 

\begin{comment}
Therefore, the performance of EH3-based is not robust, even if its query times may be shorter than those of Precomputed.
{\bf JFM: I suggest removing ``query times'', because the story is distracting.}
For query efficiency, EH3-based has a shorter $t_1$ than Precomputed, because it hardly finds any candidate.  As we will shown later in \autoref{sec:eva}, we have found that $t_1$ is roughly linear to the number of candidates found in probing the buckets. Its $t_2$ is also shorter, because it is faster to compute a range-sum by EH3 in this case than to read from the precomputed table in DRAM.
\end{comment}

%\textbf{Original description:\autoref{tab:feigen_vs_dyadic_another} clearly shows that when $d=6400$, a typical distance for queries in the real dataset \autoref{sec:eva}, the recall of EH3-based is lower than that of vanilla MP-RW-LSH by 1.4. This difference becomes more pronounced when $d$ increases. For example, when $d=$\SI{13300}{}, vanilla MP-RW-LSH achieves recall $0.0208$, but recall value of EH3-based MP-RW-LSH is only $0.0019$, which is 10.9 times smaller than the recall value of vanilla MP-RW-LSH. This corresponds with the ``valley'' in \autoref{fig:coll_prob}, where success probability of EH3-based MP-RW-LSH is approximately equal to 0 where vanilla MP-RW-LSH still have success probability around 0.1. For query efficiency, EH3 has a shorter $t_1$ than vanilla, because it hardly finds any candidate. For example (\textbf{Huayi: As we will shown later in \autoref{sec:eva}}) we have found that $t_1$ is roughly linear to the number of candidates found in probing the buckets. Its $t_2$ is also shorter, because it is faster to compute a range-sum by EH3 in this case than to read from the precomputed table in DRAM.}

%\autoref{tab:feigen_vs_dyadic_another} clearly shows that, for the same number of hash tables, EH3 has a shorter $t_2$ than DST by a factor of $4.1$ to $4.9$, which is because its algorithm is simpler in using integer operations only and no transforms, and a shorter $t_1$ by a factor of $3.2$ to $4$, which is because it hardly finds any candidate. We have found that $t_1$ is roughly linear to the number of candidates found in probing the buckets. The $t_1$ of DST on the first row of  \autoref{tab:feigen_vs_dyadic_another} with that on the third column of \autoref{tab:perf} measured from normal queries, 

 %times that of EH3, the former can achieve much better accuracy ($9.1$ to $10.1$ times as high recall) than  the latter.
%$t_1$ is shorter for EH3, because it returns fewer candidates.
 
 %Under these schemes, the distribution of $f_{\mathbf{V}}(\mathbf{x})  - f_{\mathbf{V}}(\mathbf{q})$ is far from Gaussian, which directly degrades the performance. The GRW-LSH algorithm


\subsection{Our Solution: DST-based GRW-LSH}\label{sec:grwlsh}

%We can certainly solve 
Again we fix $\vec{\mathbf{s}}$ and $\vec{\mathbf{q}}$ that are $d_1$ apart in $L_1$ distance.
The ERS problem in RW-LSH can be cleanly solved using our RW-DST as follows.
Each DST instance (one for each random walk sequence) is generated using a different (cheap)  
$2$-wise independent hash function at each of the $\log_2 U$ levels.  This way, 
each range-sum $S^{\tau_j}[q_j, s_j)$, that is a part of $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}})$, is a strict $|s_j - q_j|$-step random walk according to \autoref{cor:stdist}, and hence $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}})$ is a
strict $|s_j - q_j|$-step random walk.   
Since the pdf of $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}})$ statistically defines an RW-LSH scheme, the RW-DST-augmented RW-LSH is statistically equivalent to the original RW-LSH.

\begin{comment}
to generate the underlying range sums.  
Since the behavior of RW-LSH is determined entirely by the pdf of 

 above, because by  \autoref{cor:stdist}, a hashing-based DST with cheap two-wise independent low-level hash functions guarantees that $S^\tau[q, s)$ follows the same distribution as a $|q - s|$-step strict random walk, which %is exactly what is needed by ANNS.
%In \autoref{sec:dsthash},  that a surprisingly cheap implementation of DST that uses  with two-wise independence 
%Therefore, by maintaining $m$ independent instances of such DSTs, one for each random walk $\tau$, we have an efficient DST-based implementation of RW-LSH that
%Therefore, we can evaluate $f(\mathbf{s})$ by generating the range-sum of each random walk $S^{\tau_j}[0, s_j)$ with the method described inn order to generate range-sums of single-step random walks that has the same distribution as ``real'' random walks,  and using . on the $j^{th}$ coordinate this DST uses t.I, which uses the definition of splits in \autoref{sec:randw} and l This leads to the following This implementation , because each of the range-sums $S^{\tau}[q, s)$ is a  random walk by.the DST-based GRW-LSH (defined below) is even better in thatand 
%does not need the precomputed tables and guarantees  the $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$ to be a strict$d_1$-step random walk, which 
is sufficient for all the theoretical efficacy guarantees of RW-LSH as we have shown above.
This is already a desirable solution, yet we will show that it is even better to replace RW-LSH with 
\end{comment}

We propose an even better solution called GRW-LSH ( walk LSH).
% that is based on our ERS-Gaussian solution.
A raw hash value function $f$ is defined in GRW-LSH in the same way as in RW-LSH, except each random walk sequence $\tau_j$ is replaced by 
a Gaussian random walk (GRW) sequence $\xi_j$.  In a GRW sequence, the underlying RVs are i.i.d. with standard Gaussian distribution instead.
%as just explained.  mutually independentin a $v$-step random walk
As a result, each $s_j$-step random walk along $\tau_j$ is replaced by an $s_j$-step GRW  along $\xi_j$.
% and the other definitions, such as $g(\vec{\mathbf{s}})$, remain the same.
This way, $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$, which as just explained has the distribution of a $d_1$-step strict random walk %and has a probability distribution very close to the Gaussian distribution $N(0, d_1)$
under RW-LSH, now has Gaussian distribution $\mathcal{N}(0, d_1)$ under GRW-LSH.
Since the former distribution is always statistically close to the latter distribution {\color{red} and especially so when $d_1$ is reasonably large
(say when $d_1 > 25$)}, GRW-LSH  is statistically very close to RW-LSH.
As a result, its multi-probe extension MP-GRW-LSH has nearly the 
same query efficacy as MP-RW-LSH, as will be shown in \autoref{sec:eva}.  

It is straightforward to implement (the step of hashing $\vec{\mathbf{q}}$) GRW-LSH:   Each range-sum $S^{\xi_j} [0, q_j)$ is computed using our Gaussian-DST.
As explained above, using a different
$2$-wise independent hash function at every level of a DST instance is enough to ensure statistical equivalence (between the original GRW-LSH and
the Gaussian-DST-augmented GRW-LSH);  but for all practical purposes, we will use wyhash functions instead.  
GRW-LSH is a better solution than RW-DST-augmented RW-LSH, since to compute a Gaussian range-sum is several times faster than to compute a random walk range-sum, as shown in \autoref{tab:perf}.

%Therefore, we focus on the DST-based efficient implementation of only GRW-LSH, which we simply refer to as GRW-LSH in the sequel, and we refer to the original scheme in~\cite{mprwlsh} with precomputed tables as RW-LSH. 

\begin{comment}

%replacing a $v$-step random walk (in RW-LSH) by a $v$-step(in GRW-LSH)ERS solution for 
The primary motivation for using Gaussian random walks  is that the it 
can be efficiently computed using our Gaussian-DSTs. 
Our measurements 
show that each dyadic split operation for Gaussian 
can be accomplished in a couple of nanoseconds.  Hence even when $v$ is as large as $2^{20}$, the $20$ dyadic splits involved to 
compute the $v$-step Gaussian random walk take a total of roughly \SI{95.1}{ns} to compute.  In comparison, in RW-LSH, even to read a precomputed value from the gigantic 
table (stored in DRAM) takes tens of nanoseconds.  Hence GRW-LSH usually affords faster LSH computation while paying zero storage cost for it.  
This said, we do not consider
GRW-LSH a separate contribution to the LSH literature, since it is conceptually very close to RW-LSH.  We consider it a contribution to the ERS literature as a novel application of 
our ERS-for-Gaussian solution.



%[to move with the closeness paragraph several paragraphs before]
%Since the latter is always statistically close to the former and especially so when $v$ is reasonably large
%(say when $v > 25$), the resulting GRW-LSH (... LSH) is statistically close to RW-LSH.  

We stress the difference between our GRW-LSH and the traditional GP(Gaussian projection)-LSH~\cite{Datar_LSH_2004}, which also uses Gaussian random variables, that GP-LSH  is suitable for querying on $L_2$ distance, but our GRW-LSH focuses on $L_1$ distance. In GP-LSH, the raw hash value $f(\mathbf{s})$ is defined as $\vec{\mathbf{s}}\cdot \vec{\bm{\eta}}$, where ``$\cdot$'' is the inner product (which is mathematically a {\it projection}) and $\vec{\bm{\eta}}=\langle \eta_1,\cdots, \eta_m\rangle$ is an $m$-dimensional i.i.d. standard Gaussian random vector (fixed after generation). The most stressed difference is that in GRW-LSH, the $j^{th}$ dimension contributes to $f(\mathbf{s})$ a $s_j$-step Gaussian random walk, which is the sum of $s_j$ i.i.d. standard Gaussian RVs, whereas in GP-LSH, it contributes $s_j\eta_j$, which is $s_j$ times a fixed Gaussian RV $\eta_j$. 
Therefore, for GP-LSH $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$ follows $\mathcal{N}(0, d_2^2)$, which reflects the $L_2$ distance between $\vec{\mathbf{s}}$ and $\vec{\mathbf{q}}$ instead of the $L_1$ distance.

\end{comment}


\begin{comment}
[duplicate]In \autoref{sec:dsthash}, we have shown that a surprisingly cheap implementation of DST that uses low-level hash functions with two-wise independence guarantees the same distribution of range-sums as a ``real'' random walk.
Therefore, by maintaining $m$ independent such DSTs, one for each random walk $\tau$, we have an efficient DST-based implementation of RW-LSH that
%Therefore, we can evaluate $f(\mathbf{s})$ by generating the range-sum of each random walk $S^{\tau_j}[0, s_j)$ with the method described inn order to generate range-sums of single-step random walks that has the same distribution as ``real'' random walks,  and using . on the $j^{th}$ coordinate this DST uses t.I, which uses the definition of splits in \autoref{sec:randw} and l This leads to the following This implementation 
does not need the precomputed tables and guarantees  the $f(\mathbf{s})  - f(\mathbf{q})$ to be a $d_1$-step random walk, because each of the range-sums $S^{\tau}[q, s)$ is a $|q - s|$-step random walk by \autoref{cor:stdist}.
%Obviously, we can avoid the precomputed table by directly generating the range-sum $S^{\tau}[0, t)$ of each random walk $\tau$ with dyadic simulation as . study the efficient implementation with dyadic simulation of only
This DST-based RW-LSH implementation may be useful in some applications that restrict the hash values to integers. However, we will show that the DST-based GRW-LSH (defined below) is even better in that it is faster and as accurate. 
As a result, we focus on the DST-based efficient implementation of only GRW-LSH, which we simply refer to as GRW-LSH in the sequel, and we refer to the original scheme in~\cite{mprwlsh} with precomputed tables as RW-LSH in the sequel. 


[duplicate] In GRW-LSH, the raw hash value function $f$ is %a random walk projection 
parameterized by a vector of $m$ mutually independent Ganssian random walks $\bm{\zeta} = \langle \zeta_1, \cdots, \zeta_m \rangle$. %, which we unrigorously refer as ``Brownian with Gaussian steps motions'' in the sequel to distinguish from the random walks with integer steps in RW-LSH. 
Each  $\zeta_j$ is defined by a sequence of steps that are i.i.d. standard Gaussian RVs, which differs from the (integer-valued random walk) $\tau_j$ at the marginal distribution of each step. Given a data point $\mathbf{s} = \langle s_1, s_2, \cdots, s_m \rangle$, $f(\mathbf{s})$ is defined as $\sum_{j=1}^m S^{\zeta_j}[0, s_j)$.
Similarly, GRW-LSH requires that each $s_j$, $j=1,2,\cdots, m$, be a nonnegative integer. GRW-LSH achieves similar accuracy in ANNS-$L_1$ as RW-LSH, because Gaussian random walks are statistically close to integer-valued random walks when the number of steps is large. %and it is better suited for a DST-based implmentation, 

[duplicate] Our DST-based GRW-LSH implementation is the same as the DST-based RW-LSH above, except that it uses the split definitions in \autoref{sec:gauss} to generate Gaussian steps instead of single-step random walks in \autoref{sec:randw}. It runs faster than the DST-based RW-LSH, because Gaussian distribution is  ``nice'', so its range-sums can be generated four times as fast as those of single-step random walks (shown in \autoref{sec:dyaperf}). %uses the splits described in~ and low-level hash function that are two-wise independent for each Brownian motion $\zeta$, 
It also has a similar guarantee as above that
$f(\mathbf{s}) - f(\mathbf{q}) = \sum_{j=1}^m (S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j))$ is a Gaussian random walk of $\sum_{j=1}^m |s_j-q_j| = d_1$ steps and follows Gaussian distribution $\mathcal{N}(0, d_1)$, for the following 
reason:  For each $j$, $j = 1, 2,\cdots, m$, $S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j)$ equals to either $S^{\zeta_j}[q_j, s_j)$ or $S^{\zeta_j}[s_j, q_j)$ depending on which one in $s_j$ and $q_j$ is greater, which is always an
$|s_j - q_j|$-step Gaussian random walk along the sequence $\zeta_j$, and these 
$m$ Gaussian random walks are mutually independent since they are along different sequences. 
The distribution of $f(\mathbf{s}) - f(\mathbf{q})$ resembles its counterpart in GP-LSH~\cite{Datar_LSH_2004} and differs only in the variance, since the latter follows $\mathcal{N}(0, d_2^2)$ where %$\mathcal{N}(0, d_2^2)$. 
$d_2^2$ is the squared $L_2$ distance between $\mathbf{s}$ and $\mathbf{q}$, \ie $d_2 ^2= \sum_{j=1}^m (s_j-q_j)^2$. This resemblance is important, because it implies that GRW-LSH is an LSH function similarly to GP-LSH and inherits GP-LSH's multi-probe extension~\cite{lv2007multiprobe}, which greatly reduces the number of hash tables for reaching a target query accuracy. We call the version of GRW-LSH with multi-probe extension MP-GRW-LSH in the sequel.
\end{comment}

%Obviously, we can avoid the precomputed table by directly generating the range-sum $S^{\tau}[0, t)$ of each random walk $\tau$ with dyadic simulation as . study the efficient implementation with dyadic simulation of only
%This DST-based RW-LSH implementation may be useful in some applications that restrict the hash values to integers. 



%In GRW-LSH, the raw hash value function $f$ is %a random walk projection 
%parameterized by a vector of $m$ mutually independent Ganssian random walks $\bm{\zeta} = \langle \zeta_1, \cdots, \zeta_m \rangle$. %, which we unrigorously refer as ``Brownian with Gaussian steps motions'' in the sequel to distinguish from the random walks with integer steps in RW-LSH. 
%Each  $\zeta_j$ is defined by a sequence of steps that are i.i.d. standard Gaussian RVs, which differs from the (integer-valued random walk) $\tau_j$ at the marginal distribution of each step. Given a data point $\mathbf{s} = \langle s_1, s_2, \cdots, s_m \rangle$, $f(\mathbf{s})$ is defined as $\sum_{j=1}^m S^{\zeta_j}[0, s_j)$.
%Similarly, GRW-LSH requires that each $s_j$, $j=1,2,\cdots, m$, be a nonnegative integer. GRW-LSH achieves similar accuracy in ANNS-$L_1$ as RW-LSH, because Gaussian random walks are statistically close to integer-valued random walks when the number of steps is large. %and it is better suited for a DST-based implmentation, 



%Let $\mathbf{q}= \langle q_1, q_2, \cdots, q_m \rangle$ be the query point.  
%We denote as $d_1$ the value of the $L_1$ distance between $\mathbf{s}$ and $\mathbf{q}$, that is, $d_1 = \sum_{j=1}^m |s_j-q_j|$;
%$d_1$ is a nonnegative integer since every $s_j$ and $q_j$ is.
%Then 
%Our DST-based GRW-LSH implementation is the same as the DST-based RW-LSH above, except that it uses the split definitions in \autoref{sec:gauss} to generate Gaussian steps instead of single-step random walks in \autoref{sec:randw}. It runs faster than the DST-based RW-LSH, because Gaussian distribution is  ``nice', so its range-sums can be generated four times as fast as those of single-step random walks (shown in \autoref{sec:dyaperf}). %uses the splits described in~ and low-level hash function that are two-wise independent for each Brownian motion $\zeta$, 
%It also has a similar guarantee as above that
%$f(\mathbf{s}) - f(\mathbf{q}) = \sum_{j=1}^m (S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j))$ is a Gaussian random walk of $\sum_{j=1}^m |s_j-q_j| = d_1$ steps and follows Gaussian distribution $\mathcal{N}(0, d_1)$, for the following 
%reason:  For each $j$, $j = 1, 2,\cdots, m$, $S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j)$ equals to either $S^{\zeta_j}[q_j, s_j)$ or $S^{\zeta_j}[s_j, q_j)$ depending on which one in $s_j$ and $q_j$ is greater, which is always an
%$|s_j - q_j|$-step Gaussian random walk along the sequence $\zeta_j$, and these 
%$m$ Gaussian random walks are mutually independent since they are along different %sequences. 
%The distribution of $f(\mathbf{s}) - f(\mathbf{q})$ resembles its counterpart in GP-LSH~\cite{Datar_LSH_2004} and differs only in the variance, since the latter follows $\mathcal{N}(0, d_2^2)$ where %$\mathcal{N}(0, d_2^2)$. 
%$d_2^2$ is the squared $L_2$ distance between $\mathbf{s}$ and $\mathbf{q}$, \ie $d_2 ^2= \sum_{j=1}^m (s_j-q_j)^2$. This resemblance is important, because it implies that GRW-LSH is an LSH function similarly to GP-LSH and inherits GP-LSH's multi-probe extension~\cite{lv2007multiprobe}, which greatly reduces the number of hash tables for reaching a target query accuracy.

%We now describe the implementation of each Brownian motion $\zeta$ via dyadic simulation (here we drop the subscript $j$, with the understanding that each $\zeta_j$ is an independent instance of $\zeta$). Unlike in data streaming, a surprisingly cheap implementation of dyadic simulation has all theoretical guarantees of BM-LSH on ANNS-$L_1$, even though its singletons are not mutually independent. In this implementation, the random strings $C_\alpha$ (in \autoref{sec:overview}) are generated with a two-wise hash function on each level of the simulation tree, so a simulation tree takes only $O(\log U)$ space and generates each range-sum in $O(\log U)$ time. According to \autoref{th:stdist}, this implementation guarantees that each range-sum $S^{\zeta} [a, b)$ follows distribution $\mathcal{N}(0, b-a)$, so for each $a, b = 0, 1, \cdots, U-1$ (without loss of generality, suppose $b> a$), $\zeta(b) - \zeta(a)$ has the same distribution of an
%$(b-a)$-step Brownian motion.
%This is sufficient to show that $f(\mathbf{s}) - f(\mathbf{t})$ follows $\mathcal{N}(0, d_1)$ and all theoretical guarantees of BM-LSH above.


==> sections/lsh.tex <==
\color{black}
\section{ANNS-$L_1$ Application}\label{sec:ann}
% NOTE: organization of paper       we may need to move the backgrounds of ANN forward and add some contents in introduction.

%[background on ANNS and LSH]





%LSH~\cite{Indyk_ANN_1998} is one of the most popular ANNS solution approaches. 
%In LSH, the key intellectual component of an LSH scheme is its hash function family 
%$\mathcal{H}$.
%Any function $h$ sampled uniformly at random from $\mathcal{H}$ has the following 
%nice collision property:  It maps two distinct points in $\mathcal{D}$ to the same hash %value with probability $p_1$
%if they are close to each other (say no more than distance $r_1$ apart) and with probability $p_2 < p_1$ if they are far apart (say more than $r_2 > r_1$ apart), respectively. 

%In this section, we introduce MP-GRW-LSH, the application of dyadic simulation on ANNS-$L_1$ that improves MP-RW-LSH~\cite{mprwlsh} by scaling highly efficient ANNS queries to huge universes without having to store a large precomputed table. We also show that dyadic simulation is the preferred option over existing range-summable schemes such as EH3~\cite{feigenbaum} on ANNS, because the performance of ANNS is determined by the distribution of the generated range-sums. 
%While the former has a theoretical guarantee on this, the latter does not and can have degraded performances for worst-case queries.


In this section, we first describe an ERS 
problem that arises in MP-RW-LSH, the aforementioned multi-probe LSH solution
for ANNS-$L_1$ proposed in~\cite{mprwlsh}.  Then we study why this problem cannot be robustly
solved using an existing ERS solution called EH3~\cite{feigenbaum}.  Finally, we describe MP-GRW-LSH, a slight variant of MP-RW-LSH that 
can cleanly and robustly solve this problem using our Gaussian-DST.
% Gaussian-DST and
%has nearly identical query efficacy and better efficiency as 
%MP-RW-LSH.





%[change s to vector t, q to vector q]
In ANNS-$L_1$, given a query point $\vec{\mathbf{q}}$, 
we search in a massive dataset $\mathcal{D}$, which lies in a space of high dimensionality (say $m$),  
for one or more points $\mathbf{s}$ in $\mathcal{D}$ that are \emph{among the closest} to $\vec{\mathbf{q}}$ according to the $L_1$ distance.  
Here the $L_1$ distance between any two $m$-dimensional points $\vec{\mathbf{s}}= \langle s_1, s_2, \cdots, s_m\rangle$ and $\vec{\mathbf{q}} = \langle q_1, q_2, \cdots, q_m\rangle$, denoted as $  \|\vec{\mathbf{q}} - \vec{\mathbf{s}}\|_1$, 
is defined as  $\sum_{j=1}^m |q_j - s_j|$.

%\subsection{Locality-Sensitive Hashing (LSH)}d(\mathbf{q}, \mathbf{s})=
\subsection{The RW-LSH Algorithm}

LSH~\cite{Indyk_ANN_1998} is one of the most popular ANNS solution approaches. 
%JFM-1 (new) We first describe RW-LSH, % (Random Walk LSH), 
% and then show how to use dyadic simulation to efficiently implement our ERS-based variant called BM-LSH.(an $m$-dimensional dataset) 
In an LSH scheme, typically a vector of $M > 1$ LSH functions $\vec{\mathbf{g}} = \langle g_1$, $g_2$, $\cdots$, $g_M\rangle$ 
are used to map each point $\vec{\mathbf{s}}$ in $\mathcal{D}$ to an $M$-dimensional vector of independent hash values 
${\overrightarrow{\mathbf{g}(\mathbf{s})}} = \langle g_1(\vec{\mathbf{s}}), g_2(\vec{\mathbf{s}}), \cdots, g_M(\vec{\mathbf{s}})\rangle$.  
This point $\vec{\mathbf{s}}$ is to be stored in a hash bucket indexed 
% \textbf{Jingfan: We do not need to mention $g(\cdot)$ since use hash vector as index in hash table is common sense for readers and our iDEC also write as ``vector as hash key''.}
%({\color{red} say using a conventional hash function $g(\cdot)$}) 
by the vector ${\overrightarrow{\mathbf{g}(\mathbf{s})}}$;
hence we identify this hash bucket as ${\overrightarrow{\mathbf{g}(\mathbf{s})}}$. 
% \textbf{Huayi: I think we need the following sentence to explain each hash table needs one LSH function vector and the meaning of $n$.}
%{\color{red} These $n$ points in $\mathcal{D}$ are 
%stored in a hash table
%using their corresponding vectors as hash keys.}
%({\it e.g.}, the point $\beta$ is to be stored in hash bucket %
%$g(\langle h_1(\beta), h_2(\beta), \cdots, h_k(\beta)\rangle)$.  
Then given a query point $\vec{\mathbf{q}}$, the search procedure, in a standard LSH solution, is to
probe all points in the \emph{epicenter bucket} ${\overrightarrow{\mathbf{g}(\mathbf{q})}}$
%bin 
%that the vector $\langle h_1(\alpha), h_2(\alpha), \cdots, h_k(\alpha)\rangle$ would be inserted into, 
in the hope that 
some nearest neighbors of $\vec{\mathbf{q}}$ are mapped to the same vector (bucket). %bin.
%We regard this search procedure as hard-decision decoding, since 
%the query point $\alpha$ is ``decoded'' to precisely the vector 
%$\langle h_1(\alpha), h_2(\alpha), \cdots, h_k(\alpha)\rangle$ and only the corresponding bucket is probed. 
%$\mathbf{s}\in\mathbb{Z}^{m\smash[t]{\mathstrut}}_{\geq 0}$ is a data or query point,

%A standard LSH solution is one in which only a single hash bucket is searched in each hash table.   is one in which the algorithm(as in standard LSH)


Unlike a standard LSH solution,
a multi-probe LSH solution probes not only the epicenter bucket, but also 
$T > 0$ other nearby buckets whose success probabilities (of containing a nearest neighbor) are among the highest.
%$T$  (excluding the epicenter bucket).
Among LSH solutions, a multi-probe one, if it can be found, is arguably the most desirable one because its index size for achieving the 
same query accuracy is much smaller than that of a standard LSH solution~\cite{mprwlsh}.  


%We now describe what 

%{\color{blue} (Add by Huayi) To simplify notation, we focus on only one hash function $g(\vec{\mathbf{s}})$ and drop its subscript in the sequel.}
An LSH function $g(\vec{\mathbf{s}})$ in RW-LSH~\cite{mprwlsh}
%the first multi-probe solution for ANNS-$L_1$. % and in BM-LSH, our ERS-based variant of RW-LSH that has an efficient implementation with dyadic simulation. 
%To simplify notation, we focus on only one hash function $g(\mathbf{s})$ and drop its subscript in the sequel. 
%l, with the understanding that each $g_j(\mathbf{s})$, $j=1,2,\cdots, M$, is an independent instance of $g(\mathbf{s})$.
%In both LSH schemes, same
takes the  following form:  
$g(\vec{\mathbf{s}}) \triangleq  \left\lfloor (f(\vec{\mathbf{s}}) + B)/W \right\rfloor$, 
where  $W > 0$ is a constant and $B$ is a RV (fixed after generation) uniformly distributed in $[0, W]$. % In this section and~\autoref{sec:eva}, we reuse the letter $W$, since it will not cause confusions.
Here $f(\vec{\mathbf{s}})$ is called the \emph{raw hash value} of $\vec{\mathbf{s}}$. 


Before we describe such an $f(\cdot)$, we need to introduce some notations.
Let $\tau$ be a sequence of independent RVs $X_0$, $X_1$, $X_2$, $\cdots$ 
%{\bf [add superscript $\tau$ to them ]  JFM: maybe not} 
that each has a single-step random walk distribution.
When necessary, we call $\tau$ a {\it strict} random walk sequence to emphasize the (strict) independence among its steps.
% {\bf[delete?] and to highlight its difference with  
%a random walk (sequence) whose steps are strongly correlated. } 
Let $q$ and $s$ be two nonnegative integers such that $q \le s$.  
We define $S^{\tau}[q, s)$ as the $(s-q)$-step random walk $X_q+ X_{q+1} + \cdots + X_{s-1}$.  
Clearly, $S^{\tau}[q, s)$ is also a range-sum, with the underlying RVs being the sequence $\tau$.  
For notation convenience in the following, we also define the value of $S^{\tau}[s, q)$ as $-S^{\tau}[q, s)$.

In RW-LSH, the raw hash value function $f(\cdot)$ is parameterized by a vector of $m$ (which is also the dimension of the dataset $\mathcal{D}$) 
such strict random walk sequences $\vec{\bm{\tau}} = \langle \tau_1, \tau_2, \cdots, \tau_m \rangle$ that 
are  independent.
%Each $\tau_j$ is a sequence of single-step random walks that are mutually independent. 
%i.i.d. random variables, each of which takes value $1$ or $-1$ with equal probability $1/2$;  the value of each random variable is fixed 
%once it is generated. %, just as the computational model in \autoref{sec:overview}.  
%\textbf{In the sequel, we refer to such a random walk with mutually independent steps as a ``real'' random walk, in contrast to other instances that does not guarantee mutual %independent steps.}
Given a data point $\vec{\mathbf{s}} = \langle s_1, s_2, \cdots, s_m \rangle$, the raw hash value $f(\vec{\mathbf{s}})$ is defined as $\sum_{j=1}^m S^{\tau_j}[0, s_j)$.
In other words, $f(\vec{\mathbf{s}})$ is the result of randomly walking $s_1$ steps along sequence $\tau_1$, $s_2$ steps along $\tau_2$, $\cdots$, and $s_m$ steps along $\tau_m$.
RW-LSH requires that each $s_j$, $j = 1, 2,\cdots, m$, be a nonnegative even integer.  

%This requirement is imposed on all data points in $\mathcal{D}$  
%and all query points, to guarantee a monotonocity condition that, as we will explain shortly, qualifies a hash function family as LSH.  

We now fix a query point $\vec{\mathbf{q}}$ and a point $\vec{\mathbf{s}}$ in the dataset $\mathcal{D}$.  
We now state some facts that will be used both next and soon in~\autoref{sec:grwlsh}.
Let $d_1$ be the $L_1$ distance between $\vec{\mathbf{q}}$ and $\vec{\mathbf{s}}$, that is, $d_1 = \sum_{j=1}^m |s_j-q_j|$.
%$d_1$ is a nonnegative integer since every $s_j$ and $q_j$ is.
%The performance of LSH heavily relies on the distribution of 
Then, $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})= \sum_{j=1}^m\left(S^{\tau_j}[0, s_j) -S^{\tau_j}[0, q_j) \right) =  \sum_{j=1}^mS^{\tau_j}[q_j, s_j)$~\cite{mprwlsh}. 
%Here, we have to clarify a subtle issue on notation. We have
%defined the range-sum $S^{\tau_j}[q_j, s_j)$ only when $q_j\leq s_j$, but it might be $q_j > s_j$, in which case we define $S^{\tau_j}[q_j, s_j) \triangleq -S^{\tau_j}[s_j, q_j)$.
%Since $f(\mathbf{s})  - f(\mathbf{q})$  .
%the random walks   $\langle \tau_1, \tau_2, \cdots, \tau_m \rangle$ are mutually independent, and because$f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$ has the same distribution as a  
%each   has the distribution of $d_1$-step random walk, because it is the sum of $m$ independent range-sums,
Note that each range-sum $S^{\tau_j}[q_j, s_j)$ has the distribution of a $|s_j - q_j|$-step random walk 
whether $q_j\leq s_j$ or $q_j> s_j$, since (the pdf of) every underlying single-step random walk is symmetric about $0$.
Since the random walks $S^{\tau_j}[q_j, s_j)$, $j = 1, 2, \cdots, m$, are independent (as they are along independent sequences), $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$
has the distribution of a $d_1$-step random walk, and hence is parameterized only by  $d_1$.
When $d_1$ is not small (say when $d_1 > 25$), this distribution can be closely approximated as $\mathcal{N}(0, d_1)$.
It has been shown in~\cite{mprwlsh} that this distribution being approximately Gaussian leads to every nice property of RW-LSH and its multi-probe 
extension MP-RW-LSH.

%highly efficient (w.r.t. query time) and
%effective (w.r.t. query accuracy).

 %(thanks to sin$|q_j - s_j|$-step random walk gle-step random walk has a symmetric distribution about 0).the number of steps
% Here we need to use a property of  (and the same for Gaussian distribution $X$): and, it because, the distribution of the range-sum of $|s_j-q_j|$ i.i.d. steps,
 %$S^{\tau_j}[s_j, q_j)$ is symmetric about $0$, or in other words $S^{\tau_j}[s_j, q_j)$ and $-S^{\tau_j}[s_j, q_j)$ have the same distribution, because
%the underlying RV $X$ at each step is symmetric about $0$.

%[JFM] Recall that the performance of (standard or multi-probe) LSH relies on the distribution of 

\begin{comment}
Now we are ready to derive the pdf of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$.

 which we already know is the sum of $m$ independent range-sums $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality), so it is important that each $S^{\tau}[q, s)$ is the range-sum of a \emph{strict} random walk. Under this condition,  $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$  is a strict random walk of $d_1$ i.i.d. steps, which is  parameterized only by  $d_1$.
When $d_1$ is not small, the distribution of a $d_1$-step random walk can be very closely approximated as the Gaussian distribution $\mathcal{N}(0, d_1)$.
It has been shown in~\cite{mprwlsh} that this Gaussian distribution alone makes MP-RW-LSH highly efficient (w.r.t. query time) and
effective (w.r.t. query accuracy).


%It is not hard to show that , is a  this $d_1$-step random walk.  Therefore,  , which is JFM] Since  if the random walks are strict, and in general relies onthe distribution of each range-sum .[], $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$ is a deterministic function of $d_1$


[duplicated] When $d_1$ is not small, the distribution of $d_1$-step random walk can be very closely approximated as the Gaussian distribution $\mathcal{N}(0, d_1)$.
It has been shown in~\cite{mprwlsh} that this Gaussian distribution alone that makes MP-RW-LSH highly efficient (w.r.t. query time) and
effective (w.r.t. query accuracy).
It is not hard to show that $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$, the marginal 
(collision) probability for $\vec{\mathbf{s}}$ to have the same LSH value (by the LSH function $g()$) as the query point $\vec{\mathbf{q}}$, is a (deterministic) linear functional of the pdf of this $d_1$-step random walk.  Therefore, the performance guarantee of LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality), which is a deterministic function of $d_1$ (parameterized by $W$ used  {\color{red}in $g(\vec{\mathbf{s}})$ }) if the random walks are strict.
\end{comment}

%(the total number of $f(\cdot)$ functions)as large as hundreds to

Recall that 
In the MP-RW-LSH scheme, given a query point $\vec{\mathbf{q}}= \langle q_1, q_2, \cdots, q_m \rangle$, we need to compute the raw hash value $f(\vec{\mathbf{q}}) 
= \sum_{j=1}^m S^{\tau_j}[0, q_j)$
for $L M$ ($L$ hash tables each using a vector 
of $M$ hash functions) such ($f$)'s.
Computing these range-sums one (random walk) step at a time is a relatively computationally heavy task, since
%is to compute, given a query point $\vec{\mathbf{q}}= \langle q_1, q_2, \cdots, q_m \rangle$,
%$L M$ ($L$ hash tables each using a vector 
%of $M$ hash functions) such raw hash values of $\vec{\mathbf{q}}$.  
although each step takes only nanoseconds to compute, there
are simply too many of them:
There are a total of $O(LMmU)$ steps, where $LM$  is typically in hundreds, 
the data dimension $m$ can be in thousands, and the maximum possible number of steps $U$ to walk along 
each random walk sequence $\tau$ can be hundreds of thousands.   As a result, it is not uncommon for $LMmU$ to be on the
order of $10^{10}$ or $10^{11}$.  This translates into tens of seconds of or minutes of computation time just for the raw hash values
of $\vec{\mathbf{q}}$.  In contrast, the rest of the ANNS query can often be done in tens of milliseconds.  
To reduce the time of computing these range-sums, RW-LSH precomputes and stores all $S^{\tau_j}[0, q_j)$ values for $q_j = 0, 1, 2,\cdots, U$ and for each random walk 
sequence $\tau_j$.  This reduces the time complexity to $O(LMm)$ but bloats the total size of precomputation tables to $O(LMmU)$, which can translate into 
tens of gigabytes of storage as will be shown in~\autoref{sec:eva}.
%The ERS solutions that we will describe soon achieve the better of both worlds: It does not need precomputed tables, and the complexities in both space and evaluation time are as low as $O(LMm\log U)$.
% for each range-sum $S^{\tau}[0, q)$ achieves
\begin{comment}
To reduce the time of evaluating $f(\mathbf{s})$, the baseline solution of RW-LSH precomputes and stores each  $S^{\tau_j}[0, s_j)$ for $t = 2, 4, 6, \cdots, U_j$ where $U_j$ is the maximum possible (even) 
value for the $j^{th}$ coordinate of a data point.  For any random walk $\tau_j$, the baseline RW-LSH needs $U_j$ bytes for storing the precomputed table. Although
the storage cost of each precomputed table, which is roughly $O(mMU)$, supposing $U$ is the maximum value among $U_j$, is small relative to the size of each hash table, which is $O(n_d)$ and  $n_d$ is the size of the dataset, for large datasets, this cost can increase the total index size by several hundred times, for some smaller datasets where both $m$ and $U_j$ are very large (relative to the dataset size), 
as we will show in~\autoref{sec:eva}. 
\end{comment}

%We will explain shortly why this assumption is not 
%overly restrictive for real-world applications. 




%To reduce the storage cost of precomputed tables, the authors of \cite{mprwlsh} proposes ``long jump'', which reduces the storage cost by $32l$ times by paying $l$ CPU instructions for evaluating each range-sum $S^{\tau_j}[0, t)$. Even with this solution, the product of space and time complexities of RW-LSH is still $O(U_j)$ for each random walk, which is not scalable for future databases where $U_j$ might be gigantic.

%efficient range-summable (ERS) algorithms  to save the space of the precompute table
% ERS solutions, which only takes a small space and poly-logarithmic time. We can indeed use dyadic simulation to implement RW-LSH by generating range-summable single-step random walks , but %generate , but a better solution is to generate Gaussian random variables instead, because the latter can be  since it does not require rejection sampling. In BM-LSH, by changing the distribution of each step from a single-step random walk to a standard Gaussian random variable, we reformulate the random walk in RW-LSH to a discrete time Brownian motion. This reformulation is justified because a random walk is statistically close to a Brownian motion when $n$ (the number of steps) is large.
 

 %Since the evaluation of RW-LSH resolves to the ERS problem, 
 %Readers may wonder if
%{\bf no BCH3 anymore} 

\subsection{Why EH3 Cannot Solve This Problem}

We have considered whether EH3~\cite{feigenbaum}, an ERS scheme for single-step random walks, can be used to generate these range-sums for RW-LSH.  
The answer is ``no'' for the following reason.
  %One possible option is  which is shown by~\cite{rusu-jour} as the fastest range-summable scheme that has both theoretical guarantee (approximate $4$-wise independence) and good empirical performance (when estimating the size of joins). However, we show that EH3 is not very suitable for ANNS-$L_1$, for the following reasons.or BCH3~\cite{rusu-jour}
%   Recall that the efficacy of RW-LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ to be of a strict random walk.
  Although every underlying RV generated by EH3 has the  %EH3 scheme in \etal{Feigenbaum}~\cite{feigenbaum} generates range-summable random variables whosebe used to and BCH3of   matches that of
  marginal distribution of a single-step random walk, these %is highly ordered (deterministic)  (as required they only preserves the three-wise independence among  andir generated random variables
RVs are strongly correlated, since as explained earlier EH3 achieves ERS by systematically destroying all independence beyond $4$-wise among the underlying RVs.  
Hence the resulting range-sum $S^\tau[q, s)$ (where $\tau$ is generated by EH3)
%guaranteed to have the same standard deviation as those from an authentic 
%random walk, they may structure when more than three consecutive random variables are concerned. generated are  Thereforefollow a very different distribution than that of
behave very differently from a $(s - q)$-step random walk. %For example, when $[q, s)$ is a dyadic interval of width $2^l$ 
%{\bf JFM: I think $l$ is best. (DO WE WANT TO USE l here?)}, %the range-sum $S^\tau[q, s)$ generated by BCH3 is equal to $0$ with probability $1-2^{-l}$, 
%and has absolute value $2^l$ with probability $2^{-l}$~\cite{rusu-jour}.
%This distortion seriously impacts the distribution of $f(\mathbf{s})  - f(\mathbf{q})$ and the accuracy of RW-LSH.
%EH3 has a slightly better distribution of range-sums than BCH3 that is no longer 0 with high probability, but that is still far from that of a strict random walk.
%Although EH3 has a slightly stronger guarantee than BCH3 of approximate four-wise independence, so it has theoretical guarantees in the accuracy of estimating the $L_2$ moment in data streams in its proposed application, but it suffers from the same problem as above. %the generated range-sums still follow a very different distribution from
% is, its detailed distribution may be very different from the latter.$S^{\tau}[0, 10^6)$ 
For example, when $[q, s)$ is a dyadic range and  $s - q = 4^l$, the range-sum $S^\tau[q, s)$ 
%generated by EH3 
takes values $2^l$ and $-2^l$ each with probability 1/2.
%follows uniform distribution in $\{2^l, -2^l\}$~\cite{rusu-jour}, so its absolute value is always $2^l$! 

\begin{comment}
\autoref{fig:distcomp} shows another example in which $[a, b)$ is  $[0, 10^6)$, which is not a dyadic interval. The histogram at the top is plotted from one million range-sums $S^{\tau}[0, 10^6)$ generated from EH3 with different seeds, and that at the bottom is from %one million range-sums of the same range from , which
a ``real'' random walk with empirically independent steps is generated by the built-in \texttt{mt19937} PRNG (not range-summable) in C++.%, and plot its distribution histogram at the top of \autoref{fig:distcomp}. at the bottom
%plot the histogram of the range-sum  generated from EH3 with one million different seeds  from  (not range-summable) 
%As a reference, we also plot the histogram of $S^{\tau}[0, 10^6)$ in 
 \begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{figures/histogram.eps}
	\caption{Distribution of generated random walks (Y axis normalized to probability density).}\label{fig:distcomp}
\end{figure}
From \autoref{fig:distcomp}, the distribution of range-sums generated by EH3 is far from that of the ``real'' random walk below, but concentrates at some special points near $1000$ (its standard deviation) and $-1000$. 
\end{comment}
%In contrast, the distribution of the range-sums generated by dyadic simulation % and of the independent non-range-summable random walk are distributed
%is close to the reference Gaussian distribution. This shows dyadic simulation is more suitable to ANN applications where the distribution of range-sums is crucial to the performance.
%In an even more extreme example, 
%Therefore, the performance of applying EH3 to MP-RW-LSH leads to unstable performance and significant degradation for some special queries on which the distribution of the produced range-sums is far from that of random walks. This will be illustrated by simulations in \autoref{sec:feigen_sim}.

 %preserves the independence between %different steps of the Brownian motion with the use of $O(\log U)$ two-wise independent hash functions (to be explained in ??) %if a two-wise independent hash function is used on each level of the simulation tree (to be explained later), 
%, so it is better suited for this application. of this distribution onof the distribution of range-sums , corresponding to recalls changes with $d_1$


%It has been shown in~\cite{stablelsh} that the performance guarantee of standard 
A key metric for measuring the quality of any LSH function family is $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$, the 
(collision) probability for $\vec{\mathbf{s}}$ to have the same LSH value (by the LSH function $g(\cdot)$) as the query point $\vec{\mathbf{q}}$.
%(so that $\vec{\mathbf{s}}$ can be found by the ANNS query in case it is a nearest neighbor of $\vec{\mathbf{q}}$).
In RW-LSH, this probability is a (deterministic) linear functional of the pdf of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}}) = \sum_{j=1}^mS^{\tau_j}[q_j, s_j)$.
%It as shown in~\cite{} that this pdf leads to virtually every nice property of RW-LSH.
% can be derived from the pdf of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$.
%(parameterized by $W$ {\color{red} used in $g(\vec{\mathbf{s}})$}). For a similar reason, the performance guarantee of multi-probe LSH also relies on the distribution of $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$~\cite{mprwlsh}.
We now study how the use of EH3 for generating the sequences $\tau_j$, $j = 1,2, \cdots, m$, impacts 
%the damaging effect of this strong correlation among the random walk steps on 
the collision probability $\Pr[g(\vec{\mathbf{s}}) = g(\vec{\mathbf{q}})]$ by distorting the range sums $S^{\tau_j}[q_j, s_j)$, $j=1,2, \cdots, m$.
We do so by zooming in on its damaging effect on a single sequence $\tau_1$ as follows:
%To isolate the effect of a single EH3-generated random walk sequence on the corresponding range sum, 
%$S^\tau[q, s)$ affects the collision probability, we now place further restrictions on these two points while keeping them $d_1$ apart in $L_1$ distance.
We let $\vec{\mathbf{q}} = \vec{\mathbf{s}}$ in every coordinate except the first, where $s_1 = 0$ and $q_1 = D$, so that $d_1 =  \sum_{j=1}^m |s_j-q_j| = D$.  
This way the value $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}}) = S^{\tau_1}[0, s_1)$, and hence the collision probability, is affected by only $\tau_1$.
%When the single-step random walks in the sequence $\tau_1$ is  independent,
%$f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}}) $ is a strict random walk with $d$ steps.  

In \autoref{fig:coll_prob}, we compare this collision probability ($y$-axis), which is a function of $D$ ($x$-axis), in two cases:  (1) \emph{original},
when $\tau_1$ is a strict random walk;  (2) \emph{EH3-augmented}, when $\tau_1$ is generated by EH3.
In case (1), this probability is monotonically decreasing as $D$ increases.
This monotonicity property has been widely used as a litmus test for an ``aspiring'' LSH function family~\cite{Indyk_ANN_1998}.
%qualifying requirement 
% for a (hash) function family to become a legitimate LSH function family [?] {\bf talk with Huayi}.
In contrast, in case (2), the collision probability jumps up and down when $D$ becomes larger.
%The obvious oscillation of the blue line in \autoref{fig:coll_prob} shows that the distortion of the distribution %of range-sums by EH3 shown in \autoref{fig:distcomp} against the ideal case with independent steps. 
%This phenomenon is extreme
This behavior automatically disqualifies the ``EH3-augmented'' RW-LSH, as an LSH function family.  
Furthermore, when the distance $D$ is chosen so that the collision probability (curve) falls into a ``valley'' (e.g., between \SI{16000}{} and \SI{17000}{}), 
%the collision probability becomes close to 0.
%As a result, 
the (success) probability for $\vec{\mathbf{q}}$ to be hashed into the epicenter bucket and be found by the ANNS query becomes very close to 0.
In this case, the query accuracy can be very low, 
%It can be shown that this probability remains low 
even when multi-probe is used, as we will show next to some extent.  
%has a significant influence on the collision probability  against ideal RW-LSH, especially in the ``valleys'' in which it is impossible to find the data point in the epicenter bucket! 
%(The first two valleys occur at distance $16384$ and $49152$.) 
%As a result, it is difficult to guarantee robust performance when EH3 is used to implement RW-LSH.  

% happens to cause the

\begin{comment}
[added]
To further verify 
We have evaluated the ANNS-$L_1$ query accuracy of MP-RW-LSH using EH3 on the Enron dataset (see ???), when the distance of the nearest neighbor to a query point
We have found that its recall value is an order of and that of MP-RW-LSH using precomputed tables.
show 
%tune the parameter for the ANNS with EH3
%which may lead to significant performance degradation in some bad cases. 


%[maybe still useful]
%When the single-step random walks in the sequence $\tau_1$ is mutually indepdent,
%$f(...) - f(...)$ is an authentic random walk with $d$ steps.  


[duplicate]
When the single-step random walks in the sequence $\tau_1$ is mutually indepdent,
$f(...) - f(...)$ is an authentic random walk with $d$ steps.  






[duplicate]
it is the sum of $m$ independent range-sums, and the range-sum on the $j^{th}$ coordinate is a $|q_j - s_j|$-step random walk. Therefore, the performance guarantee of LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality).

[mostly spent]
hashed by a single LSH function $g$.  
in the following (overly simple) simulation, we set the LSH bucket width $W=122$ (same as the simulation below) and regard the range-sum $S^\tau[0, d)$ as the difference of the raw hash values $f(\mathbf{s}) - f(\mathbf{q})$, corresponding to the case where %$m=1$, $\mathbf{s}=\langle 0\rangle$, and $\mathbf{q}=\langle d\rangle$. 
$\mathbf{s}$ and $\mathbf{q}$ differ only at the $j^{th}$ coordinate, with $s_j=0$ and $q_j=d$. We plot the frequency of hash collisions (\ie $g(\mathbf{s}) = g(\mathbf{q})$) in one million runs for each $d$ on a wide range in \autoref{fig:coll_prob}, against ideal RW-LSH. %(directly computed from the property that $f(\mat

[duplicate]In this section, we show why existing range-summable generation schemes, such as EH3~\cite{feigenbaum}, is not suitable for ANNS.  In particular, we show by simulation that the dependency between the components of the EH3 scheme interferes the distribution of the difference of raw hash values $f(\mathbf{s})  - f(\mathbf{q})$, making it far from Gaussian.

\end{comment}
% samplesThe distribution of the final position shold$To compare the distribution of range-sums, we generate $1$ million range-sums of 1 million standard gaussian random variables from existing range-summable sketches for $L_1$ \cite{feigenbaum} and dyadic simulation and plot the histograms as \autoref{fig:distcomp} against the distribution of one-million step random walks and reference Gaussian $\mathcal{N}(0, 10^6)$. Ideally, the range-sums should follow Gaussian distribution with mean $0$ and standard deviation $1000$ (bottom figure). 



%[maybe still useful]
%it is the sum of $m$ independent range-sums, and the range-sum on the $j^{th}$ coordinate is a $|q_j - s_j|$-step random walk. Therefore, the performance guarantee of LSH relies on the distribution of each range-sum $S^{\tau}[q, s)$ (We drop subscript $j$ and assume $q \leq s$ without loss of generality).

%[mostly spent]
%hashed by a single LSH function $g$.  
%in the following (overly simple) simulation, we set the LSH bucket width $W=122$ (same as the simulation below) and regard the range-sum $S^\tau[0, d)$ as the difference of the raw hash values $f(\mathbf{s}) - f(\mathbf{q})$, corresponding to the case where %$m=1$, $\mathbf{s}=\langle 0\rangle$, and $\mathbf{q}=\langle d\rangle$. 
%$\mathbf{s}$ and $\mathbf{q}$ differ only at the $j^{th}$ coordinate, with $s_j=0$ and $q_j=d$. We plot the frequency of hash collisions (\ie $g(\mathbf{s}) = g(\mathbf{q})$) in one million runs for each $d$ on a wide range in \autoref{fig:coll_prob}, against ideal RW-LSH. %(directly computed from the property that $f(\mathbf{s}) - f(\mathbf{q})$ is $\mathcal{N}(0, d)$, the approximation of a $d$-step random walk).
%especially the collision probability (of having the same hash value) of RW-LSH. We draw   with a varying number of steps generated by EH3 similarly to the simulation above. % The following simulation provides a more intuitive view on how the distribution of the random walk (of the difference of raw hash values) influence the performance of ANNS. 
%In this   %fix the query point at $0$, and increase the first coordinate of the nearest neighbor while fixing the other coordinates at $0$.  (equivalent to the case when data and query points are one-dimensional, the query points is $0$, and the data point $d$ is moving).
%\autoref{fig:coll_prob} shows the  of EH3 against 
%

\begin{figure}[!ht]
	\centering
	\caption{Comparison of collision probabilities, $W=122$.}\label{fig:coll_prob}
	\includegraphics[width=0.51\textwidth]{figures/collprob.eps}
\end{figure}

% Figure.\, \ref{fig:coll_prob} gives an example in which the dependence of ETH3 significantly affect the collision probability (of finding a nearest neighbor in the same bucket). %Therefore, the generated sequence is not a real random walk, so $f(\mathbf{s}) - f(\mathbf{t})$ will not always converge to Gaussian distribution as required by the LSH function and is very sensitive to input. 
%We will show in ??? that the range-summable ``random-walk'' scheme by~\cite{feigenbaum} is not suitable for ANNS-$L_1$.


%\textbf{The probability of $|g(\mathbf{s}) - g(\mathbf{q})|=1$ also oscillates in a similar manner, so the probability of finding $\mathbf{s}$ even with multi-probe used is not stable. Note that the numbers in \autoref{fig:coll_prob} do not directly explain the next experiment, because the collision probability depends on the nearest neighbor $\mathbf{s}$, which is no longer $\langle 0\rangle$ in real datasets. }

%In comparison, dyadic simulation can generate range-summable random variables that are nearly perfectly independent, so it is better suited for the ANNS-$L_1$ application. We can indeed use dyadic simulation to generate empirically independent range-summable single-step random walks as in \autoref{sec:randw}, but a better solution is to generate Gaussian random variables instead, because the latter can be generated four times as fast as random walks since it does not require rejection sampling. In BM-LSH, by changing the distribution of each step from a single-step random walk to a standard Gaussian random variable, we reformulate the random walk in RW-LSH to a discrete time Brownian motion. This reformulation is justified because a random walk is statistically close to a Brownian motion when $n$ (the number of steps) is large.

%Since the range-sum of  we may use (rounded) Gaussian distribution approximation in rejection sampling. However, we think it might be better to just take the easy step: to use the range-summable scheme for Gaussian distribution in this application. For this purpose
%We reformulate RW-LSH to a closely related stochastic process, a discrete time Brownian motion. 







\begin{comment}
\textcolor{teal}{
How to efficiently search for similarity on large (large element number, high dimension) databases? 
(definition of c-ANN)
We focus on $l_1$ distance, because it is important (robust to outliers) and underexplored.
A thread of high performance ANN by Locality Sensitive Hashing (LSH) indices. For similar pairs of (data and query) points that are closer under $l_1$ metric (than a certain threshold), the LSH function maps them to the same bucket with higher probability. But for dissimilar pairs of points, this LSH function maps them to the same bucket with very low probability.(definition of LSH)
% One basic LSH is constructed with stable distribution, which is generic for $l_p$ distance with $1\leq p\leq 2$. 
In addition to the ``hard decoding" schemes that works only when the data and query are in the same bucket, researchers have put forward ``soft decoding" schemes, such as SRS and multiprobe \cite{multiprobe}, which also search nearby buckets for data candidates. These schemes achieve higher memory efficiency, but they require the distribution of the difference of hash values $f(\mathbf{x})-f(\mathbf{q})$ to be concentrated so that near neighbors will always be hashed close to the query.  However, the only? $l_1$ LSH function $f$ till now is based on stable distributions \cite{stablelsh}, under which the distribution of $f(\mathbf{x})-f(\mathbf{q})$ follows the corresponding stable distribution for $l_p$ norm with $1\leq p\leq 2$. Although Gaussian distribution (stable for $l_2$) is nicely concentrated, Cauchy distribution (stable for $l_1$) has a heavy tail. As a result, a large proportion of data points may be hashed far away from the query point under the Cauchy scheme, which is why multiprobing performs well on $l_2$ but is less effective on $l_1$. 
}\end{comment}
 
% \subsection{Comparison with EH3 Scheme}\label{sec:feigen_sim}
 %However, no existing range-summable scheme maintains the distribution of the range-sum as perfect Gaussian as required by the LSH propery (and multiprobing). 
%[duplicate]In this section, we show why existing range-summable generation schemes, such as EH3~\cite{feigenbaum}, is not suitable for ANNS.  In particular, we show by simulation that the dependency between the components of the EH3 scheme interferes the distribution of the difference of raw hash values $f(\mathbf{s})  - f(\mathbf{q})$, making it far from Gaussian.
 
%[duplicate]At first, we compare the distribution of generated range-sums from simulation. In each run of the simulation, we generate the final position of a random walk or a Brownian motion with the following three schemes. \textbf{Sequence of schemes?} The first one is dyadic simulation for standard Gaussian target distribution, which generates the final position of a Brownian motion $S^{\zeta}[0, 10^6)$. The second scheme is EH3, which generates the final position of a ``random walk'' $S^{\tau}[0, 10^6)$ with the same number of steps. The third scheme is a ``real'' random walk $S^{\tau}[0, 10^6)$ from empirically independently steps (not range-summable) generated by the built-in \texttt{mt19937} PRNG in C++. %The third scheme is to use range-summable  to generate a random walk for the same $\tau(t)$ at $t=10^6$. 
%For all three schemes above, we draw the histogram (normalized to probability density) from one million independent runs and show at the bottom of \autoref{fig:distcomp} the reference Gaussian distribution $\mathcal{N}(0, 10^6)$ , %draw the histogram for the distribution of the final position, 
%to which all of the top three figures should converge. %is the distribution should all converge to with mean $0$ and standard deviation $1000$ (bottom figure). 

% samplesThe distribution of the final position shold$To compare the distribution of range-sums, we generate $1$ million range-sums of 1 million standard gaussian random variables from existing range-summable sketches for $L_1$ \cite{feigenbaum} and dyadic simulation and plot the histograms as \autoref{fig:distcomp} against the distribution of one-million step random walks and reference Gaussian $\mathcal{N}(0, 10^6)$. Ideally, the range-sums should follow Gaussian distribution with mean $0$ and standard deviation $1000$ (bottom figure). 
 

 
%[duplicate] From \autoref{fig:distcomp}, the distribution of range-sums generated by EH3 is far from that of the ``real'' random walk, but concentrates at some special points near $\pm1000$ (in order to have $0$ mean and $1000$ standard deviation). In contrast, the distribution of the range-sums generated by dyadic simulation % and of the independent non-range-summable random walk are distributed
%is close to the reference Gaussian distribution. This shows dyadic simulation is more suitable to ANN applications where the distribution of range-sums is crucial to the performance.
% \textcolor{teal}{However, no existing range-summable scheme maintains the distribution of the range-sum as perfect Gaussian as required by the LSH propery (and multiprobing). For example, the scheme in \cite{feigenbaum} can only guarantee approximate four-wise independence, which sacrifices all higher orders of independence in return for range-summability, and although \cite{rusu-jour} described several range-summable schemes with a higher degree of independence, the time complexity of these schemes is too high. }%Four-wise independence is sufficient for bounding the variance of the estimator in the streaming application, but for ANN, 
%To intuitively show  the impact of this distribution on the performance of ANNS, especially the collision probability (of having the same hash value) of RW-LSH. We draw \autoref{fig:coll_prob}  with a varying number of steps generated by EH3 similarly to the simulation above. % The following simulation provides a more intuitive view on how the distribution of the random walk (of the difference of raw hash values) influence the performance of ANNS. 
%In this (overly simple) simulation, we set the LSH bucket width $W=100$ and regard the range-sum $S^\tau[0, d)$ as the difference of the raw hash values $f(s) - f(q)$, corresponding to the case where $m=1$ and $s=\langle 0\rangle$. %fix the query point at $0$, and increase the first coordinate of the nearest neighbor while fixing the other coordinates at $0$.  (equivalent to the case when data and query points are one-dimensional, the query points is $0$, and the data point $d$ is moving).
%\autoref{fig:coll_prob} shows the ratio of hash collisions in one million runs for each $d$ of EH3 against ideal RW-LSH (directly computed from the property that $f(s) - f(q)$ is $\mathcal{N}(0, d)$, the approximation of a $d$-step random walk).
 %\begin{figure}
 %	\centering
 %	\includegraphics[width=0.48\textwidth]{figures/coll_prob_100.png}
 %	\caption{Comparison of collision probabilities.}\label{fig:coll_prob}
 %\end{figure}
% Figure.\, \ref{fig:coll_prob} gives an example in which the dependence of ETH3 significantly affect the collision probability (of finding a nearest neighbor in the same bucket). %Therefore, the generated sequence is not a real random walk, so $f(\mathbf{s}) - f(\mathbf{t})$ will not always converge to Gaussian distribution as required by the LSH function and is very sensitive to input. 
 %We will show in ??? that the range-summable ``random-walk'' scheme by~\cite{feigenbaum} is not suitable for ANNS-$L_1$.
%The obvious oscillation of the blue line in \autoref{fig:coll_prob} shows that the distortion of the distribution of range-sums by EH3 shown in \autoref{fig:distcomp} has a significant influence on the collision probability  of RW-LSH against the ideal case with independent steps. This phenomenon is extreme in the ``valleys'' in which it is impossible to find the data point in the epicenter bucket! (The first two valleys occur at distance $16384$ and $49152$.) As a result, it is difficult to guarantee consistent performance when EH3 is used to implement RW-LSH, %tune the parameter for the ANNS with EH3
%which may lead to significant performance degradation in some bad cases.
%\subsection{Comparison between Feigenbaum and Dyadic}
% \begin{table}[!htb]
% 	\caption{Comparison between MP-BM-LSH and MP-RW-LSH(EH3) on synthetic dataset. $M=7$, $W=100$}\label{tab:feigen_vs_dyadic}
% 	\centering
% 	\begin{tabular} {@{}c c c c c@{}}
% 		\specialrule{.1em}{.05em}{.05em} 
% 	\multirow{2}{*}{$L$} & \multicolumn{2}{c}{MP-BM-LSH}  & \multicolumn{2}{c}{MP-RW-LSH (EH3)} \\\cline{2-5}
% 	& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
% 	6  & 0.0820 & 1.0878 & 0.0065 & 0.9088\\
% 	10 & 0.1287 & 1.7429 & 0.0129 & 1.4614  \\
% 	20 & 0.2402 & 3.3721 & 0.0228 & 2.8278  \\
% 	40 & 0.4201 & 6.7092 & 0.0442 & 5.5682\\
% 		\specialrule{.1em}{.05em}{.05em} 
% 	\end{tabular}
% \end{table} 
\begin{comment}
\begin{table}[!htb]
	\caption{Comparison between MP-BM-LSH and MP-RW-LSH(EH3) on synthetic dataset. $M=7$, $W=100$}\label{tab:feigen_vs_dyadic}
	\centering
	\begin{tabular} {@{}c c c c c@{}}
		\specialrule{.1em}{.05em}{.05em} 
		\multirow{2}{*}{$L$} & \multicolumn{2}{c}{MP-BM-LSH}  & \multicolumn{2}{c}{MP-RW-LSH (EH3)} \\\cline{2-5}
		& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
		6  & 0.0820 & 1.03+0.06 & 0.0065 & 0.85+0.06\\
		10 & 0.1287 & 1.65+0.10 & 0.0129 & 1.37+0.10  \\
		20 & 0.2402 & 3.17+0.20 & 0.0228 & 2.64+0.19  \\
		40 & 0.4201 & 6.26+0.45 & 0.0442 & 5.18+0.40\\
		\specialrule{.1em}{.05em}{.05em} 
	\end{tabular}MP-RW-LSH (precomputed) and MP-RW-LSH (EH3) on synthetic Enron dataseComparison between two different MP-RW-LSH
\end{table}\end{comment}
\begin{table}[!htb]
\caption{Original vs EH3-augmented. }\label{tab:feigen_vs_dyadic_another}
\centering
%\begin{tabular} {@{}c c c c c@{}}
%\specialrule{.1em}{.05em}{.05em} 
%\multirow{2}{*}{$L$} & \multicolumn{2}{c}{Precomputed}  & \multicolumn{2}{c}{EH3} \\\cline{2-5}
%& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
%10 & 0.1111 & 2.64+2.42 & 0.0100 & 0.64+1.12  \\
%15 & 0.1647	& 4.09+4.98 & 0.0147 & 1.05+1.64 \\
%20 & 0.2080	& 4.70+8.21 & 0.0180 & 1.25+2.16  \\
%\specialrule{.1em}{.05em}{.05em} 
%\end{tabular}
\begin{tabular} {@{}c | c c c c@{}}
	\specialrule{.1em}{.05em}{.05em} 
	 \multicolumn{2}{c} {$L$ } & 10 & 15 & 20 \\
	\specialrule{.1em}{.05em}{.05em} 
	  \multirow{2}{*}{Recall} &original & 0.1111 & 0.1647 & 0.2080\\\cline{2-5}
 &EH3-augmented& 0.0100& 0.0147 & 0.0180	\\
	\specialrule{.1em}{.05em}{.05em} 
\end{tabular}
\end{table}  
% \begin{table}[!htb]
% 	\caption{Comparison results on Enron dataset with synthetic queries. }\label{tab:feigen_vs_dyadic_another}
% 	\centering
% 	\begin{tabular} {@{}c c c c c@{}}
% 		\specialrule{.1em}{.05em}{.05em} 
% 		\multirow{2}{*}{$d$ } & \multicolumn{2}{c}{Precomputed}  & \multicolumn{2}{c}{EH3} \\\cline{2-5}
% 		& Recall & Query Time (ms) & Recall & Query Time (ms) \\\specialrule{.1em}{.05em}{.05em} 
% 		6400  & 0.5880 & 10.58+2.77 & 0.4321 & 6.41+1.01 \\
% 		8400 & 0.1709 & 6.68+2.35 & 0.1109 & 3.25+1.01  \\
% 		13300 & 0.0208	& 2.44+2.14 & 0.0019 & 0.65+1.01  \\
% 		16600 & 0.0084	& 1.33+2.10 & 0.0001 & 0.20+1.02 \\
% 		\specialrule{.1em}{.05em}{.05em} 
% 	\end{tabular}
% \end{table} 
% in the worst casethe Audio dataset (to define in \autoref{subsec:exp_set}). Each query is generated by conduct the following experiment in in the worst cases
%$M=9$, $W=122$between MP-GRW-LSH and MP-RW-LSH(EH3)

\begin{comment}
Description for varying distance: To show how the performance of EH3-based MP-RW-LSH degrades, we compare it  with the vanilla MP-RW-LSH with precomputed tables~\cite{mprwlsh}. %on the  dataset . 
In the experiments, we use Enron (see \autoref{tab:dataset-stats}) as the dataset $\mathcal{D}$, and generate \SI{10000} synthetic queries from the following procedure for each $d$. First, we randomly sample one point from the Enron database. Then, we generate the query point from randomly choosing one coordinate of the sampled data point and adding $d$ while keeping other coordinates unchanged, similar to the restriction above. %which is a variable parameter reflecting how far the query is from its neareat neighborroughly the position of the first ``valley'' in \autoref{fig:coll_prob}, to this coordinate value. MP-BM-LSH (from dyadic simulation) and MP-RW-LSH (from EH3) with different number of hash tables 
For different distance value $d$, the recalls and query times of both algorithms reported in~\autoref{tab:feigen_vs_dyadic} are averaged for these \SI{10000} queries.
We use the same index structure (hash tables) as in \autoref{sec:eva}, with the same set of parameters $M=9$, $T=100$, $W=122$. We show how recall and query time (written as $t_1+t_2$) change when  $d$ increases.\end{comment}

%As an example of the worst case, we generate the distance between the data and query points areplease refer to \autoref{subsec:ann-comp-algorithmsfor the meaning of these parameters)



%\textbf{Huayi Paragraph for the generation of synthetic dataset: \autoref{fig:distcomp} clearly shows that the success probability of EH3-based LSH is close to 0 for distance equal to 17600 when hash bucket width $W=100$. Based on this fact, we generate synthetic dataset where the distance of each query point to its corresponding nearest neighbor is 17600. More precisely, we first randomly sample one point from database. Then we generate the query point from randomly choosing one coordinate of the sampling point and adding 17600 on the coordinate value of this point. We use such generation process in order to achieve the similar success probability value as shown in \autoref{fig:distcomp}. We generate 1000 different query points and report the query performance of Feigenbaum and Dyadic on the synthetic dataset with different number of hash tables in~\autoref{tab:feigen_vs_dyadic}.}$M=9$, $W=122$index structure (hash tables) , with the same, which is roughly the position of the first ``valley'' in \autoref{fig:coll_prob},

We illustrate this ``fall into the valley'' effect by performing the following controlled ANNS-query experiment involving both 
the original and the  EH3-augmented MP-RW-LSH.  
%To show how the performances of EH3-based MP-RW-LSH (EH3-based for short in the sequel) degrades, we compare it  with the original MP-RW-LSH with precomputed tables~\cite{mprwlsh} (Precomputed for short).
In this experiment, we use Enron (see \autoref{tab:dataset-stats}) as the dataset $\mathcal{D}$ and generate \SI{10000}{} synthetic queries that target a 
``statistical fall'' distance
$D$ = \SI{13300}{}.  This $D$ is not in the middle of the first ``valley'' (between \SI{16000}{} and \SI{17000}{}) shown in~\autoref{fig:coll_prob} (for the $s_j = 0$ case)
for the following reason.
Even when $D$ is fixed, the value of an EH3-generated range-sum 
$S^{\tau_j}[s_j, s_j + D]$, and hence the shape of the corresponding collision probability curve, varies when $s_j$ varies (as 
it does in this experiment), so this $D$ optimizes, to some extent, the probability of ``fall'' over the set of $s_j$ values that are actually encountered.
% this $D$ is not in the middle the first ``valley'' shown \autoref{fig:coll_prob}).  
Each query is generated as follows.  First, we randomly sample a point $\vec{\mathbf{s}}$ from $\mathcal{D}$.  Then, we pick a dimension $j$ uniformly at
random (out of the $m$ dimensions), and set the query point $\vec{\mathbf{q}}$ such that $\vec{\mathbf{q}}$ is identical to $\vec{\mathbf{s}}$ in every dimension except the $j^{th}$, where $q_j = s_j + D$.
%Note that despite our ``statistically targeted push'', 
%only a small percentage of query points actually ``fall into the valley'', 
%and hence we are not overly ``exaggerating'' EH3's damaging effect here.
%generate the query point from randomly choosing one coordinate of the sampled data point and adding \SI{13300}{} to this coordinate value while keeping other coordinates %unchanged, similar to the restriction above. 
For both the original and the EH3-augmented, we use the same set of parameters $M=9$, $T=100$, $W=122$ as in~\autoref{sec:eva}, and report their average 
recalls (over these \SI{10000}{} queries)
under the same set of $L$ (number of hash tables) values.
\autoref{tab:feigen_vs_dyadic_another} shows that recall values of the original are between $11.1$ and $11.6$ times larger than those of EH3-augmented. 

%Note that here the recalls are lower than those in~\autoref{sec:eva}, because $d$, the distance between the query point and its nearest neighbor is \SI{13300}{}, which corresponds with the ``valley'' in \autoref{fig:coll_prob}, are ??? times of those typical in ~\autoref{sec:eva}. Under such a large distance, the recalls of EH3-based is approximately equal to $0$ while Precomputed still have recalls around $0.1$. 

\begin{comment}
Therefore, the performance of EH3-based is not robust, even if its query times may be shorter than those of Precomputed.
{\bf JFM: I suggest removing ``query times'', because the story is distracting.}
For query efficiency, EH3-based has a shorter $t_1$ than Precomputed, because it hardly finds any candidate.  As we will shown later in \autoref{sec:eva}, we have found that $t_1$ is roughly linear to the number of candidates found in probing the buckets. Its $t_2$ is also shorter, because it is faster to compute a range-sum by EH3 in this case than to read from the precomputed table in DRAM.
\end{comment}

%\textbf{Original description:\autoref{tab:feigen_vs_dyadic_another} clearly shows that when $d=6400$, a typical distance for queries in the real dataset \autoref{sec:eva}, the recall of EH3-based is lower than that of vanilla MP-RW-LSH by 1.4. This difference becomes more pronounced when $d$ increases. For example, when $d=$\SI{13300}{}, vanilla MP-RW-LSH achieves recall $0.0208$, but recall value of EH3-based MP-RW-LSH is only $0.0019$, which is 10.9 times smaller than the recall value of vanilla MP-RW-LSH. This corresponds with the ``valley'' in \autoref{fig:coll_prob}, where success probability of EH3-based MP-RW-LSH is approximately equal to 0 where vanilla MP-RW-LSH still have success probability around 0.1. For query efficiency, EH3 has a shorter $t_1$ than vanilla, because it hardly finds any candidate. For example (\textbf{Huayi: As we will shown later in \autoref{sec:eva}}) we have found that $t_1$ is roughly linear to the number of candidates found in probing the buckets. Its $t_2$ is also shorter, because it is faster to compute a range-sum by EH3 in this case than to read from the precomputed table in DRAM.}

%\autoref{tab:feigen_vs_dyadic_another} clearly shows that, for the same number of hash tables, EH3 has a shorter $t_2$ than DST by a factor of $4.1$ to $4.9$, which is because its algorithm is simpler in using integer operations only and no transforms, and a shorter $t_1$ by a factor of $3.2$ to $4$, which is because it hardly finds any candidate. We have found that $t_1$ is roughly linear to the number of candidates found in probing the buckets. The $t_1$ of DST on the first row of  \autoref{tab:feigen_vs_dyadic_another} with that on the third column of \autoref{tab:perf} measured from normal queries, 

 %times that of EH3, the former can achieve much better accuracy ($9.1$ to $10.1$ times as high recall) than  the latter.
%$t_1$ is shorter for EH3, because it returns fewer candidates.
 
 %Under these schemes, the distribution of $f_{\mathbf{V}}(\mathbf{x})  - f_{\mathbf{V}}(\mathbf{q})$ is far from Gaussian, which directly degrades the performance. The GRW-LSH algorithm


\subsection{Our Clean Solution: MP-GRW-LSH}\label{sec:grwlsh}

%We can certainly solve 
Again we fix $\vec{\mathbf{s}}$ and $\vec{\mathbf{q}}$ that are $d_1$ apart in $L_1$ distance.
The ERS problem in RW-LSH can be solved using our RW-DST as follows.
Each DST instance (one for each random walk sequence) is generated using a different (cheap)  
$2$-wise independent hash function at each of the $\log_2 U$ levels.  This way, 
each range-sum $S^{\tau_j}[q_j, s_j)$, that is a part of $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}})$, is a strict $|s_j - q_j|$-step random walk according to \autoref{cor:stdist}, and hence $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}})$ is a
strict $|s_j - q_j|$-step random walk.   
Since the pdf of $f(\vec{\mathbf{s}}) - f(\vec{\mathbf{q}})$ statistically defines an RW-LSH scheme, the RW-DST-augmented RW-LSH is statistically equivalent to the original RW-LSH.  

%However, as shown in Table~\ref{tab:perf}, splitting a random walk RV is relatively expensive operation.

\begin{comment}
to generate the underlying range sums.  
Since the behavior of RW-LSH is determined entirely by the pdf of 

 above, because by  \autoref{cor:stdist}, a hashing-based DST with cheap two-wise independent low-level hash functions guarantees that $S^\tau[q, s)$ follows the same distribution as a $|q - s|$-step strict random walk, which %is exactly what is needed by ANNS.
%In \autoref{sec:dsthash},  that a surprisingly cheap implementation of DST that uses  with two-wise independence 
%Therefore, by maintaining $m$ independent instances of such DSTs, one for each random walk $\tau$, we have an efficient DST-based implementation of RW-LSH that
%Therefore, we can evaluate $f(\mathbf{s})$ by generating the range-sum of each random walk $S^{\tau_j}[0, s_j)$ with the method described inn order to generate range-sums of single-step random walks that has the same distribution as ``real'' random walks,  and using . on the $j^{th}$ coordinate this DST uses t.I, which uses the definition of splits in \autoref{sec:randw} and l This leads to the following This implementation , because each of the range-sums $S^{\tau}[q, s)$ is a  random walk by.the DST-based GRW-LSH (defined below) is even better in thatand 
%does not need the precomputed tables and guarantees  the $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$ to be a strict$d_1$-step random walk, which 
is sufficient for all the theoretical efficacy guarantees of RW-LSH as we have shown above.
This is already a desirable solution, yet we will show that it is even better to replace RW-LSH with 
\end{comment}

We propose an even better solution called GRW-LSH (Gaussian random walk LSH).
% that is based on our ERS-Gaussian solution.
In GRW-LSH, a raw hash value function $f$ is defined in the same way as in RW-LSH, except each random walk sequence $\tau_j$ is replaced by 
a Gaussian random walk (GRW) sequence $\xi_j$.  In a GRW sequence, the underlying RVs are i.i.d. with standard Gaussian distribution instead.
%as just explained.  mutually independentin a $v$-step random walk
As a result, each $s_j$-step random walk along $\tau_j$ is replaced by an $s_j$-step GRW along $\xi_j$.
% and the other definitions, such as $g(\vec{\mathbf{s}})$, remain the same.
This way, $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$, which as just explained has the distribution of a $d_1$-step strict random walk %and has a probability distribution very close to the Gaussian distribution $N(0, d_1)$
under RW-LSH, now has Gaussian distribution $\mathcal{N}(0, d_1)$ under GRW-LSH.
Since the former distribution is always statistically close to the latter distribution and especially so when $d_1$ is reasonably large
(say when $d_1 > 25$), GRW-LSH  is statistically very close to RW-LSH.
As a result, its multi-probe extension MP-GRW-LSH has nearly the 
same query efficacy as MP-RW-LSH, as will be shown in \autoref{sec:eva}.  

It is straightforward to implement (the step of hashing $\vec{\mathbf{q}}$ in) GRW-LSH:   Each range-sum $S^{\xi_j} [0, q_j)$ is computed using our Gaussian-DST.
As explained above, using a different
$2$-wise independent hash function at every level of a DST instance is enough to ensure statistical equivalence (between the original GRW-LSH and
the Gaussian-DST-augmented GRW-LSH);  but for all practical purposes, we will use {\tt wyhash} functions instead.  
The Gaussian-DST-augmented GRW-LSH is a better solution than the RW-DST-augmented RW-LSH, since to compute a Gaussian range-sum is several times faster than to compute a random walk range-sum, as shown in \autoref{tab:perf}.

%Therefore, we focus on the DST-based efficient implementation of only GRW-LSH, which we simply refer to as GRW-LSH in the sequel, and we refer to the original scheme in~\cite{mprwlsh} with precomputed tables as RW-LSH. 

\begin{comment}

%replacing a $v$-step random walk (in RW-LSH) by a $v$-step(in GRW-LSH)ERS solution for 
The primary motivation for using Gaussian random walks  is that the it 
can be efficiently computed using our Gaussian-DSTs. 
Our measurements 
show that each dyadic split operation for Gaussian 
can be accomplished in a couple of nanoseconds.  Hence even when $v$ is as large as $2^{20}$, the $20$ dyadic splits involved to 
compute the $v$-step Gaussian random walk take a total of roughly \SI{95.1}{ns} to compute.  In comparison, in RW-LSH, even to read a precomputed value from the gigantic 
table (stored in DRAM) takes tens of nanoseconds.  Hence GRW-LSH usually affords faster LSH computation while paying zero storage cost for it.  
This said, we do not consider
GRW-LSH a separate contribution to the LSH literature, since it is conceptually very close to RW-LSH.  We consider it a contribution to the ERS literature as a novel application of 
our ERS-for-Gaussian solution.



%[to move with the closeness paragraph several paragraphs before]
%Since the latter is always statistically close to the former and especially so when $v$ is reasonably large
%(say when $v > 25$), the resulting GRW-LSH (... LSH) is statistically close to RW-LSH.  

We stress the difference between our GRW-LSH and the traditional GP(Gaussian projection)-LSH~\cite{Datar_LSH_2004}, which also uses Gaussian random variables, that GP-LSH  is suitable for querying on $L_2$ distance, but our GRW-LSH focuses on $L_1$ distance. In GP-LSH, the raw hash value $f(\mathbf{s})$ is defined as $\vec{\mathbf{s}}\cdot \vec{\bm{\eta}}$, where ``$\cdot$'' is the inner product (which is mathematically a {\it projection}) and $\vec{\bm{\eta}}=\langle \eta_1,\cdots, \eta_m\rangle$ is an $m$-dimensional i.i.d. standard Gaussian random vector (fixed after generation). The most stressed difference is that in GRW-LSH, the $j^{th}$ dimension contributes to $f(\mathbf{s})$ a $s_j$-step Gaussian random walk, which is the sum of $s_j$ i.i.d. standard Gaussian RVs, whereas in GP-LSH, it contributes $s_j\eta_j$, which is $s_j$ times a fixed Gaussian RV $\eta_j$. 
Therefore, for GP-LSH $f(\vec{\mathbf{s}})  - f(\vec{\mathbf{q}})$ follows $\mathcal{N}(0, d_2^2)$, which reflects the $L_2$ distance between $\vec{\mathbf{s}}$ and $\vec{\mathbf{q}}$ instead of the $L_1$ distance.

\end{comment}


\begin{comment}
[duplicate]In \autoref{sec:dsthash}, we have shown that a surprisingly cheap implementation of DST that uses low-level hash functions with two-wise independence guarantees the same distribution of range-sums as a ``real'' random walk.
Therefore, by maintaining $m$ independent such DSTs, one for each random walk $\tau$, we have an efficient DST-based implementation of RW-LSH that
%Therefore, we can evaluate $f(\mathbf{s})$ by generating the range-sum of each random walk $S^{\tau_j}[0, s_j)$ with the method described inn order to generate range-sums of single-step random walks that has the same distribution as ``real'' random walks,  and using . on the $j^{th}$ coordinate this DST uses t.I, which uses the definition of splits in \autoref{sec:randw} and l This leads to the following This implementation 
does not need the precomputed tables and guarantees  the $f(\mathbf{s})  - f(\mathbf{q})$ to be a $d_1$-step random walk, because each of the range-sums $S^{\tau}[q, s)$ is a $|q - s|$-step random walk by \autoref{cor:stdist}.
%Obviously, we can avoid the precomputed table by directly generating the range-sum $S^{\tau}[0, t)$ of each random walk $\tau$ with dyadic simulation as . study the efficient implementation with dyadic simulation of only
This DST-based RW-LSH implementation may be useful in some applications that restrict the hash values to integers. However, we will show that the DST-based GRW-LSH (defined below) is even better in that it is faster and as accurate. 
As a result, we focus on the DST-based efficient implementation of only GRW-LSH, which we simply refer to as GRW-LSH in the sequel, and we refer to the original scheme in~\cite{mprwlsh} with precomputed tables as RW-LSH in the sequel. 


[duplicate] In GRW-LSH, the raw hash value function $f$ is %a random walk projection 
parameterized by a vector of $m$ mutually independent Ganssian random walks $\bm{\zeta} = \langle \zeta_1, \cdots, \zeta_m \rangle$. %, which we unrigorously refer as ``Brownian with Gaussian steps motions'' in the sequel to distinguish from the random walks with integer steps in RW-LSH. 
Each  $\zeta_j$ is defined by a sequence of steps that are i.i.d. standard Gaussian RVs, which differs from the (integer-valued random walk) $\tau_j$ at the marginal distribution of each step. Given a data point $\mathbf{s} = \langle s_1, s_2, \cdots, s_m \rangle$, $f(\mathbf{s})$ is defined as $\sum_{j=1}^m S^{\zeta_j}[0, s_j)$.
Similarly, GRW-LSH requires that each $s_j$, $j=1,2,\cdots, m$, be a nonnegative integer. GRW-LSH achieves similar accuracy in ANNS-$L_1$ as RW-LSH, because Gaussian random walks are statistically close to integer-valued random walks when the number of steps is large. %and it is better suited for a DST-based implmentation, 

[duplicate] Our DST-based GRW-LSH implementation is the same as the DST-based RW-LSH above, except that it uses the split definitions in \autoref{sec:gauss} to generate Gaussian steps instead of single-step random walks in \autoref{sec:randw}. It runs faster than the DST-based RW-LSH, because Gaussian distribution is  ``nice'', so its range-sums can be generated four times as fast as those of single-step random walks (shown in \autoref{sec:dyaperf}). %uses the splits described in~ and low-level hash function that are two-wise independent for each Brownian motion $\zeta$, 
It also has a similar guarantee as above that
$f(\mathbf{s}) - f(\mathbf{q}) = \sum_{j=1}^m (S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j))$ is a Gaussian random walk of $\sum_{j=1}^m |s_j-q_j| = d_1$ steps and follows Gaussian distribution $\mathcal{N}(0, d_1)$, for the following 
reason:  For each $j$, $j = 1, 2,\cdots, m$, $S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j)$ equals to either $S^{\zeta_j}[q_j, s_j)$ or $S^{\zeta_j}[s_j, q_j)$ depending on which one in $s_j$ and $q_j$ is greater, which is always an
$|s_j - q_j|$-step Gaussian random walk along the sequence $\zeta_j$, and these 
$m$ Gaussian random walks are mutually independent since they are along different sequences. 
The distribution of $f(\mathbf{s}) - f(\mathbf{q})$ resembles its counterpart in GP-LSH~\cite{Datar_LSH_2004} and differs only in the variance, since the latter follows $\mathcal{N}(0, d_2^2)$ where %$\mathcal{N}(0, d_2^2)$. 
$d_2^2$ is the squared $L_2$ distance between $\mathbf{s}$ and $\mathbf{q}$, \ie $d_2 ^2= \sum_{j=1}^m (s_j-q_j)^2$. This resemblance is important, because it implies that GRW-LSH is an LSH function similarly to GP-LSH and inherits GP-LSH's multi-probe extension~\cite{lv2007multiprobe}, which greatly reduces the number of hash tables for reaching a target query accuracy. We call the version of GRW-LSH with multi-probe extension MP-GRW-LSH in the sequel.
\end{comment}

%Obviously, we can avoid the precomputed table by directly generating the range-sum $S^{\tau}[0, t)$ of each random walk $\tau$ with dyadic simulation as . study the efficient implementation with dyadic simulation of only
%This DST-based RW-LSH implementation may be useful in some applications that restrict the hash values to integers. 



%In GRW-LSH, the raw hash value function $f$ is %a random walk projection 
%parameterized by a vector of $m$ mutually independent Ganssian random walks $\bm{\zeta} = \langle \zeta_1, \cdots, \zeta_m \rangle$. %, which we unrigorously refer as ``Brownian with Gaussian steps motions'' in the sequel to distinguish from the random walks with integer steps in RW-LSH. 
%Each  $\zeta_j$ is defined by a sequence of steps that are i.i.d. standard Gaussian RVs, which differs from the (integer-valued random walk) $\tau_j$ at the marginal distribution of each step. Given a data point $\mathbf{s} = \langle s_1, s_2, \cdots, s_m \rangle$, $f(\mathbf{s})$ is defined as $\sum_{j=1}^m S^{\zeta_j}[0, s_j)$.
%Similarly, GRW-LSH requires that each $s_j$, $j=1,2,\cdots, m$, be a nonnegative integer. GRW-LSH achieves similar accuracy in ANNS-$L_1$ as RW-LSH, because Gaussian random walks are statistically close to integer-valued random walks when the number of steps is large. %and it is better suited for a DST-based implmentation, 



%Let $\mathbf{q}= \langle q_1, q_2, \cdots, q_m \rangle$ be the query point.  
%We denote as $d_1$ the value of the $L_1$ distance between $\mathbf{s}$ and $\mathbf{q}$, that is, $d_1 = \sum_{j=1}^m |s_j-q_j|$;
%$d_1$ is a nonnegative integer since every $s_j$ and $q_j$ is.
%Then 
%Our DST-based GRW-LSH implementation is the same as the DST-based RW-LSH above, except that it uses the split definitions in \autoref{sec:gauss} to generate Gaussian steps instead of single-step random walks in \autoref{sec:randw}. It runs faster than the DST-based RW-LSH, because Gaussian distribution is  ``nice', so its range-sums can be generated four times as fast as those of single-step random walks (shown in \autoref{sec:dyaperf}). %uses the splits described in~ and low-level hash function that are two-wise independent for each Brownian motion $\zeta$, 
%It also has a similar guarantee as above that
%$f(\mathbf{s}) - f(\mathbf{q}) = \sum_{j=1}^m (S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j))$ is a Gaussian random walk of $\sum_{j=1}^m |s_j-q_j| = d_1$ steps and follows Gaussian distribution $\mathcal{N}(0, d_1)$, for the following 
%reason:  For each $j$, $j = 1, 2,\cdots, m$, $S^{\zeta_j}[0, s_j) - S^{\zeta_j}[0, q_j)$ equals to either $S^{\zeta_j}[q_j, s_j)$ or $S^{\zeta_j}[s_j, q_j)$ depending on which one in $s_j$ and $q_j$ is greater, which is always an
%$|s_j - q_j|$-step Gaussian random walk along the sequence $\zeta_j$, and these 
%$m$ Gaussian random walks are mutually independent since they are along different %sequences. 
%The distribution of $f(\mathbf{s}) - f(\mathbf{q})$ resembles its counterpart in GP-LSH~\cite{Datar_LSH_2004} and differs only in the variance, since the latter follows $\mathcal{N}(0, d_2^2)$ where %$\mathcal{N}(0, d_2^2)$. 
%$d_2^2$ is the squared $L_2$ distance between $\mathbf{s}$ and $\mathbf{q}$, \ie $d_2 ^2= \sum_{j=1}^m (s_j-q_j)^2$. This resemblance is important, because it implies that GRW-LSH is an LSH function similarly to GP-LSH and inherits GP-LSH's multi-probe extension~\cite{lv2007multiprobe}, which greatly reduces the number of hash tables for reaching a target query accuracy.

%We now describe the implementation of each Brownian motion $\zeta$ via dyadic simulation (here we drop the subscript $j$, with the understanding that each $\zeta_j$ is an independent instance of $\zeta$). Unlike in data streaming, a surprisingly cheap implementation of dyadic simulation has all theoretical guarantees of BM-LSH on ANNS-$L_1$, even though its singletons are not mutually independent. In this implementation, the random strings $C_\alpha$ (in \autoref{sec:overview}) are generated with a two-wise hash function on each level of the simulation tree, so a simulation tree takes only $O(\log U)$ space and generates each range-sum in $O(\log U)$ time. According to \autoref{th:stdist}, this implementation guarantees that each range-sum $S^{\zeta} [a, b)$ follows distribution $\mathcal{N}(0, b-a)$, so for each $a, b = 0, 1, \cdots, U-1$ (without loss of generality, suppose $b> a$), $\zeta(b) - \zeta(a)$ has the same distribution of an
%$(b-a)$-step Brownian motion.
%This is sufficient to show that $f(\mathbf{s}) - f(\mathbf{t})$ follows $\mathcal{N}(0, d_1)$ and all theoretical guarantees of BM-LSH above.


==> sections/nisan-extra.tex <==
============== old below

[duplicate]To begin with, we show some backgrounds on Nisan's PRNG. According to~\cite{stabledist}, for any algorithm in $space(S)$ (any finite state machine (FSM) with at most $2^S$ states) that uses $R$ (independent and uniform) random bits, (the algorithm consumes these bits in $O(S)$ chunks and one chunk at a time) Nisan's PRNG can expand a random seed of $O(S\log R)$ bits into $R$ pseudorandom bits that are indistinguishable from real random bits to that algorithm. The meaning of ``indistinguishable'' is as follows: We treat the distribution of the running result as a vector $D(X)$ with $2^S$ coordinates depending on the distribution of the input $X$. We define that the random variable $X$ is uniformly randomly drawn from $\{0, 1\}^R$, and $Y$ is the generating result of Nisan's PRNG from a uniform random seed of $O(S\log R)$ bits. According to~\cite{stabledist}, the following bound on the $L_1$ difference (or total-variation distance) between two vectors $D(X)$ and $D(Y)$ holds
\begin{equation}
	\|D(X) - D(Y)\|_1 \leq 2^{O(S)}.
\end{equation}
Nisan's PRNG can be implemented with $O(S)$ storage, apart from the $O(S\log R)$ random bits, and any chunk of $O(S)$ bits can be computed using $O(\log R)$ arithmetic operations on $O(S)$-bit words. 

For estimating the $L_1$-norm, we focus on one accumulator $A$ (dropping the superscript $j$) of the online stage of \autoref{algo:indyk-new}. The random variables $X_0, X_1, \cdots, X_{U-1}$ that generate the range-updates are generated by a DST implemented by Nisan's PRNG.
We will show that the online stage, using range-updates generated from the DST instead of point-updates that are directly from Nisan's PRNG, is still space-bounded, so the arguments in Indyk's original proof still holds.
%the raw statistics of this accumulator after the online stage is indistinguishable from the Cauchy random variables in the ideal case.
%We show that  that in the ideal case where $X_0, X_1, \cdots, X_{U-1}$ are i.i.d., by showing that .  as ~\cite{stabledist}only need tofor each $j=1,2,\cdots, r$ , and its final state refers to the raw statistics for estimation
Therefore, our solution achieves $(\epsilon, \delta)$ approximation for the same reason Indyk's point-update algorithm does.

================= old above
=============== old below

[duplicate]  (using floating-point numbers instead of infinitely precise real numbers), so the running result of the online stage (the state of accumulators) from Nisan's PRNG is indistinguishable from the ideal case when they rely on independent random bits. 
%That probability would be negligibly small when $S$ is logarithmic to $U$, so our algorithm (equivalent to a space-bounded one) cannot distinguish the difference between uniform random bits and Nisan's PRNG. 
Therefore, any estimator in the offline stage will have the same theoretical guarantee as if the accumulators were calculated from independent random variables.


% For any possible running result of the algorithm, the probability of reaching this result (with the ideal scheme) when truly random bits are used differs from the probability of reaching the same result (with the practical scheme) when the random bits are generated by Nisan's PRNG by at most $2^{-cS}$ for some constant $c$ that is independent of $S$ and $R$. \textcolor{red}{This is an intuitive explanation of the total variation distance (L1 distance in distribution) claim in Indyk's paper.} That probability would be negligibly small when $S$ is logarithmic to $U$.
%If we treat the computation of each estimate $\hat{L}_0$ as a run of the target algorithm, whose success probability is roughly $3/4$, this small difference in the success probability is negligible for 
%With $S=\Omega(\log U)$, the probability that the ideal scheme succeeds but the practical scheme fails is at most $O(U^{-c})$, which is negligible in
%\textcolor{blue}{(from Indyk's paper)}


\begin{comment}
+++++++++++++++++++++++++++++++++++++++++\\
----------------------------------------------------------------------------------------------------- 

\textcolor{teal}{According to \cite{stabledist}, for any algorithm in $space(S)$ that uses $R$ (independent and uniform) random bits, (the algorithm consumes these bits in $O(S)$ chunks and one chunk at a time) Nisan's PRNG can expand $O(S\log R)$ random bits into $R$ bits that are indistinguishable from independent random bits from that algorithm. The meaning of ``indistinguishable" is as follows: For any possible running result of the algorithm, the probability of reaching this result (with the ideal scheme) when truly random bits are used differs from the probability of reaching the same result (with the practical scheme) when the random bits are generated by Nisan's PRNG by at most $2^{-cS}$ for some constant $c$ that is independent of $S$ and $R$. \textcolor{red}{This is an intuitive explanation of the total variation distance (L1 distance in distribution) claim in Indyk's paper.} That probability would be negligibly small when $S$ is logarithmic to the size of universe..}

-----------------------------------------------------------------------------------------------------\\
+++++++++++++++++++++++++++++++++++++++++\\
\end{comment}

\textbf{We have to assume each random sample that follows exponential (or Cauchy, Gaussian) distribution can be calculated within a relative error of $\epsilon$ with high probability from a chunk of $K\ll U$ random bits, and these samples, after the transformation, can be stored in a word of $B=O(\log\frac{1}{\epsilon} + \log\log U)$ bits (suppose as a floating number with relative precision $O(\epsilon)$ and average $1/U$).} 

%For $L_1$ estimation, the rejection sampling technique of generating range-summable Cauchy random variables has a success probability of $1/2$ per round, so in the worst case we have to prepare $O(\log \frac{U}{\delta_1})$ samples to bound the failure rate to $\delta_1 = \frac{\epsilon^2\delta}{\log1/\delta}$ (by union bound). This only inflates the number of chunks by a small ($O(\log \frac{U}{\delta\epsilon})$) multiplicative factor, which would become just a small additive term after taking the logarithm on the number of chunks.

%Storing $U$ independent random samples $B$ and $W$ as required by \autoref{lem:minexp} takes $O(U(\log\frac{1}{\epsilon} + \log U))$ space.
%In this section, we use Nisan's PRNG \cite{nisan}, which has been described in \autoref{sec:srcrandom}, to reduce the storage demand to $O(\log \frac{1}{\epsilon}\log^2 U)$ without sacrificing time complexity too much.

%Recall that the PRNG introduces at most $O(2^{-cS})$ probability of failure, where $S$ is the space of the algorithm that uses PRNG. In our case, we treat the computation of each estimate $\hat{L}_0$ as a run of the target algorithm, whose success probability is roughly $3/4$. Then, this small difference in the success probability is negligible for $S=\Omega(\log U)$.

%Nisan's generator can generate bit sequences that is indistinguishable from random bits to any algorithm that uses bounded space. More specifically, for any algorithm in $space(S)$ that uses $R$ (independent and uniform) random bits, (because of the space limit, such an algorithm can only accept these bits as a sequence of $O(S)$ chunks.) Nisan's generator can expand $O(S\log R)$ random bits into $R$ bits that is indistinguishable from independent random bits from the algorithm. The meaning of ``indistinguishable" is as follows: For any possible running result, the difference of the probability of reaching that result between the idealized algorithm (that uses truly random bits) and the practical algorithm (that uses Nisan's generator) is at most $2^{-cS}$ for some constant $c$ that is independent of $S$ and $R$. \textcolor{red}{This is an intuitive explanation of the total variation distance (L1 distance in distribution) claim in Indyk's paper.} If we treat the computation of each estimate $\hat{L}_0$ as a run of the target algorithm, whose success probability is roughly $3/4$, this small difference in the success probability is negligible for $S=\Omega(\log U)$.

%\textcolor{blue}{(from Indyk's paper)}
%Nisan's generator can be implemented with $O(S)$ storage, and any chunk of $O(S)$ bits can be computed using $O(\log R)$ arithmetic operations on $O(S)$-bit words. In our case, the number of random bits is $O(M(\log M + \log \frac{1}{\epsilon}))$for the original version of \autoref{algo:indyk-new}

Before proving the online stage with range-updates is space-bounded, we now recall the proof in~\cite{stabledist} that the online stage with point-updates is space-bounded. In the online stage, a deterministic function $\mathcal{F}(\cdot)$ transforms each random chunk $C_i$ to the random variable $X_i$ with Gaussian or Cauchy distribution, and %we use a large array of counters  to track effect of all updates, \ie $\sigma_i = \sum_{t:i\in[a_t, b_t)} \delta_t$ for $i=0,1,\cdots, U-1$. The value of 
the accumulator after the online stage equals $A=\sum_{i=0}^{U-1} \sigma_i X_i = \sum_{i=0}^{U-1} \sigma_i \mathcal{F}(C_i)$. The online stage can be converted to following space-bounded algorithm that has the same final state of the accumulator. First, the original input stream is ``collapsed'' to a stream of $(i, \sigma_i)$ in increasing order of $i = 0, 1, \cdots, U-1$, and second, Indyk's algorithm computes the accumulator using the collapsed stream as input. The first part can be naively implemented in $O(1)$ space and $U$ passes of the stream, which is fine, because \autoref{th:nisan} only requires the online stage to be an FSM, but does not care the running time of the FSM.
%which leads to exactly the same final state accumulator valu
%Note that  Therefore, we can ``collapse''  in small space and use the ``collapsed'' stream as input, because both streams lead to  (final state).  given the ``collapsed'' stream  as input
The second part is space-bounded, because it obviously satisfies the following two conditions. (1) Each chunk of random string $C_i$ is generated from Nisan's PRNG only once. (2) Maintaining one accumulator only needs small space $B$.

\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{figures/nisan.png}
	\caption{An illustration of the space-bounded DST.% For simplicity, only the prefixes of the stored range-sums are shown in the stacks. The blue line shows the path on which the space-bounded algorithm traverses the DST.
	}\label{fig:nisan}
\end{figure}

%When dyadic simulation is used in \autoref{algo:indyk-new}the collapsed input for the same reason using the collapsed stream  to satisfy the two conditions above, it needs to store
For the online stage with range-updates, we use a similar space-bounded conversion as above. The first part ``collapses'' the range-update stream to a point-update stream of $(i, \sigma_i)$ following the same format as above, and the second part takes the collapsed stream as input, generates each point-update (singleton $X_i$) in increasing order of $i$ one by one from the DST implemented with Nisan's PRNG. It stores 
the range-sum of every unused right-child after each split in a stack. Recall that in the simulation tree, the range-sum of any dyadic interval can be deterministically computed from the range-sum $S_\alpha$ and the random string $C_\alpha$ at its direct parent $\alpha$. Because the indices are increasing in the collapsed stream, the index of the next tuple  $i'$ is greater than $i$, the index of the last one. The path from root to $i'$ must diverge from the path to $i$ by selecting a right child instead of a left child at some point, so by storing the range-sum of all right children, we can always restart the simulation at the point of diverge.

In the following example shown in \autoref{fig:nisan}, the universe has size $U=16$, and the collapsed stream consists of the following indices $0, 3,4, 7,8,9,10$ (The increments $\delta_t$ are dropped, because they do not affect the proof). Each of such singleton is associated with the state of the stack at the moment it is generated. In the figure, only the prefixes are shown, but actually the corresponding range-sums $S$ are stored. The blue line shows the DST is traversed by the space-bounded second part to generate the target singletons. Starting at the root,
it takes four splits to generate $X_0$, which generates four right-children $1*$, $01*$, $001*$, and $0001$, but neither of them is used in computing $X_0$, so $S_{1*}, S_{01*}, S_{001*}$, and $X_1 = S_{0001}$ are stored in the stack.   
%In the example shown in \autoref{fig:nisan}, , each of which is associated with the state . The space-bounded DST outputs the singletons one by one in the increasing order for the same of simplicity, which is also fine, because the running time does not matter. 
After $X_0$ is generated, the next target is $X_3$, so the space-bounded DST pops $S_{0001}$ and recovers $S_{001*}$ from the stack, which is then split to $X_2$ and $X_3$. The next target is $X_4$, so it recovers $S_{01*}$, which generates $X_4$ in two splits and the two right-children $S_{011*}$ and $X_5 = S_{0101}$ are pushed to the stack. The next target is $X_7$, which is computed by recovering and splitting $S_{011*}$. After that, the value $S_{1*}$ is recovered to generate $X_8$, and so on.
%For example, when the collapsed stream contains four tuples $(i, \delta_i)$ as $(0, 2), (1, -2), (3, 7), (5, -7)$, the following sequence of evaluations and stack operations are called: push($S_{1*}$), push($S_{01*}$), push($S_{001}$), eval($X_0$), eval($X_1$), pop($S_{001}$), push($S_{011}$), eval($X_3$), pop($S_{011}$), pop($S_{01*}$), push($S_{11*}$), push($S_{101}$), eval($X_5$).
%The online stage with stacked dyadic simulation on the collapsed stream satisfies each range-sum pushed in the stack $S_{\alpha1}$ corresponds in one-to-one way to a split and to a random string $C_\alpha$ used in that split. , , so the online stage with dyadic simulation uses a bounded amount of space of , satisfying condition (2) above.
Condition (1) is satisfied, because during the online stage, each range-sum is pushed in the stack only once (as in the example above), so each random string, which is exclusive to one range-sum, is generated only once. Condition (2) is also satisfied with a space bound of $O(K+B\log U)$ (dominated by the second term), because the depth of the stack is $O(\log U)$, upper bounded by the depth of the simulation tree.




[duplicate] Since our data streaming algorithm % (except the rejection sampling one for $L_1$) 
requires at most $U$ such chunks, one for the sum of universe and $U-1$ for each non-leaf vertex, % (one for each possible dyadic interval $\alpha$ on the simulation tree), the space complexity of Nisan's PRNG isgenerating any range-update is 
Nisan's PRNG can generate all these chunks from a seed of  bits, and with $O(\log U)$ arithmetic operations of generating an arbitrary chunk. , and the generation of each random string $C$ takes $O(\log U)$ arithmetic operations on $O(B\log U)$-bit words. The time complexity of generating any range-sum from dyadic simulation, which takes $O(\log U)$ splits, is $O(B\log ^2 U)$ .This only inflates the complexity of DST from the most efficient implementation of hash functions by a factor of $O(\log U)$.

====================== old  above



\begin{comment}
show the overall space and time complexities for our data streaming algorithm. The space complexity to store all seeds of Nisan's PRNGs is $O(\frac{1}{\epsilon^2})\log\frac{1}{\delta}B\log U\log (UA)$ (which is the dominant term of memory complexity).
For each input tuple, the update of all sketches takes $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta}\log U\log UA)$ arithmetic operations. Note that this is the (worst case) complexity for a theoretical guarantee. In practice, we can use very fast hash functions (such as wyhash\footnote{\url{https://github.com/wangyi-fudan/wyhash}}) to generate random bits for the samples and observe nearly no degradation in performance. With these hash functions, the practical complexity of using dyadic simulation for estimating $L_0$ is $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta})$ space and $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta}\log U)$ time. 

The remaining problem is to show that our data streaming algorithm is space-bounded. It seems that our sketching algorithm (for a single sketch) is naturally in space($O(\log U+ \log1/\epsilon)$), because it only maintains a sketch in space $O(\log\frac{1}{\epsilon} + \log\log U)$ and processes samples of  $O(\log U + \log1/\epsilon)$ bits sequentially. However, we should pay attention to the caveat here: Nisan's generator works only for space(S) randomness testing algorithms that has only one-way access to the random bits (each random sample can be generated only once), whereas our sketching algorithm may view the same chunk repeatedly if the same dyadic interval is traversed multiple times as we process the input. 
%In particular, the random samples for the hash functions at the root is viewed for almost every input element. 

To show the correctness of using Nisan's generator, we have to convert our sketching algorithm to a model algorithm that only has one-way access to the random bits. The model algorithm is purely theoretic and we do not care about its running time, so it can process the input stream \emph{in any sequence} (as it is allowed to scan the stream for the scratch for the next desired input.) Recall that our input stream consists of disjoint dyadic intervals, so in particular, we assume the model algorithm processes these intervals in an order that their range-minimums can be generated by a one-way pre-order traversal of all vertices (and their randomness) of the simulation tree. 

We use the following example to illustrate our model algorithm. Suppose the universe $\mathcal{U} = [0, 16)$ and the input stream has two tuples $([5, 10), 3)$ and $([6, 12), 1)$. The first step of our model algorithm decomposes the two input intervals $[5, 10)$ and $[6, 12)$ into dyadic intervals (and merges the tuples for the same dyadic interval). The transformed input stream of dyadic intervals now becomes $([5,6), 3)$, $([6, 8), 4)$, $([8, 10), 3)$, $([8, 12), 1)$ (the prefixes of these dyadic intervals are $0101$, $011$, $100$ and $10$). The second step is to generate the range-sums of these dyadic intervals (and all ancestors) in the simulation tree by the following Depth First Search (DFS) order: $\mathcal{E}$, $0$, $01$, $010$, $0101$, $011$, $1$, $10$, 	$100$. The model algorithm uses the greatest amount of memory when generating $S_{0101}$, at which time it has to store the following random variables: $S_{\mathcal{E}}$, $W_{\mathcal{E}}$, $W_{0}$, $W_{01}$, $W_{010}$, $W_{0101}$.

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{figures/dfstree.png}
\caption{The nodes visited by DFS in the following example. }\label{fig:dfstree}
\end{figure}

In general, our model (space-bounded version) algorithm can return \emph{exactly the same} sketch $Y[k]$ while storing the samples of $O(\log U)$ ancestor vertices (maintaining state for DFS), which takes  $O(B\log U)$ bits in total (neglecting higher order logarithms). Therefore, the space bound for the equivalent model algorithm is $S=O(B\log U)$. With a properly configured Nisan's PRNG, the model algorithm cannot tell the difference between true random bits and Nisan's PRNG, and so cannot our data streaming algorithm.%we can generate the random bits with a Nisan's generator that performs $\tilde{O}(\log U)$ arithmetic operations on $\tilde{O}(\log\frac{1}{\epsilon}\log U)$-bit words for each random sample, and the size of the seed is $\tilde{O}(\log\frac{1}{\epsilon}\log^2 U)$.

Now we show the overall space and time complexities for our data streaming algorithm. The space complexity to store all seeds of Nisan's PRNGs is $O(\frac{1}{\epsilon^2})\log\frac{1}{\delta}B\log U\log (UA)$ (which is the dominant term of memory complexity).
For each input tuple, the update of all sketches takes $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta}\log U\log UA)$ arithmetic operations. Note that this is the (worst case) complexity for a theoretical guarantee. In practice, we can use very fast hash functions (such as wyhash\footnote{\url{https://github.com/wangyi-fudan/wyhash}}) to generate random bits for the samples and observe nearly no degradation in performance. With these hash functions, the practical complexity of using dyadic simulation for estimating $L_0$ is $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta})$ space and $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta}\log U)$ time. %, which matches the complexity of \cite{rangeeff} in terms of $U$, although our scheme is much simpler and requires no explicit finite field operations.
%(note: we can easily aggregate sketches from different sources, but \cite{rangeeff} cannot.)

+++++++++++++++++++++++++++++++++++++++++\\
----------------------------------------------------------------------------------------------------- 

\textcolor{teal}{Storing $U$ independent random samples $B$ and $W$ as required by \autoref{lem:minexp} takes $O(U(\log\frac{1}{\epsilon} + \log U))$ space.
In this section, we use Nisan's PRNG \cite{nisan}, which has been described in \autoref{sec:srcrandom}, to reduce the storage demand to $O(\log \frac{1}{\epsilon}\log^2 U)$ without sacrificing time complexity too much.
\\
Recall that the PRNG introduces at most $O(2^{-cS})$ probability of failure, where $S$ is the space of the algorithm that uses PRNG. In our case, we treat the computation of each estimate $\hat{L}_0$ as a run of the target algorithm, whose success probability is roughly $3/4$. Then, this small difference in the success probability is negligible for $S=\Omega(\log U)$.
\\
%Nisan's generator can generate bit sequences that is indistinguishable from random bits to any algorithm that uses bounded space. More specifically, for any algorithm in $space(S)$ that uses $R$ (independent and uniform) random bits, (because of the space limit, such an algorithm can only accept these bits as a sequence of $O(S)$ chunks.) Nisan's generator can expand $O(S\log R)$ random bits into $R$ bits that is indistinguishable from independent random bits from the algorithm. The meaning of ``indistinguishable" is as follows: For any possible running result, the difference of the probability of reaching that result between the idealized algorithm (that uses truly random bits) and the practical algorithm (that uses Nisan's generator) is at most $2^{-cS}$ for some constant $c$ that is independent of $S$ and $R$. \textcolor{red}{This is an intuitive explanation of the total variation distance (L1 distance in distribution) claim in Indyk's paper.} If we treat the computation of each estimate $\hat{L}_0$ as a run of the target algorithm, whose success probability is roughly $3/4$, this small difference in the success probability is negligible for $S=\Omega(\log U)$.
%\textcolor{blue}{(from Indyk's paper)}
%Nisan's generator can be implemented with $O(S)$ storage, and any chunk of $O(S)$ bits can be computed using $O(\log R)$ arithmetic operations on $O(S)$-bit words. In our case, the number of random bits is $O(M(\log M + \log \frac{1}{\epsilon}))$
It seems that our sketching algorithm (for a single sketch) is naturally in space($O(\log U)$), because it only maintains a sketch in space $O(\log\frac{1}{\epsilon} + \log\log U)$ and processes samples of  $O(\log U + \log1/\epsilon)$ bits sequentially. However, we should pay attention to the caveat here: Nisan's generator works only for space(S) randomness testing algorithms that has only one-way access to the random bits (each random sample can be generated only once), whereas our sketching algorithm may view the same chunk repeatedly if the same dyadic interval is traversed multiple times as we process the input. 
%In particular, the random samples for the hash functions at the root is viewed for almost every input element. 
\\
To show the correctness of using Nisan's generator, we have to convert our sketching algorithm to a model algorithm that only has one-way access to the random bits. The model algorithm is purely theoretic and we do not care about its running time, so it can process the input stream \emph{in any sequence} (as it is allowed to scan the stream for the scratch for the next desired input.) Recall that our input stream consists of disjoint dyadic intervals, so in particular, we assume the model algorithm processes these intervals in increasing order, whose range-minimums can be generated by a one-way pre-order traversal of all vertices (and their randomness) of the simulation tree. Using a Depth First Search (DFS) algorithm, our model algorithm can return the sketch $Y[k]$ while storing the samples $B$ and $W$ of $O(\log U)$ ancestor vertices, which takes  $\tilde{O}(\log\frac{1}{\epsilon}\log U)$ bits in total (neglecting higher order logarithms). Therefore, we can generate the random bits with a Nisan's generator that performs $\tilde{O}(\log U)$ arithmetic operations on $\tilde{O}(\log\frac{1}{\epsilon}\log U)$-bit words for each random sample, and the size of the seed is $\tilde{O}(\log\frac{1}{\epsilon}\log^2 U)$.
\\
Since we use an independent simulation tree for each sketch, the pseudorandom seeds (which is the dominant term of memory complexity) is $\tilde{O}(\frac{1}{\epsilon^2}\log\frac{1}{\epsilon}\log\frac{1}{\delta}\log^2 U)$. For each input tuple, the update of all sketches takes $\tilde{O}(\frac{1}{\epsilon^2}\log\frac{1}{\delta}\log^2 U)$ arithmetic operations. Note that this is the (worst case) complexity for a theoretical guarantee. In practice, we can use very fast hash functions (such as wyhash\footnote{\url{https://github.com/wangyi-fudan/wyhash}}) to generate random bits for the samples and observe nearly no degradation in performance. With these hash functions, the practical complexity of using dyadic simulation for estimating $L_0$ is $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta})$ space and $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta}\log U)$ time, which matches the complexity of \cite{rangeeff} in terms of $U$, although our scheme is much simpler and requires no explicit finite field operations.
(note: we can easily aggregate sketches from different sources, but \cite{rangeeff} cannot.)}

-----------------------------------------------------------------------------------------------------\\
+++++++++++++++++++++++++++++++++++++++++\\
\end{comment}

========================== moved in the second time

%\subsection{DST Implementation with Nisan's PRNG}\label{sec:nisandst}

\begin{comment}

The second implementation uses Nisan's PRNG~\cite{nisan} to generate the random strings $C_{\alpha*}$.
%To begin with, we show some backgrounds on Nisan's PRNG. , any algorithm in $space(S)$ (in with aprovides the following theoretical guarantee according toFor any finite state machine (FSM) that uses  $R$  random bits, (the algorithm consumes these bits in $O(S)$ chunks and one chunk at a time) $W^l_{(i*)}$, which ``fools'' any finite state machine (FSM) , 
Nisan's PRNG can expand a random seed of $O(S\log R)$ bits into $R$ pseudorandom bits that look indistinguishable from truly random (independent and uniform)  bits to any finite state machine FSM that uses $S$ bits of memory (having at most $2^S$ states). %which reads only a chunk of $O(S)$ bits at one time. 
\end{comment}

\begin{comment}
The meaning of ``indistinguishable'' is as follows. After consuming all input bits, the final state of the FSM follows a distribution that is a function of the distribution of its inputs. We denote this function as  $D(\cdot)$, the distribution of truly random bits as $T$, and the distribution of pseudorandom bits generated by Nisan's PRNG as $P$. Both $D(T)$ and $D(P)$ are regarded as a vector with $2^S$ coordinates, and the value at each coordinate equals to the probability of having the corresponding state as the final state.
% We treat the distribution of the running result as  $D(X)$ with  depending on the distribution of the input $X$. We define that the random variable $X$ is uniformly randomly drawn from $\{0, 1\}^R$, and $Y$ is the generating result of Nisan's PRNG from a uniform random seed of $O(S\log R)$ bits.
\begin{theorem}\cite{stabledist}\label{th:nisan}
With the definitions above, the following bound on the $L_1$ difference between two vectors $D(T)$ and $D(P)$ (or equivalently, the total-variation distance between two distributions)  holds
\begin{equation}\label{eq:nisan}
\|D(T) - D(P)\|_1 \leq 2^{-O(S)}.
\end{equation}
Nisan's PRNG can be implemented with $O(S)$ storage, apart from the $O(S\log R)$-bit seed, and any chunk of $O(S)$ bits can be computed using $O(\log R)$ arithmetic operations on $O(S)$-bit words. 
\end{theorem}

In the second implementation,
we generate $W^l_{(i*)}$ by transforming from the pseudorandom chunk $C_{2^l+i}$.
\end{comment} 

\begin{comment}
Each DST uses $O(U)$ such chunks (the same number as $W$'s), so supposing each chunk is of $B$ bits, the number of pseudorandom bits consumed by each DST is $R=O(BU)$. %We will use Nisan's PRNG to fool the DST and its downstream application together, which can be regarded as an FSM with space bound $S$, so 
In our case, the FSM refers to the DST together with the downstream algorithm (\eg Indyk's algorithm in \autoref{sec:datastreaming}), and its final state refers to the raw statistics.
Supposing the space bound of the FSM is $S$ for the moment, the space complexity of Nisan's PRNG is $O(S\log R)$, which dominates the space complexity of the DST based on it. %, where $S$ is the space bound of the DST when converted to an FSM. %, and each DST uses $U$ chunks $C_0, C_1, \cdots, C_{U-1}$ ($C_0$ generates the range-sum of uour algorithm can be regarded as an FSM withniverse). dominated by the seed of (The specification of the downstream algorithm and the proof for space bound are in )
Each split that requires a $W$ takes $O(\log BU) = O(\log U)$ arithmetic operations (because $B\ll U$), so the time complexity for computing any range-sum is $O(\log^2 U)$ by \autoref{cor:2logntime}.
% is generated from   resulted in applying a low-level .offers a stronger theoretical guarantee in the following sense. of this implementation in , which is required for application-level guarantees inwe can always set \autoref{sec:datastreaming}, as in all applications described in \autoref{sec:datastreaming}space and

Although the  time complexities of using Nisan's PRNG is higher than using hash functions by a factor of $\log U$, the former is more powerful in that it completely emulates the ideal case and provides all theoretical guarantees in it as long as the downstream algorithm is space-bounded. This result is useful for the theoretical guarantees of the $L_1$ streaming algorithm in  \autoref{sec:dstheo}. %That is because,  \textbf{$S$ is usually large enough (say $O(\log U)$ in all applications described in \autoref{sec:datastreaming})} to make the right-hand side of \autoref{eq:nisan} negligibly small, so $D(P)$ becomes indistinguishable from $D(T)$. Therefore, it is impossible to distinguish from the final state of the downstream algorithm whether true random bits or pseudorandom bits are used, so in both cases, the final state has the same theoretical guarantees.  %Therefore, the second implementation with Nisan's PRNG provides the same theo the final state of FSM follows nearly the same distribution  $\approx D(T)$.retical guarantand has the same guarantees under these two cases .ees as the ideal case.

\end{comment}

\begin{definition}
	A (randomized) streaming algorithm returns an $(\epsilon, \delta)$-approximate estimator $\hat{d}_1$ if the probability for the relative error to be greater than $\epsilon$ is at most $\delta$, \ie
	$	\Pr(|d_1 - \hat{d}_1| > \epsilon d_1 ) < \delta.$
\end{definition} 



\begin{comment}
By the stability property, supposing the singletons $X_0, X_1, \cdots, X_{U-1}$ (we drop the superscript $j$ here, because the same is true for each $j=1,2, \cdots, r$) are i.i.d. (an ideal case that will take too much space to generate these random variables), the distribution of each sketch $A$ is 
%determined by the stability property: It is 
$\mathcal{N}(0, d_2^2)$ for $L_2$ estimation and $\mathrm{Cauchy}(0, d_1)$ for $L_1$ after the online stage. The only remaining task is to estimate the parameters $d_2$ or $d_1$ from the sketches $A[1\cdots r]$, which is treated as random samples from these distributions.

For $L_2$ norm, Indyk's algorithm~\cite{stabledist} uses the following estimator for the variance of a Gaussian random variable with known mean $0$. %square of $L_2$ norm
%, we will use the following UMVUE\cite{sttinf} for $d^2_2$, the variance of Gaussian samples whose expectation is known,
\begin{equation}\label{eq:gauesti}
\hat{d}_2^2 = \frac{A^2[1]+A^2[2] + \cdots+A^2[r]}{r}.
\end{equation}
By a simple application of Chebyshev's inequality, this probability for an estimate to fail (to have larger relative error than $\epsilon$) can be bounded by $1/4$ with $r = O(1/\epsilon^2)$ sketches. To further boost the success probability to $1-\delta$ for arbitrarily small $\delta$, Indyk's algorithm performs $O(\log 1/\delta)$ independent estimations and use the median of all estimates as the final estimate. 

\begin{comment}

+++++++++++++++++++++++++++++++++++++++++\\
-----------------------------------------------------------------------------------------------------

\textcolor{teal}{For $L_2$ estimation, we will use the following UMVUE\cite{sttinf} for $d^2_2$, the variance of Gaussian samples whose expectation is known,
\begin{equation}\label{eq:gauesti}
\hat{d}_2^2 = \frac{Y^2[1]+\cdots+Y^2[l]}{l}.
\end{equation}
5. The variance of the estimator is $Var[\hat{d}_2^2] = \frac{2d_2^4}{l}$. By Chebyshev's inequality, the following large deviation bound holds
\begin{displaymath}
\mathcal{P}\left(\left|\hat{d}_2 - d_2\right|\geq \epsilon d_2\right) \leq 	\mathcal{P}\left(\left|\hat{d}^2_2 - d^2_2\right|\geq \epsilon d^2_2\right) \leq \frac{2}{\epsilon^2 l}.
\end{displaymath}
6. With $l = O(1/\epsilon^2)$ sketches, this probability for an estimator to fail (to have larger relative error than $\epsilon$) can be bounded by $1/4$. We then repeat the \autoref{algo:indyk} for $O(\log 1/\delta)$ times and take the median of all estimates. This median fails only if more than half of the estimators fail, so with $O(\log 1/\delta)$ independent estimates, the probability that the median fails is less than $\delta$. In this way,  we have an $(\epsilon, \delta)$-approximate estimator for $L_0$ with $O(\frac{1}{\epsilon^2}\log \frac{1}{\delta})$ sketches (and the same memory overhead).}

-----------------------------------------------------------------------------------------------------\\
+++++++++++++++++++++++++++++++++++++++++
\end{comment}
%So far we have described Indyk's algorithm, and now we show why the timethat are indistinguishable from the  RVs that follow   in the ideal case.  complexity canso they are be an issue for interval streams. To analyze the time complexity of Indyk's algorithm, we focus on the time complexity of the online stage: in particular the time of each update for an input tuple in the stream. The time complexity for each update is the time to update each sketch multiplied by the total number of sketchesTo meet the ``indistinguishable'' guarantee, the RVs $X_0, X_1, \cdots, X_{U-1}$ are generated from Nisan's PRNG, whose output is indistinguishable from being truly random (as in the ideal case) to any space-bounded finite space machine (FSM).  $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta})$. In Indyk's original algorithm, the update for each point input $(i_t, \delta_t)$ is to increment $c\cdot X_{i, j}$ to each sketch, and if the input is an interval $([a_t, b_t), \delta_t)$, the increment is a range-sum  $c\cdot\sum_{i=a_t}^{b_t-1} X_{i, j}$ of the hash values. Even if each $X_{i, j}$ can be evaluated with low complexity (say $O(1)$), this algorithm does not scale to large intervals $[a, b)$ since $b-a$ might be gigantic. Fortunately, we can use dyadic simulation to direct generate range-sums (summing over $i$ for any fixed $j$, and we will use one independent instance of simulation tree for each $j$) in $O(\log U)$ time instead of $b-a$ (which is $O(U)$ in the worst case). Therefore, with dyadic simulation, each update of Indyk's algorithm can be efficiently performed in $O(\frac{1}{\epsilon^2}\log\frac{1}{\delta}\log U)$ time even for arbitrary interval inputs.for any estimatorand when the accuracy of estimation is guaranteed as in~.when all underlying random variables are mutually independentto generate underlying random variablesCauchy

%\subsection{Estimation of $L_2$ with Range-updates}\label{sec:ersl2}
%[may be duplicate to the one in intro] As shown in \autoref{sec:streamintro}, Indyk's algorithm has high time complexity when directly applied to a range-update data stream whose updates are gigantic intervals. Hopefully, at the arrival of tuple $([a_t, b_t), \delta_t)$, the range-update on \autoref{indyk:update-new} boils down to the range-sum $\sum_{i=a_t}^{b_t-1} X_i^j$, which can be efficiently generated by ERS procedures such as dyadic simulation. % can significantly reduce the time complexity of computing each range-update. 
% In this section, we show that with dyadic simulation, we can easily generate range-updates  that make Indyk's algorithm efficient from range-sums of Gaussian and Cauchy random variables. 
%we current do not know {\bf }


%Theoretically, we will show that, by using generation schemes with stronger guarantees, we can achieve $(\epsilon, \delta)$-approximation of the $L_1$ and $L_2$ norms respectively while inflating the complexities of dyadic simulation only slightly.
\begin{comment}

+++++++++++++++++++++++++++++++++++++++++\\
-----------------------------------------------------------------------------------------------------

\textcolor{teal}{For the running time, \autoref{algo:indyk} differs from Indyk's original algorithm in \autoref{indyk:update}. The original algorithm only handles a stream of point updates in the form of $(j_i, c_i)$ and increments $c_i\cdot sh(j_i)$ to each sketch. Our improved algorithm handles interval updates, and correspondingly, the increment is a range-sum $ c_i\cdot \sum_{j=a_i}^{b_i} sh_i(j)$. Therefore, in order for low update complexity, we need a family of range-summable Gaussian (or Cauchy) random variables indexed by $j\in\mathcal{U}$ for each $sh_i$. With dyadic simulation, each update for all sketches only takes $O(l\log U\log )=O(\frac{1}{\epsilon^2}\log  U \log\frac{1}{\delta} )$ time.}

-----------------------------------------------------------------------------------------------------\\
+++++++++++++++++++++++++++++++++++++++++
\end{comment}

%So far in describing Indyk's algorithm, we have assumed that all the random variables $X_{i, j}$ are mutually independent in order to apply the stability property. As we have mentioned above, in order to consistently access this large number ($rU$) of random variables, we have to either use hash functions or Nisan's PRNG to reduce the demand in memory, so readers may worry if these alternatives will compromise the performance of Indyk's algorithm. Empirically, the answer is ``no'', supported by the Kolmogorov-Smirnov testing on an artificial data stream in \autoref{sec:kstest}, in which the random variables are generated by our implementation of dyadic simulation with off-the-shelf hash functions.

% an assumption widely used in the data streaming context~\cite{ams} (Tug-of-War) and is slightly stronger than some existing hash functions such as tabulation hashing~\cite{tabulation}, which is three-wise independent. The reason is from the following fact, which can be proved by simply comparing each term of the power-$k$ multinomial expansion and applying $k$-wise independence on the product of expectations. %(when $X_0^j, X_1^j, \cdots,  are mutually independent).
%We also worked out how to achieve the same theoretical guarantee as in the ideal case while using hash functions or Nisan's PRNG to limit the memory footprint to polylog$(U)$.
% we have a strong guarantee  

%\begin{theorem}\cite{ams}\label{th:fourwise2}
%	Let $r= 16/\epsilon^2$. If the underlying random variables $X_i^j$ for $i=0, 1, \cdots, U-1$ and %$j=1,2,\cdots, r$ are four-wise independent and they all follow distribution $X$ with $E[X] = 0$ and $Var[X] = 1$, then the probability that the estimator in \autoref{eq:gauesti} deviates from $d^2_2$ by at more than $\epsilon d^2_2$ is at most $1/8$. %the probability for an estimate to fail (to have larger relative error than $\epsilon$ can be bounded by $1/4$ with $r = O(1/\epsilon^2)$ accumulators. and use the median of all estimates as the final estimate
%	To further boost the success probability to $1-\delta$ for arbitrarily small $\delta$, the streaming algorithm only needs to return the median of $2\log 1/\delta$ independent estimations as above. 
%\end{theorem}to guarantee $(\epsilon, \delta)$-approximation with $O(1/\epsilon^2\cdot\log1/\delta)$ accumulators, $X^j_0$, $X^j_1$, $\cdots$, $X^j_{U-1}$ are required to be four-wise independent, but not necessarily mutually independent.\autoref{th:fourwise}underlying random variables are four-wise independent if the
%, which results in $O(1/\epsilon^2\log1/\delta\log U)$ complexity in both storing the accumulators and the time for each range-update.
%For the estimation of $L_2$ norm, to achieve the same performance guarantee as above, dyadic simulation only requires the hash functions used for the splits to be four-wise independent, to run one DST that serves 
%and the four-wise independence of low-level hash functions  used in the implementation are 
%which can be achieved by evaluating a polynomial of degree $3$ modulus a prime number $p$ (polynomial hashing) or by tabulation hashing~\cite{tabulation4wise}. 
%\begin{fact}\label{fact:kmoment}
\begin{comment}
Suppose the deterministic function $\mathcal{O}(\mathbf{X}) = \sum_{i=0}^{U-1}\sigma_i X_i$ is a linear combination of the elements of its input, where $\mathbf{X}$ is a $U$-dimensional random vector. Suppose we know the marginal distribution of each element $X_i$, $i=0, 1, \cdots, U-1$, and that the elements of $\mathbf{X}$ are $k$-wise independent, then $E[\mathcal{O}^{k}(\mathbf{X})]$ is a determined constant that does not depend on whether the elements of $X$ are mutually independent or not.%by observing $E[\mathcal{O}^{k}(\mathbf{X})]$.
%\end{fact}

When the online stage terminates, each accumulator $A[j] = \sum_{i=0}^{U-1} \sigma_i X_i^j$.
%Suppose the value of counters (defined in \autoref{sec:streamintro}) are $\sigma_0, \sigma_1, \cdots, \sigma_{U-1}$ after the online stage. At that time, 
% is a linear combination of some random variables with fixed coefficients .
By \autoref{fact:kmoment}, we cannot tell from the expectation $E[A^2[j]]$ whether the random variables $X_0^j, X_1^j, \cdots, X_{U-1}^j$  for any fixed $j$ are mutually independent as long as they are two-wise independent. By the linearity of expectation, $E[\hat{d}_2^2] = 1/r\cdot \sum_{j=1}^rE[A^2[j]]$, which is the same expectation as in the ideal case, so the estimator for $d_2^2$ is unbiased because it is unbiased in the ideal case. Furthermore, because the sequences $X_0^j, X_1^j, \cdots, X_{U-1}^j$ for different $j$ are generated from independent instances of simulation trees, $A[j]$ are mutually independent for $j=1, 2, \cdots, r$. Therefore, by \autoref{fact:kmoment}, we cannot tell from the variance of the estimator, which is 
\begin{align}
Var[\hat{d}_2^2] &= E[\hat{d}_2^4] - E^2[\hat{d}_2^2] \nonumber\\&= \frac{1}{r^2}\cdot \left(\sum_{j=1}^r E[A^4[j]] + 2 \sum_{j=1}^k \sum_{j'=1}^{j-1}E[A^2[j]A^2[j']]\right) - E^2[\hat{d}_2^2], %if the random vector $(X_{i,j})_{i=0, 1, \cdots, U-1}$ are mutually  
\end{align}
whether $X_0^j, X_1^j, \cdots, X_{U-1}^j$ for each $j$ are mutually independent as long as they are four-wise independent. By \autoref{th:nwise}, using one four-wise independent on each level of our dyadic simulation algorithm generates four-wise independent singletons (elements) in $X_0^j, X_1^j, \cdots, X_{U-1}^j$ for each fixed $j$, so both the expectation and the variance of the estimator exactly equal to those in the ideal case, which fact leads to the same $(\epsilon, \delta)$-approximation  guarantee from Chebyshev's inequality.
\end{comment}



%Our $L_2$ scheme is an exception: only  (wyhash, like most popular hash functions, is not four-wise independent theoretically) hash functions, instead of Nisan's generator are required for theoretical guarantee of $(\epsilon, \delta)$-approximation. That is, again, because of the two ``nice'' properties of Gaussian distribution. Firstly, the final value (after processing the stream) of each sketch $Y[k]$ is a linear combination of $S_\mathcal{E}$ and $W_{\alpha}$'a (for all possible dyadic intervals $\alpha$ in the simulation tree), because of the linear property of dyadic simulation for Gaussian (Lemma\,\ref{th:leafsamp}). Secondly, since the Gaussian distribution is sufficiently concentrated, it is a common practice to use the root mean square \autoref{eq:gauesti} instead of the median as the estimator~\cite{stabledist}. Therefore, we can bound the variance of the estimator as long as the linear components $W_{\alpha}$ are four-wise independent (by applying a four-wise independent hash function on the binary prefix like $W_\alpha = h(\alpha)$), for the same reasoning as in the AMS sketch~\cite{ams}. \textbf{Feigenbaum for L2?}

%JFM-9 (from old 5.2.10) Note that the time complexities shown in the last paragraph are based on the assumption that each hash value $sh_i(j)$ can be evaluated in $O(1)$ time. This is true in the practical sense, because we can just use off-the-shelf hash functions as each $sh_i(\cdot)$, which has only $O(1)$ complexity and generates empirically ``independent'' hash values, as will be shown in ??. Due to the space limits, we will not give a thorough performance evaluation on the data streaming application for the lack of benchmarks and competitors, but focus on the ANNS application in ??.



%For $L_1$ norm, % If theoretical guarantees are required (instead of empirical performance relying on the off-the-shelf hash functions). Actually, Indyk's original algorithm~\cite{stabledist}  also faces the same problem, since it requires the generation of $O(U)$ independent random variables ($X_i$ above), but the requirement of being $U$-wise independent is too strong and can hardly be implemented in small space. W
%We postpone the proof to \autoref{sec:dstheo} after describing the next streaming application on estimating the $F_0$ moment, because %it is technical and requires some background knowledge on Nisan's PRNG.
%the proofs are similar for these two algorithms.


\begin{comment}

+++++++++++++++++++++++++++++++++++++++++\\
-----------------------------------------------------------------------------------------------------

\textcolor{teal}{
The descriptions above rely on two assumptions: 1) All random samples are generated with infinite precision. 2) All random samples are independent.
%As in Indyk's original algorithm, \autoref{algo:indyk} relies on the stability property of stable distribution, which requires the hashes to be  Because it is hard to generate $U$ independent random variables in small memory, 
As in Indyk's original algorithm, we remove these assumptions by using Nisan's pseudorandom generator \cite{nisan} to generate random variables (with fixed precision) that looks independent to our small-memory sketching algorithm. %The theoretical proof of $(\epsilon, \delta)$ approximation resembles that of $L_0$ estimation, so we do not provide a separate proof for $L_1$ and $L_2$ in this paper.
The theoretical guarantees of these generators will be specified in \autoref{sec:gautheo} and \autoref{sec:cautheo}.}

-----------------------------------------------------------------------------------------------------\\
+++++++++++++++++++++++++++++++++++++++++
\end{comment}


%\subsection{Theoretical Guarantees for Data Streaming}
%In this section, we show how to apply Nisan's PRNG for a theoretical approximation guarantee of our data streaming algorithms with dyadic simulation. In particular, we show the time and space complexities of achieving $(\epsilon, \delta)$-approximation. We first describe the proof of Indyk's original algorithm~\cite{stabledist} for standard streams (with point-updates), and then generalize it to apply to dyadic simulation for range-update streams.%so we only provide a sketchy proof that focuses on the differences between dyadic simulation and Indyk's original algorithm.for the splits

%We now describe how to bring the theoretical guarantees in the ideal case to practical settings. The median estimator is not ``well-bahaved'', so the argument for $L_2$ cannot be used. \cite{stabledist} generated raw statistics from Nisan's PRNG.  Since the online stage is an FSM with small space, it cannot tell whether it is in the ideal case or is being fooled by Nisan's PRNG, so the distribution of its final state (the raw statistics) is indistinguishable from that in the ideal case, which is $\mathrm{Cauchy}(0, d_1)$. In this way, any estimator on the raw statistics achieves the same theoretical guarantee of $(\epsilon, \delta)$-approximation as in the ideal case.  



%To support range-updates for $L_1$ estimation, we generate $X_0, X_1$, $\cdots$, $X^j_{U-1}$ with a DST for standard Cauchy singletons, similar to $L_2$ estimation. In order to have the same theoretical guarantees as for point-updates, such a DST needs to be implemented on Nisan's PRNG  as in~\autoref{sec:nisandst}, so that the raw statistics can be indistinguishable from those in the ideal case just as in Indyk's original proof~\cite{stabledist}. Here, the algorithm that lies between the PRNG and the raw statistics is composed by both the DST and the online stage, which is an FSM with roughly $O(\log U)$ space. This is proved by a standard extension of Indyk's proof in~\cite{stabledist} to DSTs. {\bf Since our proof has many parts are in common with Indyk's proof, we skip our proof and directly show the complexities of our $L_1$ estimation algorithm.}
% Since our range-updating version works in the same way as the point-update version of Indyk's algorithm in~\cite{stabledist} works, 



%By \autoref{sec:nisandst}, the space complexity of each DST, dominated by the seed of Nisan's PRNG, is $O(S\log U)$, where $S=O(\log U)$ is the space bound for the composition of the DST and the online stage. Therefore, 
%Substituting the space bound by $S=B$, it becomes 
%the space complexity becomes $O(\log ^2 U)$, which is the same as
%the time complexity for each range-update shown in \autoref{sec:nisandst}. For %achieving $(\epsilon, \delta)$-approximation, the complexities above should be multiplied by $O(1/\epsilon^2\log1/\delta)$, the number of accumulators used in Indyk's algorithm.
%the raw statistics of this accumulator after the online stage is indistinguishable from the Cauchy random variables in the ideal case.
%We show that  that in the ideal case where $X_0, X_1, \cdots, X_{U-1}$ are i.i.d., by showing that .  as ~\cite{stabledist}
%Therefore, our solution achieves $(\epsilon, \delta)$ approximation for the same reason Indyk's point-update algorithm does.

%all the arguments of  can also be applied to our solution,  %which uses $U$ independent random chunks (one for the sum of universe and $U-1$ for each non-leaf vert(by using Nisan's PRNG)ex) to generate $U$ mutually independent random variables.our dyadic simulationrange-update streaming . Here, , which is supported by one DST implemented with Nisan's PRNG as in \autoref{sec:nisandst}. We will show that , so the theoretical guarantees of Indyk's algorithm generalizes to the wayalgorithmachieves theoretical guarantees  


